A Catalog of 531 White Dwarf Candidates in the Local Galactic Halo from Gaia Data Release 2

We present a catalog of 531 white dwarf candidates that have large apparent transverse motions relative to the Sun ($v_{T} > 200$ km s$^{-1}$), thus making them likely members of the local Galactic halo population. The candidates were selected from the Gaia Data Release 2, and are located in a great circle with $20^\circ$ width running across both Galactic poles and Galactic center and anti-center, a zone that spans 17.3% of the sky. The selection used a combination of kinematic and photometric properties, derived primarily from Gaia proper motions, $G$ magnitudes, and $G_{{\rm BP}}\,-\,G_{{\rm RP}}$ color, and including parallax whenever available. Additional validation of the white dwarf candidates is made using PanSTARRS photometric ($gri$) data. Our final catalog includes not only stars having full kinematic and luminosity estimates from reliable Gaia parallax, but also stars with presently unreliable or no available Gaia parallax measurements. We argue that our method to select local halo objects with and without reliable parallax data leads us to rounding up all possible halo white dwarfs in the Gaia catalog (in that particular section of that sky) with recorded proper motions $> 40$ mas yr$^{-1}$, and that pass our $v_{T} > 200$ km s$^{-1}$ threshold requirement. We expect this catalog will be useful for the study of the white dwarf population of the local Galactic halo.

==> tab1.tex <==
\begin{deluxetable*}{ccc}
\tablecolumns{3}
\tablewidth{0pt}
\tabletypesize{\small}
\tablecaption{Assumed Saturation and Detection Limits of \panstarrs Filters \label{tab:tab1}}
\tablehead {
   \colhead{} &
   \colhead{Bright End} &
   \colhead{Faint End} \\
   \colhead{Filter} &
   \colhead{(mag)} &
   \colhead{(mag)}
}
\decimals
\startdata
$g$ & $14.5$ & $22.5$ \\
$r$ & $15.0$ & $22.0$ \\
$i$ & $15.0$ & $21.0$
\enddata
\end{deluxetable*}



==> tab2_seta.tex <==
\begin{longrotatetable}
\begin{deluxetable*}{lcccccccclccccccccc}
\tablecolumns{19}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecaption{High-velocity White Dwarf Candidates in Set A \label{tab:tab3}}
\tablehead {
   \colhead{} &
   \colhead{RA} &
   \colhead{Dec} &
   \colhead{$\pi$} &
   \colhead{$\sigma_{\pi}$} &
   \colhead{$\mu_{\alpha}$} &
   \colhead{$\mu_{\delta}$} &
   \colhead{$G$} &
   \colhead{} &
   \colhead{} &
   \colhead{$r_{\rm PS}$} &
   \colhead{} &
   \colhead{} &
   \colhead{$v_{T,\,r}$} &
   \colhead{$v_{T,\,s}$} &
   \colhead{$v_{T,\,{\rm tot}}$} &
   \colhead{Halo WD} &
   \colhead{} &
   \colhead{} \\
   \colhead{source\_id} &
   \colhead{(deg)} &
   \colhead{(deg)} & 
   \colhead{(mas)} &
   \colhead{(mas)} &
   \colhead{(mas yr$^{-1}$)} &
   \colhead{(mas yr$^{-1}$)} &
   \colhead{(mag)} &
   \colhead{$\bpmrp$} &
   \colhead{PS1\_ID} &
   \colhead{(mag)} &
   \colhead{$g_{\rm PS}\,\,-\,\,r_{\rm PS}$} &
   \colhead{$r_{\rm PS}\,\,-\,\,i_{\rm PS}$} &
   \colhead{(km s$^{-1}$)} &
   \colhead{(km s$^{-1}$)} &
   \colhead{(km s$^{-1}$)} &
   \colhead{Likelihood (\%)} &
   \colhead{Spec\_Type} &
   \colhead{Ref.}
}
\decimals
\startdata
  2313554227856823296 & 0.535536 & -32.6280206 & 0.82 & 0.46 & 8.03 & -45.02 & 19.182 & 0.173 & \nodata & \nodata & \nodata & \nodata & 75.48 & -253.3 & 264.3 & 52.14 & \nodata & \nodata  \\
  2313582750735435776 & 0.6362011 & -32.1969737 & 5.131 & 0.124 & 268.55 & -79.49 & 16.36 & -0.317 & \nodata & \nodata & \nodata & \nodata & -188.42 & -177.27 & 258.7 & 100.0 &  DA2  & 6, 8, 29  \\
  2314458438731730304 & 0.8042194 & -31.5123699 & 0.864 & 0.898 & 40.92 & -7.09 & 20.17 & -0.042 & \nodata & \nodata & \nodata & \nodata & -182.72 & -136.19 & 227.89 & 50.04 &  DA  & 11  \\
  2319735617804258176 & 1.7831581 & -31.227056 & 7.721 & 0.11 & 351.93 & -127.25 & 16.665 & -0.263 & \nodata & \nodata & \nodata & \nodata & -155.88 & -168.77 & 229.74 & 100.0 &  DB3  & 4, 6, 13, 29  \\
  4995158325163347712 & 3.4196121 & -42.3757786 & 1.829 & 0.299 & 44.67 & -73.22 & 19.239 & -0.048 & \nodata & \nodata & \nodata & \nodata & -10.57 & -221.97 & 222.22 & 72.76 & \nodata & \nodata  \\
  2361176034960819840 & 4.6151947 & -22.3484057 & 1.275 & 0.527 & -8.87 & -68.78 & 19.699 & -0.256 & 81180046151242467 & 19.813 & -0.322 & -0.292 & 153.48 & -207.07 & 257.75 & 71.19 & \nodata & \nodata  \\
  2315640040069969152 & 7.5363943 & -32.7341348 & 4.263 & 0.361 & 269.88 & -60.1 & 19.292 & 0.194 & \nodata & \nodata & \nodata & \nodata & -224.95 & -209.53 & 307.41 & 100.0 & WD & 29  \\
  2363517582411486848 & 7.8066904 & -19.225289 & 3.227 & 0.731 & 68.39 & -149.9 & 20.135 & 0.386 & 84930078065380258 & 20.141 & 0.087 & 0.005 & 27.12 & -240.52 & 242.05 & 77.7 & \nodata & \nodata  \\
  5003556566771814784 & 8.5379902 & -37.9679847 & 0.681 & 0.652 & 39.79 & 22.04 & 20.269 & 0.165 & \nodata & \nodata & \nodata & \nodata & -316.18 & -12.03 & 316.41 & 50.52 & \nodata & \nodata  \\
  4925117858217935232 & 9.5387368 & -52.5192925 & 2.116 & 0.485 & 102.79 & -72.65 & 20.003 & 0.074 & \nodata & \nodata & \nodata & \nodata & -101.59 & -262.98 & 281.92 & 88.96 & \nodata & \nodata  \\
  5004294102850782464 & 10.1559533 & -35.6549912 & 2.785 & 0.52 & 123.76 & 42.12 & 19.679 & 0.088 & \nodata & \nodata & \nodata & \nodata & -216.71 & -50.29 & 222.47 & 70.54 & \nodata & \nodata  \\
  2369026857221068160 & 11.2063791 & -18.441024 & 1.475 & 0.255 & 54.15 & -118.71 & 18.395 & -0.06 & 85870112062521343 & 18.519 & -0.249 & -0.216 & 58.46 & -415.21 & 419.31 & 99.87 & \nodata & \nodata  \\
  5006232026455470848 & 11.3410844 & -33.4977869 & 30.373 & 0.22 & 1826.61 & -1485.17 & 18.642 & 1.508 & \nodata & \nodata & \nodata & \nodata & -116.8 & -348.34 & 367.4 & 100.0 & WD & 29  \\
  5007556727512756096 & 11.4801246 & -31.7755257 & 0.699 & 1.089 & 46.45 & 8.49 & 20.218 & -0.358 & \nodata & \nodata & \nodata & \nodata & -297.0 & -120.0 & 320.33 & 53.63 &  DA  & 7, 11  \\
  2372908034482552832 & 13.748219 & -14.016694 & 1.672 & 0.592 & 89.67 & -28.42 & 19.825 & -0.345 & 91180137480440369 & 19.942 & -0.309 & -0.250 & -165.77 & -208.84 & 266.63 & 76.23 & \nodata & \nodata  \\
  2469456695978419584 & 14.3092532 & -12.1422892 & 0.977 & 0.712 & -24.84 & -49.75 & 19.903 & -0.091 & 93420143093019686 & 19.945 & -0.191 & -0.226 & 235.69 & -131.03 & 269.67 & 62.64 & \nodata & \nodata  \\
  2359691969141234688 & 15.9303474 & -15.6287856 & 1.848 & 0.433 & 78.51 & -1.43 & 19.702 & 0.005 & 89240159302195850 & 19.763 & -0.225 & -0.259 & -163.58 & -117.59 & 201.46 & 51.41 & \nodata & \nodata  \\
  4989103211547483008 & 15.9375594 & -38.4739653 & 0.893 & 0.809 & 79.77 & -18.3 & 20.424 & -0.197 & \nodata & \nodata & \nodata & \nodata & -291.06 & -322.43 & 434.37 & 71.33 & \nodata & \nodata  \\
  2531264986219740800 & 17.1346381 & -3.4835573 & 2.31 & 0.467 & 75.18 & -152.2 & 19.362 & 0.158 & 103820171345540377 & 19.422 & -0.169 & -0.214 & 62.8 & -342.66 & 348.37 & 98.14 & \nodata & \nodata  \\
  2468676832996940928 & 19.0224697 & -12.587698 & 1.445 & 0.731 & 59.51 & -53.77 & 20.247 & -0.257 & \nodata & \nodata & \nodata & \nodata & -54.04 & -257.43 & 263.04 & 68.32 & \nodata & \nodata  \\
  4983403686865974272 & 19.516898 & -43.613763 & 3.268 & 0.494 & 148.11 & -28.56 & 19.86 & 0.169 & \nodata & \nodata & \nodata & \nodata & -145.01 & -163.83 & 218.79 & 71.95 & \nodata & \nodata  \\
  4983806318576707968 & 20.5993947 & -43.0846862 & 1.153 & 0.361 & 50.78 & -23.39 & 19.765 & -0.182 & \nodata & \nodata & \nodata & \nodata & -105.18 & -204.32 & 229.81 & 66.72 & \nodata & \nodata  \\
  2353722823593430016 & 21.1781918 & -20.2851088 & 1.773 & 0.574 & 65.72 & -76.31 & 19.643 & -0.041 & 83650211781048383 & 19.708 & -0.122 & -0.238 & -20.36 & -268.46 & 269.23 & 78.61 & \nodata & \nodata  \\
  4935444952462713984 & 21.7545609 & -44.1297011 & 3.24 & 0.564 & 281.01 & 29.24 & 20.259 & 0.602 & \nodata & \nodata & \nodata & \nodata & -347.08 & -224.41 & 413.31 & 99.83 & \nodata & \nodata  \\
  5015458647000212608 & 23.7649748 & -32.9983708 & 5.003 & 0.101 & -10.01 & -264.38 & 17.423 & -0.115 & \nodata & \nodata & \nodata & \nodata & 161.8 & -191.48 & 250.68 & 100.0 & WD & 29  \\
  2480893128736076544 & 23.892485 & -3.9558741 & 7.14 & 0.512 & 473.86 & -191.91 & 19.567 & 0.695 & \nodata & \nodata & \nodata & \nodata & -167.08 & -295.43 & 339.4 & 100.0 &  DA  & 6, 9, 29  \\
  2508720531084154624 & 25.5870249 & -1.3990516 & 6.435 & 0.472 & 110.04 & -344.33 & 18.501 & 0.128 & \nodata & \nodata & \nodata & \nodata & 97.59 & -247.73 & 266.26 & 99.97 &  DA  & 6, 9, 29  \\
  5135685360118110336 & 26.7861506 & -21.4801115 & 1.154 & 0.392 & -5.97 & -82.35 & 19.385 & -0.019 & 82220267861284279 & 19.476 & -0.255 & -0.227 & 229.03 & -249.92 & 339.0 & 88.62 & \nodata & \nodata  \\
  5139236370359249024 & 26.9629875 & -19.9986568 & 0.708 & 0.6 & 39.84 & 19.43 & 19.891 & 0.045 & 84000269629361927 & 19.923 & -0.032 & -0.153 & -289.79 & -63.59 & 296.69 & 54.55 & \nodata & \nodata  \\
  5142197118950177280 & 27.0376675 & -17.2087647 & 12.954 & 0.149 & -105.97 & -1105.83 & 17.558 & 0.47 & \nodata & \nodata & \nodata & \nodata & 281.6 & -293.13 & 406.48 & 100.0 &  DA6.9  & 6, 9, 28, 29  \\
  5139287360210678144 & 27.0492797 & -19.8039312 & 1.61 & 0.269 & -15.05 & -72.55 & 18.864 & -0.071 & 84230270492555679 & 18.935 & -0.223 & -0.279 & 167.38 & -139.86 & 218.12 & 70.3 & \nodata & \nodata  \\
  2505903071193331584 & 28.4648807 & -1.3965516 & 6.238 & 0.378 & 70.93 & -411.17 & 18.686 & 0.194 & 106320284648194992 & 18.721 & -0.024 & -0.114 & 158.56 & -274.57 & 317.06 & 100.0 &  DA  & 6, 9, 29  \\
  5017892205533257600 & 29.2639775 & -33.0111307 & 1.168 & 0.457 & 97.26 & -18.65 & 19.754 & -0.164 & \nodata & \nodata & \nodata & \nodata & -252.17 & -312.99 & 401.93 & 89.46 & \nodata & \nodata  \\
  2463291012727113216 & 29.9114872 & -8.212267 & 3.873 & 0.496 & 326.06 & -124.12 & 19.857 & 0.406 & \nodata & \nodata & \nodata & \nodata & -211.79 & -370.7 & 426.93 & 100.0 &  DA  & 17  \\
  2491046298280035584 & 30.9072034 & -4.9876942 & 5.603 & 0.105 & 159.75 & -180.35 & 16.231 & -0.363 & \nodata & \nodata & \nodata & \nodata & -5.96 & -203.73 & 203.82 & 83.81 &  DA  & 18, 29  \\
  5121541586135955456 & 31.3169848 & -24.3620272 & 1.392 & 0.417 & 73.61 & -57.44 & 19.45 & 0.308 & 78760313168325978 & 19.403 & -0.057 & -0.219 & -66.34 & -310.95 & 317.95 & 87.59 & \nodata & \nodata  \\
  4970281363483524864 & 33.6957282 & -33.0063941 & 4.046 & 0.098 & 47.55 & -164.1 & 17.252 & -0.382 & \nodata & \nodata & \nodata & \nodata & 87.17 & -180.15 & 200.13 & 51.16 & \nodata & \nodata  \\
  2493618021617765504 & 34.364321 & -2.5738253 & 2.617 & 0.304 & 26.23 & -171.63 & 18.72 & -0.299 & \nodata & \nodata & \nodata & \nodata & 166.3 & -266.85 & 314.43 & 99.92 & \nodata & \nodata  \\
  2489926613190469376 & 35.0990149 & -3.6777678 & 1.046 & 0.563 & 61.61 & -11.93 & 19.8 & 0.265 & 103580350987547230 & 19.874 & -0.230 & -0.134 & -176.6 & -222.79 & 284.29 & 63.74 &  DA+dM & 24  \\
  5118899906370680320 & 36.4594415 & -24.8214165 & 0.76 & 0.255 & 42.18 & -8.19 & 18.898 & -0.469 & \nodata & \nodata & \nodata & \nodata & -162.93 & -212.92 & 268.11 & 77.43 & \nodata & \nodata  \\
  2515538877566260224 & 37.1319392 & 4.0327821 & 1.715 & 0.392 & 80.19 & 19.13 & 19.089 & -0.228 & 112830371318299742 & 19.192 & -0.322 & -0.320 & -200.9 & -107.48 & 227.85 & 70.67 & \nodata & \nodata  \\
  5065611697758431360 & 42.05722 & -30.0243774 & 12.924 & 0.194 & 445.08 & 323.57 & 18.371 & 0.716 & \nodata & \nodata & \nodata & \nodata & -199.78 & -28.55 & 201.81 & 71.97 &  DC  & 6, 9, 29  \\
  2497775064628920832 & 42.1570995 & -0.5243219 & 3.117 & 0.508 & 186.26 & -257.42 & 19.197 & 0.244 & \nodata & \nodata & \nodata & \nodata & 47.25 & -480.85 & 483.17 & 99.98 &  DA  & 15, 23  \\
  8539322701389696 & 44.4781652 & 7.8504499 & 5.169 & 0.378 & 35.58 & -279.83 & 19.231 & 0.386 & 117420444781511246 & 19.233 & 0.063 & -0.046 & 147.82 & -212.24 & 258.64 & 99.91 & WD & 28  \\
  5185910261001126400 & 45.099867 & -4.4249488 & 7.623 & 0.526 & 288.19 & -303.84 & 19.718 & 0.928 & \nodata & \nodata & \nodata & \nodata & -8.48 & -260.24 & 260.38 & 99.94 &  DC  & 6, 9, 29  \\
  31484932074057600 & 47.5033025 & 16.5049969 & 4.442 & 0.15 & 219.26 & -177.56 & 17.511 & -0.215 & \nodata & \nodata & \nodata & \nodata & -42.24 & -298.1 & 301.08 & 100.0 &  DA  & 14, 29  \\
  5154878022776139264 & 47.6155253 & -15.0740166 & 4.805 & 0.389 & 217.31 & 16.69 & 19.447 & 0.459 & 89910476151841481 & 19.428 & 0.070 & -0.064 & -168.89 & -133.04 & 215.0 & 80.28 & \nodata & \nodata  \\
  5103559249557987200 & 48.432874 & -19.0483501 & 1.873 & 0.362 & 62.7 & -85.53 & 19.028 & -0.223 & 85140484327032461 & 19.149 & -0.321 & -0.318 & 33.16 & -266.34 & 268.4 & 90.67 & \nodata & \nodata  \\
  9509091953149568 & 50.4497427 & 6.4952236 & 2.366 & 0.433 & 29.05 & -99.86 & 19.153 & -0.021 & 115790504497194972 & 19.194 & -0.042 & -0.158 & 89.66 & -188.09 & 208.37 & 59.07 & \nodata & \nodata  \\
  57488549574450432 & 52.3064485 & 19.0209322 & 3.19 & 0.551 & 173.86 & -39.35 & 19.575 & 0.343 & 130820523061255716 & 19.582 & 0.059 & -0.058 & -150.8 & -217.75 & 264.87 & 91.66 & \nodata & \nodata  \\
  5164741020034099712 & 52.4259547 & -9.5209721 & 0.691 & 0.377 & -8.02 & -39.65 & 19.358 & -0.425 & 96570524259945293 & 19.492 & -0.330 & -0.353 & 223.84 & -164.11 & 277.56 & 68.54 & \nodata & \nodata  \\
  64177566000527744 & 54.8293599 & 20.8282104 & 1.39 & 0.818 & 62.02 & -8.19 & 20.205 & 0.337 & \nodata & \nodata & \nodata & \nodata & -137.77 & -162.96 & 213.39 & 51.82 & \nodata & \nodata  \\
  44582933060466560 & 56.3211873 & 17.8016484 & 5.481 & 0.082 & 234.24 & -178.25 & 16.644 & 0.453 & \nodata & \nodata & \nodata & \nodata & -49.08 & -249.79 & 254.56 & 100.0 &  DA  & 19  \\
  66837563803594880 & 56.6962898 & 24.9290903 & 25.209 & 0.3 & 520.94 & -1157.49 & 18.597 & 1.513 & 137910566960076155 & 18.555 & 1.151 & 0.442 & 74.42 & -226.77 & 238.67 & 100.0 &  DC  & 6, 9, 20, 29  \\
  3249527592789028096 & 57.2371574 & -3.7837177 & 8.377 & 0.516 & 420.94 & -185.94 & 19.315 & 0.7 & \nodata & \nodata & \nodata & \nodata & -108.13 & -236.88 & 260.39 & 99.99 & WD & 29  \\
  166283580171410816 & 65.1334682 & 31.1524246 & 1.278 & 0.27 & 20.78 & -51.56 & 18.736 & 0.001 & \nodata & \nodata & \nodata & \nodata & 65.99 & -195.26 & 206.11 & 56.36 & \nodata & \nodata  \\
  3204986338092948608 & 68.9093333 & -2.8090654 & 0.964 & 0.566 & 23.2 & -50.52 & 19.861 & -0.075 & 104620689093049617 & 19.928 & -0.164 & -0.233 & 73.28 & -263.39 & 273.39 & 67.78 & \nodata & \nodata  \\
  3410339960151512064 & 71.5576246 & 20.4543702 & 4.696 & 0.616 & 121.8 & -263.21 & 19.872 & 0.856 & \nodata & \nodata & \nodata & \nodata & 64.46 & -285.54 & 292.73 & 99.29 & \nodata & \nodata  \\
  3231765321744973056 & 73.2429985 & 1.4300819 & 3.285 & 0.44 & 77.1 & -122.4 & 19.58 & -0.047 & 109710732428966758 & 19.656 & -0.224 & -0.205 & 23.17 & -207.42 & 208.71 & 61.63 & \nodata & \nodata  \\
  190675794669351424 & 82.6000308 & 39.0594624 & 6.289 & 0.731 & 186.9 & -304.53 & 19.337 & 0.627 & \nodata & \nodata & \nodata & \nodata & -10.57 & -269.12 & 269.32 & 98.73 & \nodata & \nodata  \\
  190912640633346048 & 84.1201413 & 39.1805843 & 4.627 & 0.435 & 70.85 & -193.94 & 19.3 & 0.522 & \nodata & \nodata & \nodata & \nodata & -47.38 & -206.15 & 211.53 & 71.11 & \nodata & \nodata  \\
  3448038129354872320 & 84.3019834 & 32.2502903 & 5.197 & 0.097 & 220.23 & -353.85 & 16.872 & -0.087 & \nodata & \nodata & \nodata & \nodata & -3.86 & -380.11 & 380.13 & 100.0 &  DA3.0  & 3, 6, 29  \\
  3429296884940000000 & 86.2450545 & 26.0440558 & 27.681 & 0.102 & 999.63 & -1389.59 & 16.897 & 1.221 & 139250862446304059 & 16.788 & 0.799 & 0.176 & -21.57 & -292.33 & 293.12 & 100.0 &  DC  & 26, 29  \\
  3427482725113315200 & 87.4025294 & 23.4941338 & 19.252 & 0.173 & 1026.74 & -917.66 & 18.101 & 1.34 & \nodata & \nodata & \nodata & \nodata & -100.03 & -323.96 & 339.05 & 100.0 &  DC8  & 10, 28, 29  \\
  192454873200555392 & 89.7936386 & 42.81058 & 10.637 & 0.365 & -63.92 & -519.37 & 18.325 & 0.547 & \nodata & \nodata & \nodata & \nodata & -141.28 & -185.5 & 233.18 & 100.0 & WD & 29  \\
  993971057111978752 & 101.9966558 & 54.363101 & 1.194 & 0.935 & -27.01 & -53.2 & 20.411 & 0.26 & 173231019966816546 & 20.400 & -0.033 & -0.127 & -184.23 & -148.9 & 236.88 & 53.91 & \nodata & \nodata  \\
  888739097023718784 & 102.1352003 & 30.4441996 & 4.165 & 0.342 & 226.14 & -233.6 & 18.86 & 0.082 & \nodata & \nodata & \nodata & \nodata & 132.92 & -345.31 & 370.01 & 100.0 & WD & 29  \\
  3380349749709453184 & 103.6376576 & 23.5957407 & 4.327 & 0.45 & 128.32 & -167.34 & 19.677 & 0.877 & \nodata & \nodata & \nodata & \nodata & 59.55 & -223.2 & 231.0 & 89.65 & \nodata & \nodata  \\
  927666344130922240 & 116.4656264 & 47.5876319 & 1.202 & 0.716 & -34.38 & -46.41 & 19.632 & -0.084 & 165101164656245927 & 19.749 & -0.258 & -0.241 & -176.44 & -143.93 & 227.7 & 57.78 & \nodata & \nodata  \\
  1035077806847142144 & 122.8223388 & 57.4395936 & 1.927 & 0.388 & -28.65 & -79.43 & 19.464 & 0.112 & 176921228225108337 & 19.597 & -0.236 & -0.126 & -104.78 & -179.36 & 207.72 & 57.76 &  DA  & 27  \\
  1033437919613834624 & 123.2962828 & 56.0141669 & 2.35 & 0.654 & -71.48 & -86.68 & 19.964 & 0.386 & 175211232964577880 & 19.993 & 0.019 & -0.017 & -172.54 & -146.96 & 226.65 & 67.02 &  DA  & 27  \\
  935258884237774080 & 123.8100768 & 51.2197169 & 1.22 & 0.165 & -8.22 & -73.96 & 17.896 & -0.46 & \nodata & \nodata & \nodata & \nodata & -79.09 & -278.06 & 289.09 & 98.98 &  DA  & 14  \\
  709064710767864064 & 125.9964694 & 31.1977711 & 2.016 & 0.229 & -15.4 & -164.95 & 18.317 & -0.211 & \nodata & \nodata & \nodata & \nodata & -90.26 & -378.84 & 389.45 & 100.0 &  DA  & 15, 23  \\
  1042111726327205120 & 129.5914621 & 61.1698697 & 1.093 & 0.58 & -49.75 & -68.61 & 19.718 & 0.339 & 181401295914424613 & 19.815 & -0.151 & -0.036 & -245.21 & -273.52 & 367.35 & 70.97 & \nodata & \nodata  \\
  1015135144116717056 & 131.5985691 & 49.4255583 & 4.366 & 0.303 & 125.88 & -290.53 & 18.607 & 0.164 & 167311315985201581 & 18.654 & 0.037 & -0.120 & 112.65 & -324.73 & 343.72 & 100.0 &  DA  & 6, 12, 29  \\
  1017098214752414080 & 131.9754051 & 51.6682878 & 1.8 & 0.585 & -51.25 & -77.35 & 20.028 & 0.106 & \nodata & \nodata & \nodata & \nodata & -149.09 & -193.62 & 244.37 & 71.0 & \nodata & \nodata  \\
  691072714808535168 & 132.0552944 & 26.0494745 & 2.121 & 0.153 & -14.23 & -122.38 & 17.638 & -0.475 & \nodata & \nodata & \nodata & \nodata & -51.28 & -270.52 & 275.34 & 100.0 & \nodata & \nodata  \\
  692791487703945216 & 132.8142344 & 27.2317241 & 2.174 & 0.516 & -21.15 & -90.01 & 19.639 & -0.063 & \nodata & \nodata & \nodata & \nodata & -58.19 & -192.97 & 201.56 & 51.01 &  DA  & 23  \\
  719649464394142848 & 134.3361475 & 38.6923285 & 0.667 & 0.563 & -20.36 & -39.58 & 19.761 & -0.366 & \nodata & \nodata & \nodata & \nodata & -156.53 & -274.82 & 316.27 & 65.13 & \nodata & \nodata  \\
  1039876144310811904 & 139.6075611 & 61.344293 & 1.07 & 0.885 & -5.95 & -48.17 & 20.453 & 0.141 & 181611396075783988 & 20.455 & -0.091 & -0.178 & -22.15 & -213.84 & 214.99 & 50.35 & \nodata & \nodata  \\
  792955416446330112 & 145.8327221 & 31.2076676 & 0.994 & 0.628 & -44.72 & -68.18 & 19.73 & -0.197 & 145441458328369902 & 19.830 & -0.282 & -0.229 & -182.5 & -343.46 & 388.93 & 77.64 &  DA  & 23  \\
  1021962763431473280 & 148.1982125 & 56.1225877 & 1.114 & 0.431 & -14.43 & -95.93 & 19.764 & -0.298 & 175341481982167932 & 19.886 & -0.350 & -0.357 & -11.27 & -412.61 & 412.76 & 90.54 & \nodata & \nodata  \\
  820465334812545664 & 149.3355298 & 45.1143175 & 1.418 & 0.549 & -60.16 & -50.65 & 19.765 & -0.063 & 162131493356217908 & 19.883 & -0.392 & -0.346 & -177.19 & -194.15 & 262.86 & 73.05 &  DA  & 15, 23  \\
  725998697368146560 & 155.1285184 & 24.5359904 & 0.99 & 0.55 & 12.32 & -40.6 & 19.518 & -0.346 & 137441551285813800 & 19.640 & -0.277 & -0.233 & 97.26 & -178.33 & 203.13 & 50.65 & \nodata & \nodata  \\
  1046115804078881792 & 150.3441293 & 57.0201056 & 2.267 & 0.401 & -33.74 & -148.17 & 19.54 & 0.054 & 176421503441424922 & 19.588 & -0.152 & -0.207 & -24.01 & -316.81 & 317.72 & 98.23 & \nodata & \nodata  \\
  795487694804510592 & 150.8879291 & 34.8284338 & 1.782 & 0.496 & -73.97 & -35.67 & 19.685 & -0.158 & 149791508879964792 & 19.750 & -0.208 & -0.213 & -180.42 & -123.16 & 218.44 & 61.71 &  DA  & 23  \\
  827523099951377152 & 150.9605521 & 52.4756244 & 3.472 & 0.356 & -9.8 & -188.29 & 19.193 & 0.013 & 170971509606071643 & 19.262 & -0.174 & -0.223 & 25.87 & -256.13 & 257.43 & 98.53 & \nodata & \nodata  \\
  822722632184545280 & 153.4817653 & 48.3924547 & 0.628 & 0.723 & 0.74 & -73.97 & 19.574 & -0.207 & 166071534817351700 & 19.689 & -0.316 & -0.323 & 105.49 & -548.41 & 558.47 & 59.4 & \nodata & \nodata  \\
  625572157145156992 & 154.8103951 & 20.5578115 & 1.145 & 0.551 & -63.0 & 3.08 & 19.384 & -0.087 & 132661548106699934 & 19.469 & -0.213 & -0.237 & -257.94 & -40.68 & 261.13 & 68.89 & \nodata & \nodata  \\
  755606896236956288 & 155.8308359 & 38.2838106 & 1.35 & 1.456 & 28.57 & -59.17 & 19.989 & 0.018 & 153941558308211323 & 20.002 & -0.099 & -0.272 & 140.48 & -182.92 & 230.64 & 51.21 & \nodata & \nodata  \\
  1047156629273322368 & 156.6072414 & 58.4686151 & 2.047 & 0.306 & 54.97 & -126.67 & 19.106 & -0.192 & 178161566071373277 & 19.243 & -0.323 & -0.234 & 189.48 & -257.59 & 319.77 & 99.35 &  DA  & 15, 23  \\
  724156676088852608 & 160.0286705 & 24.7077606 & 5.261 & 0.473 & -189.73 & -418.63 & 19.739 & 0.446 & \nodata & \nodata & \nodata & \nodata & -68.13 & -408.5 & 414.14 & 100.0 & WD & 29  \\
  750786572836058880 & 160.4007349 & 35.6627278 & 1.172 & 0.35 & -50.18 & -70.73 & 19.133 & 0.339 & 150791604008276043 & 19.320 & -0.173 & 0.165 & -123.73 & -328.29 & 350.83 & 84.88 &  DA+M3 & 25  \\
  855361055035055104 & 161.4890613 & 59.0746242 & 17.482 & 0.135 & -1019.19 & -1462.53 & 17.678 & 0.235 & \nodata & \nodata & \nodata & \nodata & -154.06 & -458.12 & 483.33 & 100.0 &  DQ8  & 15, 23, 28, 29, 30  \\
  856513235846126720 & 170.9731502 & 57.7081659 & 10.468 & 0.522 & -30.09 & -491.29 & 19.649 & 0.655 & \nodata & \nodata & \nodata & \nodata & 72.79 & -210.65 & 222.87 & 98.14 & \nodata & \nodata  \\
  772256044901728256 & 173.3203626 & 43.998066 & 3.278 & 0.449 & -261.34 & -178.34 & 19.652 & 0.297 & \nodata & \nodata & \nodata & \nodata & -248.45 & -384.22 & 457.55 & 100.0 & \nodata & \nodata  \\
  3918117008499710848 & 174.3595201 & 14.1703918 & 1.86 & 0.067 & -79.93 & -44.7 & 13.251 & -0.549 & \nodata & \nodata & \nodata & \nodata & -137.33 & -188.7 & 233.38 & 99.65 & sd0 & 1  \\
  3973203189590794240 & 176.0652842 & 17.483731 & 10.458 & 1.78 & -359.47 & -517.58 & 20.023 & 1.107 & 128981760655651389 & 19.930 & 0.544 & 0.218 & -47.37 & -281.65 & 285.61 & 95.95 & \nodata & \nodata  \\
  3924031105452305536 & 176.2192146 & 14.8003373 & 0.982 & 0.604 & -7.72 & -50.69 & 19.429 & -0.465 & 125761762192121041 & 19.559 & -0.328 & -0.346 & 72.39 & -236.53 & 247.36 & 61.84 & \nodata & \nodata  \\
  3975344419766455936 & 177.6876309 & 19.3151177 & 1.138 & 0.557 & -50.63 & -77.41 & 19.328 & -0.178 & 131171776877218797 & 19.452 & -0.316 & -0.315 & -48.83 & -382.05 & 385.16 & 83.79 &  DA  & 27  \\
  774327078135106304 & 179.4626918 & 47.0230625 & 1.061 & 0.47 & -32.47 & -92.88 & 19.778 & -0.36 & 164421794628008419 & 19.966 & -0.414 & -0.321 & 57.12 & -435.78 & 439.51 & 89.39 & \nodata & \nodata  \\
  4006538045682928640 & 181.1204245 & 26.2669237 & 0.943 & 0.362 & -41.14 & -37.73 & 19.388 & -0.381 & 139521811205440931 & 19.541 & -0.352 & -0.318 & -97.31 & -263.24 & 280.65 & 77.33 & \nodata & \nodata  \\
  4001632578850515584 & 183.8842936 & 23.2653236 & 2.048 & 0.655 & -85.9 & -69.67 & 20.049 & 0.359 & 135911838844689044 & 20.070 & -0.102 & -0.124 & -96.66 & -237.07 & 256.02 & 75.36 &  DA  & 23  \\
  4016302739729712384 & 184.5585635 & 32.6403352 & 1.137 & 0.691 & -50.35 & -0.53 & 20.029 & -0.035 & \nodata & \nodata & \nodata & \nodata & -182.75 & -103.25 & 209.9 & 52.56 & \nodata & \nodata  \\
  3953838796960779520 & 186.0147514 & 23.5007908 & 1.592 & 0.328 & -46.76 & -52.15 & 18.965 & -0.183 & 136201860148701581 & 19.104 & -0.314 & -0.292 & -43.61 & -204.0 & 208.61 & 58.02 & \nodata & \nodata  \\
  4009114308801622656 & 186.6212886 & 27.4169465 & 3.831 & 0.965 & -186.75 & -18.32 & 20.049 & 0.329 & \nodata & \nodata & \nodata & \nodata & -188.84 & -135.01 & 232.14 & 70.74 & \nodata & \nodata  \\
  1544331701176666624 & 189.3688143 & 49.2173279 & 0.855 & 0.233 & -97.8 & -18.38 & 18.908 & -0.225 & 167061893689781562 & 19.044 & -0.321 & -0.294 & -399.79 & -380.24 & 551.74 & 99.0 &  DA  & 15  \\
  1514835411975910400 & 189.5237076 & 33.4232191 & 0.84 & 0.56 & -57.79 & -36.0 & 19.593 & -0.401 & 148101895238348589 & 19.780 & -0.415 & -0.365 & -172.35 & -343.55 & 384.35 & 75.43 &  DA  & 23  \\
  4012334052509346432 & 189.6158653 & 31.3605759 & 1.216 & 0.171 & -2.65 & -95.6 & 18.009 & -0.529 & \nodata & \nodata & \nodata & \nodata & 185.46 & -323.3 & 372.72 & 99.93 &  DA1  & 6, 23  \\
  3955090973201064320 & 191.7671317 & 22.0651585 & 2.558 & 0.725 & -13.77 & -140.27 & 20.261 & 0.58 & 134471917671659023 & 20.219 & 0.123 & -0.055 & 118.38 & -232.82 & 261.19 & 79.18 & \nodata & \nodata  \\
  3956102730057143936 & 191.9601139 & 23.5481647 & 2.275 & 0.39 & -75.98 & -65.71 & 18.925 & -0.252 & \nodata & \nodata & \nodata & \nodata & -59.65 & -200.61 & 209.29 & 61.16 &  DA  & 21, 23  \\
  3930746961129383552 & 192.8438331 & 14.4131577 & 1.602 & 0.529 & -28.74 & -80.98 & 19.788 & -0.377 & \nodata & \nodata & \nodata & \nodata & 61.68 & -246.72 & 254.31 & 74.03 & \nodata & \nodata  \\
  3691884137373037056 & 195.5027552 & 1.771876 & 3.457 & 0.287 & -145.31 & -50.31 & 18.465 & -0.06 & 110121955029776736 & 18.535 & -0.201 & -0.262 & -119.1 & -173.94 & 210.81 & 73.29 &  DA  & 11, 16, 21  \\
  1467533871993501568 & 195.8929762 & 33.6453371 & 2.737 & 0.521 & -3.88 & -145.15 & 20.069 & 0.076 & 148371958930035104 & 20.106 & -0.111 & -0.177 & 137.06 & -210.88 & 251.51 & 86.04 & \nodata & \nodata  \\
  1516252854263114368 & 195.9896475 & 35.8453465 & 1.37 & 0.421 & -47.01 & -61.36 & 19.81 & 0.246 & 151011959897205018 & 19.893 & -0.172 & -0.078 & -12.53 & -267.16 & 267.45 & 79.79 &  DA  & 25  \\
  1466187726163751808 & 197.3994017 & 31.7234213 & 1.402 & 0.828 & -106.93 & -10.14 & 20.476 & -0.282 & \nodata & \nodata & \nodata & \nodata & -275.94 & -236.04 & 363.12 & 77.73 & \nodata & \nodata  \\
  1524064854313478528 & 197.4533856 & 39.7682908 & 3.375 & 0.385 & -151.6 & -87.74 & 19.392 & -0.03 & 155721974537472683 & 19.449 & -0.193 & -0.193 & -100.14 & -224.72 & 246.02 & 94.74 & \nodata & \nodata  \\
  1446075596907317504 & 198.9902181 & 23.8339273 & 0.521 & 0.698 & -50.22 & 19.69 & 20.001 & -0.302 & \nodata & \nodata & \nodata & \nodata & -476.04 & -119.93 & 490.91 & 57.46 & \nodata & \nodata  \\
  3938433024147961984 & 199.6909134 & 17.5752818 & 4.121 & 0.748 & -174.33 & 69.4 & 20.429 & 0.721 & 129091996909820743 & 20.378 & 0.213 & 0.156 & -209.2 & -53.07 & 215.82 & 65.02 & \nodata & \nodata  \\
  3939302875285035264 & 200.5162549 & 19.5397297 & 0.814 & 0.806 & -53.78 & -3.33 & 20.367 & 0.208 & 131442005162618208 & 20.412 & -0.147 & -0.189 & -241.24 & -200.41 & 313.62 & 51.27 &  DA  & 23  \\
  1462483785023662080 & 200.8542533 & 30.6020308 & 6.246 & 0.368 & -103.33 & -406.34 & 19.45 & 0.598 & 144722008543973437 & 19.443 & 0.217 & 0.082 & 120.77 & -294.39 & 318.2 & 100.0 &  DA  & 14, 29  \\
  1448197035873529728 & 201.8006693 & 25.5505438 & 1.557 & 0.699 & -90.69 & -95.24 & 20.195 & 0.231 & 138662018008351406 & 20.237 & -0.116 & -0.168 & -48.16 & -397.57 & 400.48 & 86.98 & \nodata & \nodata  \\
  1470295123647580928 & 202.7038358 & 34.5323097 & 1.566 & 0.62 & -93.3 & -7.23 & 20.053 & 0.051 & 149432027040299457 & 20.108 & -0.154 & -0.175 & -209.95 & -190.21 & 283.29 & 77.68 & \nodata & \nodata  \\
  3717938993833933952 & 202.7268196 & 5.8686366 & 0.569 & 0.617 & -35.23 & -66.51 & 20.051 & -0.257 & \nodata & \nodata & \nodata & \nodata & 108.91 & -617.92 & 627.45 & 65.66 &  DA  & 15  \\
  3739105687884871936 & 203.9126141 & 13.021542 & 1.114 & 0.611 & 11.67 & -62.85 & 19.849 & -0.051 & 123622039126576477 & 19.899 & -0.151 & -0.209 & 202.44 & -181.72 & 272.04 & 68.88 & \nodata & \nodata  \\
  1456650699743018112 & 204.4348639 & 30.9001064 & 1.298 & 0.742 & -65.53 & -50.42 & 20.432 & -0.076 & \nodata & \nodata & \nodata & \nodata & -74.76 & -292.53 & 301.93 & 72.53 & \nodata & \nodata  \\
  1475765297075317376 & 204.6783659 & 39.1677497 & 1.119 & 0.363 & -46.98 & -12.46 & 19.727 & -0.262 & 155002046784741940 & 19.888 & -0.404 & -0.372 & -120.46 & -166.88 & 205.81 & 53.39 & \nodata & \nodata  \\
  1475692557509061504 & 204.8198163 & 38.7463039 & 0.644 & 0.589 & 10.69 & -57.84 & 20.314 & -0.106 & \nodata & \nodata & \nodata & \nodata & 330.66 & -279.61 & 433.03 & 67.15 & \nodata & \nodata  \\
  1470682632777169664 & 206.2637377 & 34.5279347 & 1.419 & 0.379 & -148.41 & -9.59 & 19.416 & -0.128 & 149432062640014154 & 19.547 & -0.315 & -0.288 & -363.33 & -338.58 & 496.63 & 98.61 & \nodata & \nodata  \\
  1499877243475417472 & 206.4661464 & 40.0169129 & 2.652 & 0.217 & -192.41 & -52.84 & 18.81 & -0.254 & 156022064665320988 & 18.944 & -0.329 & -0.292 & -201.2 & -294.55 & 356.7 & 100.0 &  DA  & 15, 21, 23, 29  \\
  3740444171496345600 & 206.496922 & 13.3617928 & 2.16 & 0.485 & -66.56 & -107.86 & 19.638 & 0.033 & 124032064970454818 & 19.711 & -0.176 & -0.182 & 32.11 & -276.32 & 278.18 & 89.25 &  DA  & 23  \\
  3723311237711768704 & 212.0567488 & 10.3950997 & 2.007 & 0.608 & -60.12 & -65.75 & 19.829 & 0.066 & 120472120568524736 & 19.894 & -0.206 & -0.240 & -9.75 & -210.18 & 210.4 & 56.64 & \nodata & \nodata  \\
  1232053429473003008 & 213.474397 & 15.5055831 & 6.808 & 0.075 & -292.26 & -39.15 & 16.351 & -0.137 & 126602134748187275 & 16.478 & -0.261 & -0.244 & -138.11 & -151.92 & 205.32 & 99.18 &  DA3.1  & 2, 6, 29  \\
  1253805652121019264 & 213.9284469 & 22.9458078 & 5.614 & 0.082 & -248.78 & -8.44 & 16.482 & -0.339 & 135532139289035494 & 16.651 & -0.359 & -0.333 & -154.71 & -142.26 & 210.18 & 99.95 &  DA2.1  & 6, 25, 29  \\
  3642680992030225536 & 214.4014566 & -4.575036 & 1.646 & 0.066 & -53.19 & -69.84 & 13.711 & -0.497 & \nodata & \nodata & \nodata & \nodata & 18.23 & -252.13 & 252.79 & 96.2 & sdB0 & 5  \\
  1255467628370145152 & 214.6178479 & 23.8899261 & 1.174 & 0.304 & -3.59 & -93.9 & 19.192 & -0.212 & 136662146178768671 & 19.309 & -0.275 & -0.249 & 237.44 & -295.75 & 379.27 & 96.19 & \nodata & \nodata  \\
  1238850537341400448 & 215.6844415 & 18.0568866 & 2.358 & 0.903 & -127.27 & -53.82 & 20.255 & 0.127 & 129662156846368908 & 20.201 & 0.103 & -0.114 & -123.27 & -248.97 & 277.82 & 77.29 & \nodata & \nodata  \\
  1239767667477407232 & 216.1414352 & 19.1094498 & 4.193 & 0.177 & -22.55 & -231.09 & 17.971 & -0.136 & 130932161414542260 & 18.070 & -0.254 & -0.301 & 151.87 & -214.1 & 262.49 & 100.0 &  DA  & 29  \\
  1177138458662659456 & 216.7080068 & 9.8257088 & 3.896 & 0.23 & 46.59 & -315.66 & 18.048 & -0.096 & 119792167081821529 & 18.167 & -0.302 & -0.281 & 293.37 & -254.25 & 388.21 & 100.0 &  WD  & 16, 29  \\
  6331284305478534912 & 217.5333204 & -7.0088351 & 1.471 & 0.499 & -70.31 & -4.63 & 19.744 & -0.089 & 99582175334839934 & 19.797 & -0.241 & -0.275 & -158.46 & -162.63 & 227.07 & 63.28 & \nodata & \nodata  \\
  1283728238299906688 & 217.6356302 & 28.6530704 & 2.283 & 0.662 & -10.57 & -117.07 & 20.105 & 0.096 & 142382176356364371 & 20.106 & -0.097 & -0.099 & 148.16 & -193.97 & 244.08 & 73.53 & \nodata & \nodata  \\
  1279378535941191040 & 218.2309704 & 25.7083681 & 0.71 & 0.73 & -28.03 & -33.24 & 20.184 & -0.196 & \nodata & \nodata & \nodata & \nodata & 10.52 & -290.22 & 290.41 & 57.88 & \nodata & \nodata  \\
  3656408154184836096 & 219.962521 & 3.0345658 & 1.708 & 0.846 & 47.93 & -63.63 & 20.482 & 0.498 & 111642199625002062 & 20.480 & 0.051 & 0.013 & 216.41 & -45.09 & 221.06 & 56.26 & \nodata & \nodata  \\
  3654933197991146496 & 220.2565704 & 1.5361987 & 3.88 & 0.457 & -287.76 & -50.91 & 18.845 & 0.103 & 109842202570044012 & 18.904 & -0.107 & -0.138 & -222.91 & -278.84 & 356.98 & 99.99 & WD & 29  \\
  1241636356209099264 & 220.523901 & 22.0566522 & 3.735 & 0.396 & 24.75 & -377.87 & 19.7 & 0.431 & 134462205238918815 & 19.693 & 0.089 & 0.011 & 345.87 & -333.62 & 480.55 & 100.0 & WD & 29  \\
  1186055424948978560 & 220.9280067 & 15.1605983 & 1.187 & 0.239 & -33.66 & -51.08 & 18.681 & 0.252 & 126192209280613293 & 18.716 & -0.058 & -0.096 & 35.01 & -241.71 & 244.23 & 80.57 &  DA  & 22  \\
  1282137691651169920 & 222.6607956 & 29.5998465 & 1.823 & 0.204 & 55.15 & -60.49 & 18.261 & -0.389 & 143522226607210512 & 18.441 & -0.386 & -0.329 & 212.47 & -12.69 & 212.84 & 70.48 &  DA  & 21, 25  \\
  1161215296909017728 & 222.7021984 & 7.557479 & 13.327 & 0.06 & -813.59 & -447.93 & 15.533 & -0.158 & \nodata & \nodata & \nodata & \nodata & -111.22 & -311.04 & 330.32 & 100.0 &  DA3.4  & 2, 6, 21, 29  \\
  3651160395639327488 & 223.5624269 & 0.2098465 & 3.484 & 0.611 & -166.45 & -81.63 & 20.096 & 0.366 & 108252235626882300 & 20.079 & -0.006 & -0.055 & -95.7 & -233.36 & 252.22 & 88.06 & \nodata & \nodata  \\
  6326108938606028032 & 224.0744952 & -9.4637709 & 3.042 & 0.286 & -47.93 & -122.37 & 18.89 & -0.038 & 96642240745414253 & 18.959 & -0.191 & -0.275 & 73.04 & -191.3 & 204.77 & 59.31 & \nodata & \nodata  \\
  6313793343222810112 & 224.3027837 & -11.0039233 & 4.373 & 0.554 & -227.11 & -108.38 & 18.938 & 0.257 & 94792243031465871 & 18.991 & -0.057 & -0.094 & -102.31 & -252.85 & 272.76 & 98.11 & \nodata & \nodata  \\
  1266232053365039104 & 224.409065 & 24.3935356 & 3.662 & 0.232 & -85.7 & -219.04 & 18.7 & 0.067 & 137272244092752710 & 18.771 & -0.194 & -0.226 & 115.05 & -281.89 & 304.47 & 100.0 & WD & 29  \\
  6307069623461134208 & 224.4868033 & -15.6606096 & 2.485 & 0.467 & -106.78 & -10.41 & 19.266 & 0.181 & 89202244870077666 & 19.320 & -0.142 & -0.173 & -135.08 & -153.77 & 204.67 & 54.34 & \nodata & \nodata  \\
  1153170543991219968 & 225.8382804 & 1.3143092 & 2.758 & 0.501 & -86.22 & -106.27 & 19.696 & 0.121 & 109572258384057797 & 19.772 & -0.166 & -0.143 & 10.6 & -234.93 & 235.17 & 79.54 &  DA  & 15, 23  \\
  6308210469853539072 & 228.0698217 & -14.7036075 & 2.225 & 0.557 & -96.94 & 1.36 & 19.641 & 0.195 & 90352280699626062 & 19.739 & -0.175 & -0.155 & -153.91 & -137.65 & 206.49 & 54.72 & \nodata & \nodata  \\
  1212348119518459392 & 228.8783363 & 19.1892131 & 10.934 & 0.459 & 114.63 & -944.37 & 19.797 & 1.593 & \nodata & \nodata & \nodata & \nodata & 317.55 & -263.12 & 412.4 & 85.52 & WD & 29  \\
  1194122404323303808 & 234.8435532 & 13.8652582 & 4.883 & 0.271 & -202.75 & -80.95 & 18.873 & 0.218 & \nodata & \nodata & \nodata & \nodata & -90.12 & -191.79 & 211.9 & 84.37 &  DA  & 21  \\
  6261795862092948992 & 235.9367938 & -16.1402168 & 3.6 & 0.493 & 31.27 & -155.34 & 19.505 & 0.07 & 88632359368152345 & 19.588 & -0.156 & -0.193 & 166.47 & -125.77 & 208.64 & 62.03 & \nodata & \nodata  \\
  4423505221809872128 & 236.899271 & 2.6669119 & 1.68 & 0.331 & -114.06 & -57.88 & 19.121 & -0.226 & \nodata & \nodata & \nodata & \nodata & -132.61 & -335.68 & 360.93 & 98.94 & \nodata & \nodata  \\
  4450868905132679040 & 241.7013581 & 7.1423043 & 0.922 & 0.429 & -32.03 & 40.46 & 19.46 & -0.103 & \nodata & \nodata & \nodata & \nodata & -261.44 & 45.16 & 265.31 & 70.07 & \nodata & \nodata  \\
  6035937275903148672 & 243.0669162 & -31.7082961 & 3.456 & 0.755 & -55.93 & -227.82 & 20.013 & 0.209 & \nodata & \nodata & \nodata & \nodata & 149.48 & -284.94 & 321.77 & 95.73 & \nodata & \nodata  \\
  4355542861909368064 & 244.6827943 & -4.8560939 & 1.246 & 0.395 & -58.86 & -9.96 & 19.069 & -0.114 & \nodata & \nodata & \nodata & \nodata & -147.27 & -172.75 & 227.01 & 65.4 & \nodata & \nodata  \\
  4384045501835601280 & 249.381827 & 1.0087415 & 6.74 & 0.446 & -334.98 & -155.54 & 19.551 & 0.757 & 109212493819111001 & 19.544 & 0.298 & 0.090 & -110.9 & -234.87 & 259.74 & 99.97 & WD & 29  \\
  4384099206106094080 & 249.4731319 & 1.4651935 & 1.29 & 0.669 & -64.46 & -32.72 & 20.005 & 0.006 & \nodata & \nodata & \nodata & \nodata & -104.63 & -244.07 & 265.55 & 68.08 & \nodata & \nodata  \\
  4341016560965371136 & 253.2074978 & -6.409742 & 1.236 & 0.562 & 16.14 & -57.38 & 19.617 & 0.173 & 100302532075038780 & 19.656 & 0.013 & -0.082 & 183.88 & -135.71 & 228.53 & 59.86 & \nodata & \nodata  \\
  6702584369952885632 & 270.635694 & -51.8003263 & 3.584 & 0.351 & -149.41 & -103.2 & 19.393 & 0.042 & \nodata & \nodata & \nodata & \nodata & 99.29 & -218.69 & 240.17 & 95.48 & \nodata & \nodata  \\
  6728441550544174208 & 281.5824116 & -40.8408711 & 0.912 & 0.454 & -23.22 & -70.72 & 19.687 & -0.331 & \nodata & \nodata & \nodata & \nodata & -34.81 & -385.34 & 386.91 & 83.06 & \nodata & \nodata  \\
  6710600423900428800 & 284.2505549 & -46.456427 & 4.375 & 0.231 & 42.59 & -294.92 & 18.404 & -0.004 & \nodata & \nodata & \nodata & \nodata & -162.39 & -279.06 & 322.87 & 100.0 & WD & 29  \\
  6718839854799506432 & 286.7160344 & -38.1252051 & 2.421 & 0.562 & -29.7 & -116.98 & 19.653 & 0.06 & \nodata & \nodata & \nodata & \nodata & -24.52 & -235.0 & 236.28 & 75.12 & \nodata & \nodata  \\
  6640368259682514560 & 289.9194028 & -55.8473579 & 3.483 & 0.547 & -140.09 & -51.13 & 19.805 & 0.038 & \nodata & \nodata & \nodata & \nodata & 157.43 & -128.1 & 202.97 & 52.95 & \nodata & \nodata  \\
  6742841300283347456 & 290.4595237 & -35.5261567 & 2.973 & 0.299 & -79.29 & -116.79 & 19.145 & 0.215 & \nodata & \nodata & \nodata & \nodata & 62.96 & -216.05 & 225.04 & 86.08 & \nodata & \nodata  \\
  6646382657004702720 & 293.508518 & -51.3050803 & 1.226 & 0.505 & -34.64 & -50.71 & 19.833 & -0.245 & \nodata & \nodata & \nodata & \nodata & 73.29 & -225.81 & 237.4 & 63.94 & \nodata & \nodata  \\
  6688913592127235584 & 296.5952164 & -40.9780137 & 0.751 & 0.355 & -18.09 & -57.3 & 19.224 & -0.424 & \nodata & \nodata & \nodata & \nodata & 22.98 & -378.47 & 379.16 & 83.8 & \nodata & \nodata  \\
  6473497510236254720 & 304.2873909 & -52.9386643 & 1.137 & 0.437 & 36.02 & -42.5 & 19.401 & -0.179 & \nodata & \nodata & \nodata & \nodata & -176.68 & -150.63 & 232.17 & 63.38 & \nodata & \nodata  \\
  6847362353085471232 & 304.6173781 & -25.8123022 & 1.273 & 0.535 & -1.41 & -58.7 & 19.28 & -0.338 & \nodata & \nodata & \nodata & \nodata & -29.65 & -216.63 & 218.65 & 58.46 & \nodata & \nodata  \\
  6849354809891475840 & 305.0785991 & -23.8995449 & 3.109 & 0.286 & -5.88 & -198.57 & 18.683 & -0.077 & \nodata & \nodata & \nodata & \nodata & -38.19 & -300.41 & 302.83 & 99.99 & \nodata & \nodata  \\
  6472240566582813824 & 305.2054122 & -55.7141452 & 0.6 & 0.662 & -17.83 & -36.74 & 20.231 & -0.179 & \nodata & \nodata & \nodata & \nodata & 95.01 & -308.16 & 322.47 & 56.77 & \nodata & \nodata  \\
  6668526653683695488 & 305.7407496 & -47.9028547 & 1.048 & 1.004 & 54.94 & -58.23 & 19.939 & 0.279 & \nodata & \nodata & \nodata & \nodata & -283.41 & -225.34 & 362.08 & 55.19 & \nodata & \nodata  \\
  6474160932360048512 & 307.9775108 & -52.7321532 & 2.925 & 0.782 & -13.93 & -144.04 & 20.17 & 0.142 & \nodata & \nodata & \nodata & \nodata & -5.15 & -234.46 & 234.51 & 71.45 & \nodata & \nodata  \\
  6675662823451111808 & 308.4693906 & -44.8033369 & 2.938 & 0.446 & -90.09 & -111.36 & 19.494 & -0.095 & \nodata & \nodata & \nodata & \nodata & 124.64 & -194.6 & 231.09 & 81.95 & \nodata & \nodata  \\
  6676586000900194304 & 309.3667501 & -41.8758341 & 3.451 & 0.263 & -84.73 & -133.01 & 18.805 & -0.006 & \nodata & \nodata & \nodata & \nodata & 97.56 & -193.42 & 216.64 & 84.22 & \nodata & \nodata  \\
  6471523921227261056 & 310.6490287 & -52.3055697 & 11.782 & 0.605 & 399.8 & -828.77 & 19.342 & 0.944 & \nodata & \nodata & \nodata & \nodata & -189.14 & -318.23 & 370.2 & 100.0 & WD & 29  \\
  6778331684495099008 & 311.511981 & -36.7094078 & 1.259 & 0.461 & -21.12 & -50.69 & 19.294 & -0.494 & \nodata & \nodata & \nodata & \nodata & 64.89 & -196.27 & 206.72 & 53.7 & \nodata & \nodata  \\
  6471548355295635712 & 311.702894 & -52.29089 & 1.369 & 0.468 & -3.27 & -101.44 & 19.379 & -0.204 & \nodata & \nodata & \nodata & \nodata & -14.81 & -351.03 & 351.34 & 89.47 & \nodata & \nodata  \\
  6780090108529839104 & 312.5537325 & -33.4830149 & 3.063 & 0.405 & -4.42 & -129.78 & 19.11 & -0.031 & \nodata & \nodata & \nodata & \nodata & -5.99 & -200.83 & 200.92 & 51.82 & \nodata & \nodata  \\
  6677077521256040576 & 312.5753706 & -42.3186445 & 1.13 & 0.188 & 56.4 & -63.27 & 17.879 & -0.292 & \nodata & \nodata & \nodata & \nodata & -252.91 & -250.08 & 355.67 & 99.58 & \nodata & \nodata  \\
  6481265907778902784 & 312.9905118 & -49.3422424 & 5.741 & 0.504 & 12.21 & -277.14 & 19.73 & 0.491 & \nodata & \nodata & \nodata & \nodata & -23.48 & -227.83 & 229.04 & 92.59 & \nodata & \nodata  \\
  6775068295327939456 & 313.6613467 & -37.8061883 & 1.244 & 1.311 & -1.08 & -70.84 & 20.508 & -0.236 & \nodata & \nodata & \nodata & \nodata & -9.53 & -269.83 & 269.99 & 59.11 & \nodata & \nodata  \\
  6802352848169916800 & 315.5241614 & -25.8074881 & 1.409 & 0.995 & 97.98 & -101.99 & 19.459 & -0.287 & \nodata & \nodata & \nodata & \nodata & -339.65 & -333.02 & 475.68 & 79.13 & \nodata & \nodata  \\
  6777159394645734400 & 315.5625041 & -35.6192817 & 2.128 & 0.464 & 48.19 & -162.9 & 19.332 & -0.095 & \nodata & \nodata & \nodata & \nodata & -117.61 & -359.57 & 378.31 & 98.2 & \nodata & \nodata  \\
  6477280517431230208 & 316.7519426 & -50.133094 & 0.869 & 0.602 & 34.72 & -35.34 & 20.1 & -0.01 & \nodata & \nodata & \nodata & \nodata & -192.12 & -189.9 & 270.13 & 62.15 & \nodata & \nodata  \\
  6788894761422611968 & 318.4884572 & -27.9987785 & 7.97 & 1.067 & -88.25 & -382.22 & 19.926 & 1.0 & 74403184884972083 & 19.797 & 0.817 & 0.153 & 53.8 & -227.02 & 233.31 & 85.66 & \nodata & \nodata  \\
  6582157678859024896 & 321.2537187 & -40.7989106 & 0.9 & 0.8 & 45.31 & -76.58 & 19.844 & -0.309 & \nodata & \nodata & \nodata & \nodata & -223.2 & -411.95 & 468.53 & 72.03 & \nodata & \nodata  \\
  6562262252178327168 & 324.2155195 & -48.8445914 & 0.926 & 0.477 & 49.6 & -118.55 & 19.743 & 0.04 & \nodata & \nodata & \nodata & \nodata & -209.26 & -623.79 & 657.95 & 89.5 & \nodata & \nodata  \\
  6811507141465107200 & 324.964601 & -25.9087404 & 7.12 & 0.337 & -149.16 & -279.27 & 18.886 & 0.292 & 76913249646780023 & 18.888 & 0.082 & -0.083 & 114.5 & -176.97 & 210.79 & 86.49 & WD & 29  \\
  6592388973858801920 & 325.2245332 & -32.521488 & 0.339 & 0.278 & -18.57 & -48.31 & 18.476 & -0.461 & \nodata & \nodata & \nodata & \nodata & 316.13 & -651.6 & 724.24 & 62.19 & \nodata & \nodata  \\
  6461055367936763520 & 327.9826935 & -55.1717318 & 1.422 & 0.746 & 38.13 & -105.84 & 20.317 & -0.21 & \nodata & \nodata & \nodata & \nodata & -84.31 & -365.27 & 374.88 & 81.9 & \nodata & \nodata  \\
  6586613617235206400 & 328.8121726 & -37.7817771 & 0.894 & 1.056 & 40.08 & -37.67 & 20.047 & -0.042 & \nodata & \nodata & \nodata & \nodata & -185.89 & -224.71 & 291.63 & 53.16 & \nodata & \nodata  \\
  6574206865465848448 & 330.0903166 & -39.5956862 & 1.795 & 0.64 & -13.44 & -86.26 & 19.966 & -0.325 & \nodata & \nodata & \nodata & \nodata & 66.86 & -220.62 & 230.53 & 64.89 & \nodata & \nodata  \\
  6559969156253872000 & 331.5600066 & -49.0175104 & 3.135 & 0.541 & 84.09 & -149.86 & 19.824 & -0.038 & \nodata & \nodata & \nodata & \nodata & -89.9 & -243.79 & 259.83 & 90.8 & \nodata & \nodata  \\
  6570048615568960384 & 333.3023035 & -41.7350159 & 1.524 & 0.761 & 72.63 & -33.24 & 19.604 & -0.017 & \nodata & \nodata & \nodata & \nodata & -204.29 & -141.45 & 248.48 & 65.17 & \nodata & \nodata  \\
  6612065078034665344 & 333.6612904 & -32.9284686 & 1.163 & 0.416 & 27.54 & -44.08 & 19.412 & -0.301 & \nodata & \nodata & \nodata & \nodata & -77.85 & -196.98 & 211.8 & 55.73 & \nodata & \nodata  \\
  6508803687597976960 & 335.3442366 & -53.1998596 & 4.884 & 0.609 & -182.93 & -117.32 & 20.146 & 0.757 & \nodata & \nodata & \nodata & \nodata & 196.96 & -75.45 & 210.91 & 66.56 & \nodata & \nodata  \\
  6625456481120798464 & 335.7298794 & -25.1761704 & 1.961 & 0.142 & 77.23 & -34.38 & 17.369 & -0.434 & 77783357297868969 & 17.604 & -0.391 & -0.268 & -165.13 & -120.35 & 204.33 & 61.62 & \nodata & \nodata  \\
  6594541851985246336 & 336.7517563 & -39.2419091 & 3.257 & 0.433 & 130.25 & -122.26 & 19.269 & 0.011 & \nodata & \nodata & \nodata & \nodata & -147.17 & -214.35 & 260.01 & 95.95 & \nodata & \nodata  \\
  6593403445133539200 & 337.5001288 & -40.5071001 & 2.965 & 0.409 & 10.09 & -181.25 & 19.039 & -0.088 & \nodata & \nodata & \nodata & \nodata & 48.56 & -286.1 & 290.19 & 98.71 & \nodata & \nodata  \\
  6503646948000155008 & 340.345897 & -58.4791486 & 0.992 & 0.802 & 44.84 & -17.34 & 20.372 & -0.195 & \nodata & \nodata & \nodata & \nodata & -184.45 & -136.92 & 229.71 & 56.22 & \nodata & \nodata  \\
  6596361616743724160 & 342.5048969 & -35.0655668 & 1.109 & 0.645 & -15.39 & -45.99 & 19.71 & -0.249 & \nodata & \nodata & \nodata & \nodata & 117.52 & -170.76 & 207.29 & 52.73 & \nodata & \nodata  \\
  6546484019801301376 & 342.9999203 & -39.5780729 & 0.967 & 0.525 & 38.51 & -18.44 & 19.351 & -0.288 & \nodata & \nodata & \nodata & \nodata & -155.72 & -139.75 & 209.24 & 53.52 & \nodata & \nodata  \\
  6603211123213159424 & 343.3070457 & -32.8666902 & 1.337 & 0.152 & 70.9 & -12.8 & 17.786 & -0.528 & \nodata & \nodata & \nodata & \nodata & -228.02 & -115.3 & 255.51 & 97.35 & \nodata & \nodata  \\
  6556445663868161920 & 347.1207453 & -32.8041628 & 0.556 & 0.159 & -22.69 & -49.67 & 17.324 & -0.266 & \nodata & \nodata & \nodata & \nodata & 320.61 & -337.88 & 465.78 & 68.36 & \nodata & \nodata  \\
  2380152677943597184 & 351.5474011 & -27.2467869 & 8.254 & 0.49 & 576.75 & -99.91 & 19.78 & 0.87 & 75303515469824224 & 19.713 & 0.483 & 0.190 & -286.17 & -176.35 & 336.14 & 100.0 &  DC  & 6, 9, 29  \\
  6528896373537262208 & 351.5527623 & -44.9972477 & 0.966 & 0.813 & 58.98 & 15.51 & 20.303 & -0.316 & \nodata & \nodata & \nodata & \nodata & -296.86 & -36.64 & 299.12 & 65.01 & \nodata & \nodata  \\
  2387355338098699904 & 354.1610861 & -22.9333806 & 1.863 & 1.092 & -70.61 & -86.4 & 19.919 & 0.159 & 80483541611700371 & 19.930 & -0.047 & -0.108 & 252.61 & -129.41 & 283.83 & 69.53 & \nodata & \nodata  \\
  2393833248293162112 & 355.2416184 & -18.3731707 & 1.238 & 0.637 & 40.64 & -49.82 & 19.048 & -0.081 & 85953552415622582 & 19.144 & -0.263 & -0.241 & -61.79 & -238.38 & 246.25 & 63.86 & \nodata & \nodata  \\
  6524709055304694400 & 355.6467509 & -48.5838391 & 0.925 & 1.073 & 57.47 & 8.59 & 20.354 & 0.057 & \nodata & \nodata & \nodata & \nodata & -286.2 & -82.36 & 297.82 & 53.25 & \nodata & \nodata  \\
  2314173669516064640 & 358.6482487 & -32.355649 & 9.131 & 0.137 & 439.31 & -46.65 & 17.096 & 0.086 & \nodata & \nodata & \nodata & \nodata & -195.04 & -120.61 & 229.32 & 100.0 & WD & 6, 9, 29  \\
\enddata
\tablerefs{1. \citet{feige:58}; 2. \citet{eggen:65}; 3. \citet{greenstein:76}; 4. \citet{eggen:78}; 5. \citet{green:86}; 6. \citet{mccook:99}; 7. \citet{croom:01}; 8. \citet{koester:01}; 9. \citet{oppenheimer:01}; 10. \citet{lepine:03};  11. \citet{croom:04}; 12. \citet{kleinman:04}; 13. \citet{salim:04}; 14. \citet{carollo:06}; 15. \citet{eisenstein:06}; 16. \citet{harris:06}; 17. \citet{kilic:06}; 18. \citet{pauli:06}; 19. \citet{kawka:09}; 20. \citet{kilic:10}; 21. \citet{girven:11}; 22. \citet{brown:12}; 23. \citet{kleinman:13}; 24. \citet{li:14}; 25. \citet{kepler:15}; 26. \citet{limoges:15}; 27. \citet{kepler:16}; 28. \citet{leggett:18}; 29. \citet{kilic:19}; 30. \citet{kawka:20}}
\end{deluxetable*}
\end{longrotatetable}


==> tab3_setb.tex <==
\begin{longrotatetable}
\begin{deluxetable*}{lcccccccclccccccccccc}
\tablecolumns{21}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecaption{High-velocity White Dwarf Candidates in Set B \label{tab:tab4}}
\tablehead {
   \colhead{} &
   \colhead{RA} &
   \colhead{Dec} &
   \colhead{$\pi$} &
   \colhead{$\sigma_{\pi}$} &
   \colhead{$\mu_{\alpha}$} &
   \colhead{$\mu_{\delta}$} &
   \colhead{$G$} &
   \colhead{} &
   \colhead{} &
   \colhead{$r_{\rm PS}$} &
   \colhead{} &
   \colhead{} &
   \colhead{$v_{T, \, r}$} &
   \colhead{$v_{T, \, s}$} &
   \colhead{$v_{T, \, {\rm tot}}$} &
   \colhead{Phot\_Dist} &
   \colhead{$v_{T, \, {\rm phot}}$} &
   \colhead{Halo WD} &
   \colhead{} &
   \colhead{}   \\
   \colhead{source\_id} &
   \colhead{(deg)} &
   \colhead{(deg)} & 
   \colhead{(mas)} &
   \colhead{(mas)} &
   \colhead{(mas yr$^{-1}$)} &
   \colhead{(mas yr$^{-1}$)} &
   \colhead{(mag)} &
   \colhead{$\bpmrp$} &
   \colhead{PS1\_ID} &
   \colhead{(mag)} &
   \colhead{$g_{\rm PS}\, \, -\, \, r_{\rm PS}$} &
   \colhead{$r_{\rm PS}\, \, -\, \, i_{\rm PS}$} &
   \colhead{(km s$^{-1}$)} &
   \colhead{(km s$^{-1}$)} &
   \colhead{(km s$^{-1}$)} &
   \colhead{(pc)} &
   \colhead{(km s$^{-1}$)} &
   \colhead{Likelihood (\%)} &
   \colhead{Spec\_Type} &
   \colhead{Ref.}
}
\decimals
\startdata 
  2336547386815432960 & 0.4013693 & -24.9199278 & 0.963 & 0.637 & 31.73 & -33.85 & 19.765 & -0.375 & 78090004012856447 & 19.966 & -0.424 & -0.401 & -63.93 & -219.22 & 228.35 & 761.06 & 167.37 & 57.66 & \nodata & \nodata  \\
  2332903880159372672 & 0.4568686 & -29.4269526 & 1.559 & 1.767 & -33.61 & -165.65 & 20.646 & 0.506 & \nodata & \nodata & \nodata & \nodata & 317.77 & -404.01 & 514.01 & 309.78 & 248.19 & 56.85 & \nodata & \nodata  \\
  2417396645764338688 & 0.8341101 & -15.153369 & 5.562 & 1.282 & 99.12 & -242.25 & 20.637 & 0.517 & 89810008340536470 & 20.562 & 0.405 & 0.241 & 22.51 & -221.94 & 223.08 & 303.91 & 377.05 & 66.71 & \nodata & \nodata  \\
  4976547514607879808 & 1.6097728 & -50.158799 & 1.021 & 0.781 & -14.99 & -60.18 & 20.301 & 0.291 & \nodata & \nodata & \nodata & \nodata & 194.0 & -212.57 & 287.79 & 348.34 & 102.4 & 57.97 & \nodata & \nodata  \\
  2417119358380854656 & 2.8410856 & -14.4837046 & 1.633 & 0.654 & 64.74 & -76.99 & 20.046 & -0.255 & \nodata & \nodata & \nodata & \nodata & -55.35 & -286.71 & 292.01 & 612.92 & 292.24 & 78.09 & \nodata & \nodata  \\
  4972559104898070400 & 3.6737048 & -52.4593757 & 0.568 & 0.927 & 88.37 & -52.78 & 20.622 & -0.184 & \nodata & \nodata & \nodata & \nodata & -418.58 & -750.54 & 859.37 & 699.61 & 341.34 & 54.97 & \nodata & \nodata  \\
  2428459412072468480 & 4.2631784 & -9.0433806 & 1.367 & 0.929 & 72.84 & 7.76 & 20.411 & 0.319 & 97140042630878399 & 20.375 & 0.008 & -0.136 & -230.99 & -105.69 & 254.02 & 353.69 & 122.8 & 58.2 & \nodata & \nodata  \\
  2335876306765946496 & 5.1596328 & -24.6330851 & 0.717 & 0.898 & 89.58 & -84.65 & 20.01 & 0.047 & 78440051595830786 & 19.789 & -0.123 & -0.201 & -242.0 & -777.58 & 814.37 & 408.38 & 238.57 & 56.73 & \nodata & \nodata  \\
  2318593912418008448 & 6.1149599 & -29.9855662 & 5.942 & 1.103 & 166.63 & -264.12 & 20.535 & 1.219 & \nodata & \nodata & \nodata & \nodata & -11.21 & -248.84 & 249.1 & 128.68 & 190.48 & 82.26 & \nodata & \nodata  \\
  2347566902802721408 & 7.4949079 & -25.0774151 & 9.354 & 1.329 & 411.14 & -331.71 & 20.713 & 1.02 & \nodata & \nodata & \nodata & \nodata & -94.39 & -250.5 & 267.7 & 174.84 & 437.81 & 96.34 & \nodata & \nodata  \\
  2348187778980328960 & 8.2369737 & -23.7491399 & 1.594 & 1.125 & 57.81 & -57.96 & 19.965 & -0.153 & 79500082370811366 & 20.209 & -0.493 & -0.081 & -59.1 & -236.06 & 243.34 & 497.08 & 192.87 & 59.79 & \nodata & \nodata  \\
  4925179671389315968 & 9.0130541 & -52.3218674 & 1.556 & 0.395 & 75.26 & -126.93 & 19.859 & 0.012 & \nodata & \nodata & \nodata & \nodata & 20.41 & -449.07 & 449.53 & 396.14 & 277.07 & 98.56 & \nodata & \nodata  \\
  4980421295935512960 & 9.2831159 & -44.7925575 & 1.088 & 1.184 & 83.08 & 23.53 & 20.871 & 0.184 & \nodata & \nodata & \nodata & \nodata & -360.78 & -106.22 & 376.1 & 517.39 & 211.77 & 59.52 & \nodata & \nodata  \\
  2376901181542193024 & 9.7267676 & -12.34503 & 0.767 & 0.774 & -26.07 & -45.51 & 19.939 & -0.33 & 93180097268016461 & 20.102 & -0.377 & -0.327 & 287.0 & -150.36 & 324.0 & 713.48 & 177.38 & 61.46 & \nodata & \nodata  \\
  4975029359632752256 & 11.9325356 & -47.9292365 & 1.749 & 0.575 & 74.34 & -12.14 & 20.191 & 0.36 & \nodata & \nodata & \nodata & \nodata & -148.2 & -140.46 & 204.18 & 303.5 & 108.36 & 52.51 & \nodata & \nodata  \\
  2376316486169368192 & 12.2342641 & -12.4113292 & 2.129 & 0.823 & 1.33 & -96.76 & 20.313 & 0.372 & 93100122342796964 & 20.331 & -0.063 & -0.112 & 116.6 & -181.12 & 215.4 & 315.83 & 144.87 & 57.05 & \nodata & \nodata  \\
  4986832002777333632 & 13.0609507 & -41.9191941 & 1.356 & 0.87 & 77.34 & 11.64 & 20.539 & 0.149 & \nodata & \nodata & \nodata & \nodata & -247.03 & -117.11 & 273.39 & 463.02 & 171.65 & 65.64 & \nodata & \nodata  \\
  2373253178054574464 & 13.2416503 & -12.7930335 & 1.497 & 0.691 & 108.41 & 14.36 & 19.701 & 0.539 & 92640132414798805 & 19.550 & -0.075 & 0.075 & -310.24 & -153.81 & 346.28 & 192.02 & 99.53 & 70.09 & \nodata & \nodata  \\
  4986280009284690432 & 15.6552863 & -41.8326656 & 1.062 & 1.258 & 49.44 & 16.93 & 20.968 & -0.166 & \nodata & \nodata & \nodata & \nodata & -223.72 & -65.74 & 233.18 & 801.96 & 198.66 & 52.83 & \nodata & \nodata  \\
  4987831802442860928 & 16.3912226 & -40.9366725 & 1.902 & 0.427 & -21.79 & -148.7 & 19.764 & -0.284 & \nodata & \nodata & \nodata & \nodata & 259.63 & -270.02 & 374.59 & 577.95 & 411.72 & 98.07 & \nodata & \nodata  \\
  2476497904018183936 & 16.7200218 & -6.6111968 & 3.025 & 0.805 & -94.41 & -131.87 & 20.267 & 0.231 & 100060167199867143 & 20.271 & 0.030 & -0.044 & 241.18 & -80.18 & 254.16 & 369.78 & 284.26 & 78.74 & \nodata & \nodata  \\
  5028171681475540736 & 17.2323774 & -30.7639274 & 2.205 & 0.704 & 14.02 & -92.67 & 20.245 & 0.044 & \nodata & \nodata & \nodata & \nodata & 89.55 & -180.44 & 201.44 & 456.58 & 202.83 & 51.05 &  DA  & 5  \\
  4984884900827506816 & 17.9430772 & -40.7531641 & 2.502 & 0.909 & 85.13 & -80.29 & 20.689 & 0.402 & \nodata & \nodata & \nodata & \nodata & -39.91 & -218.06 & 221.69 & 361.49 & 200.51 & 61.06 & \nodata & \nodata  \\
  5027059525463879424 & 18.3671131 & -32.1657249 & 3.525 & 0.687 & 145.55 & -96.13 & 19.991 & 1.051 & \nodata & \nodata & \nodata & \nodata & -83.92 & -219.03 & 234.56 & 121.06 & 100.09 & 55.33 & \nodata & \nodata  \\
  4985113156864388608 & 20.9236193 & -40.2175172 & 1.859 & 0.383 & 73.64 & -39.66 & 19.607 & -0.184 & \nodata & \nodata & \nodata & \nodata & -86.74 & -194.87 & 213.31 & 438.29 & 173.76 & 61.38 & \nodata & \nodata  \\
  2354116139518758272 & 21.13544 & -19.4312391 & 0.799 & 0.791 & 33.92 & -23.63 & 20.337 & -0.139 & \nodata & \nodata & \nodata & \nodata & -78.82 & -232.36 & 245.36 & 580.65 & 113.76 & 54.78 & \nodata & \nodata  \\
  2457014386176082688 & 21.6099434 & -13.6044436 & 8.961 & 2.15 & -10.05 & -427.28 & 20.878 & 1.141 & \nodata & \nodata & \nodata & \nodata & 139.69 & -177.74 & 226.06 & 164.48 & 333.21 & 68.3 & \nodata & \nodata  \\
  5015252419849345920 & 22.1515295 & -33.772098 & 1.65 & 0.814 & 78.53 & 20.1 & 20.483 & 0.269 & \nodata & \nodata & \nodata & \nodata & -214.28 & -91.21 & 232.89 & 389.57 & 149.68 & 60.89 & \nodata & \nodata  \\
  2458451993334234624 & 22.8894274 & -11.4340685 & 4.862 & 1.18 & -15.77 & -266.43 & 20.482 & 1.248 & 94270228894329557 & 20.447 & 0.126 & 0.031 & 169.9 & -197.1 & 260.22 & 121.67 & 153.93 & 63.54 & \nodata & \nodata  \\
  2451027270485080448 & 23.6114961 & -16.3791171 & 1.455 & 0.976 & 100.48 & 0.26 & 20.359 & 0.624 & 88340236113565376 & 20.299 & 0.098 & 0.054 & -260.84 & -197.81 & 327.37 & 234.15 & 111.52 & 55.86 & \nodata & \nodata  \\
  4959754463063099520 & 24.3112027 & -42.1417387 & 0.756 & 0.726 & 18.69 & -36.52 & 20.403 & 0.133 & \nodata & \nodata & \nodata & \nodata & 56.18 & -251.17 & 257.38 & 443.54 & 86.24 & 50.25 & \nodata & \nodata  \\
  2452515940508852096 & 24.4103249 & -15.9869399 & 1.254 & 0.769 & 57.98 & -81.36 & 20.226 & -0.564 & \nodata & \nodata & \nodata & \nodata & 13.95 & -377.25 & 377.5 & \nodata & \nodata & 77.85 & \nodata & \nodata  \\
  2481231228561342720 & 24.7701894 & -3.735437 & 0.736 & 0.669 & -1.06 & -45.6 & 19.817 & -0.452 & 103510247701747975 & 19.935 & -0.326 & -0.291 & 189.03 & -225.02 & 293.88 & \nodata & \nodata & 62.77 & \nodata & \nodata  \\
  5022836266941858560 & 24.9087809 & -29.9657926 & 4.803 & 0.679 & 181.3 & -284.69 & 20.332 & 0.805 & \nodata & \nodata & \nodata & \nodata & 33.1 & -331.47 & 333.12 & 187.49 & 299.96 & 99.68 & \nodata & \nodata  \\
  2454010550473264640 & 25.2289335 & -13.685883 & 1.059 & 0.863 & 9.97 & -64.71 & 20.445 & -0.066 & 91570252288577421 & 20.477 & -0.140 & -0.103 & 142.88 & -255.95 & 293.13 & 564.4 & 175.15 & 63.0 & \nodata & \nodata  \\
  2465225951328886400 & 25.5657929 & -8.7832764 & 10.749 & 1.43 & 565.2 & -151.79 & 20.543 & 1.032 & 97460255657380573 & 20.462 & 0.788 & 0.348 & -153.97 & -207.11 & 258.07 & 159.53 & 442.54 & 95.54 & \nodata & \nodata  \\
  2466501213017924096 & 29.7833524 & -7.2908292 & 3.077 & 0.421 & 20.58 & -149.03 & 19.172 & -0.363 & 99250297833521606 & 19.203 & -0.136 & -0.226 & 121.39 & -197.38 & 231.71 & 557.02 & 397.2 & 84.14 & \nodata & \nodata  \\
  5120667994082966016 & 30.5142352 & -26.7961767 & 4.047 & 0.853 & 85.61 & -163.37 & 20.513 & 0.712 & 75840305140175113 & 20.436 & 0.331 & 0.059 & 46.03 & -211.07 & 216.03 & 226.7 & 198.19 & 63.89 & \nodata & \nodata  \\
  2519862844481638528 & 33.4105109 & 5.5062391 & 1.844 & 0.891 & 3.95 & -94.39 & 20.149 & 0.254 & 114600334104698104 & 20.145 & 0.005 & -0.043 & 153.1 & -188.44 & 242.8 & 340.37 & 152.43 & 63.93 &  DAH  & 12 \\
  5117936218788726016 & 34.625926 & -26.1393684 & 3.32 & 0.9 & 52.75 & -284.18 & 20.218 & 0.221 & 76630346257823547 & 20.162 & 0.050 & -0.124 & 210.72 & -354.85 & 412.7 & 365.71 & 501.03 & 96.93 & \nodata & \nodata  \\
  5145369377501372928 & 36.5822448 & -16.7641994 & 8.586 & 0.754 & 180.53 & -336.24 & 20.419 & 1.409 & \nodata & \nodata & \nodata & \nodata & 46.08 & -205.58 & 210.68 & 99.19 & 179.44 & 67.49 & \nodata & \nodata  \\
  5063550937705248768 & 36.9261026 & -32.7191918 & 1.392 & 1.559 & 37.04 & -84.96 & 20.792 & 0.482 & \nodata & \nodata & \nodata & \nodata & 105.49 & -297.33 & 315.49 & 341.62 & 150.08 & 51.1 & \nodata & \nodata  \\
  5067646618518674432 & 37.8648464 & -29.1094663 & 0.997 & 0.977 & 26.34 & -84.47 & 20.825 & 0.216 & 73060378647239043 & 20.756 & -0.037 & -0.238 & 180.28 & -380.22 & 420.79 & 486.81 & 204.17 & 63.03 & \nodata & \nodata  \\
  5171053316288900736 & 39.6395718 & -12.1415285 & 0.991 & 0.736 & 57.33 & -6.96 & 20.292 & 0.388 & 93430396394390702 & 20.274 & -0.010 & -0.100 & -184.19 & -205.68 & 276.1 & 306.64 & 83.93 & 50.74 & \nodata & \nodata  \\
  5076687009280797184 & 40.8559879 & -25.7113798 & 1.599 & 0.774 & 66.91 & -41.95 & 20.495 & 0.073 & 77140408558426736 & 20.497 & -0.156 & -0.224 & -60.5 & -226.18 & 234.13 & 495.82 & 185.6 & 60.77 & \nodata & \nodata  \\
  5065484566341990272 & 40.9173033 & -30.5985143 & 0.867 & 0.862 & 40.82 & 25.29 & 20.399 & -0.008 & 71280409172471878 & 20.374 & -0.116 & -0.262 & -256.69 & -55.3 & 262.58 & 519.65 & 118.27 & 54.94 &  DA  & 5  \\
  2498627014341716992 & 41.676195 & 0.165755 & 1.597 & 0.73 & -16.64 & -66.26 & 20.284 & 0.33 & 108190416762249444 & 20.263 & 0.032 & 0.022 & 167.28 & -114.54 & 202.74 & 329.28 & 106.62 & 50.52 &  DA+M & 7  \\
  5129484251976187776 & 42.0363757 & -17.8318082 & 0.537 & 0.693 & 55.76 & 2.25 & 20.307 & -0.121 & 86600420362202174 & 20.344 & -0.209 & -0.276 & -378.71 & -315.22 & 492.73 & 561.89 & 148.64 & 55.56 & \nodata & \nodata  \\
  5072278173812317952 & 43.3537039 & -27.8441714 & 0.998 & 0.818 & 1.24 & -50.12 & 20.222 & -0.247 & 74580433537217401 & 20.327 & -0.320 & -0.256 & 161.15 & -175.25 & 238.08 & 651.83 & 154.89 & 57.0 &  DA  & 5  \\
  108405666040931840 & 44.7363511 & 20.549274 & 3.831 & 0.95 & 97.69 & -259.35 & 19.988 & 0.651 & \nodata & \nodata & \nodata & \nodata & 136.22 & -314.64 & 342.86 & 191.22 & 251.19 & 95.47 & \nodata & \nodata  \\
  5180450395495197184 & 44.8324488 & -7.2959466 & 2.142 & 1.048 & 137.15 & 5.76 & 20.563 & -0.062 & 99240448323765218 & 20.531 & -0.092 & -0.266 & -235.18 & -192.31 & 303.8 & 593.6 & 386.23 & 75.18 & \nodata & \nodata  \\
  58549647014319488 & 47.9429398 & 17.1081051 & 2.847 & 0.552 & 142.91 & -90.03 & 20.006 & 0.484 & 128530479427340395 & 20.000 & 0.174 & 0.003 & -71.93 & -271.87 & 281.22 & 237.38 & 190.05 & 93.39 & \nodata & \nodata  \\
  3262294292882537600 & 49.1801073 & -1.2598839 & 0.801 & 0.833 & 55.76 & -35.21 & 20.48 & -0.204 & \nodata & \nodata & \nodata & \nodata & -107.8 & -374.88 & 390.07 & 674.69 & 210.9 & 63.43 & \nodata & \nodata  \\
  12548726207846784 & 52.4240988 & 9.2634036 & 1.069 & 0.577 & 25.37 & -51.73 & 19.992 & 0.308 & 119110524239936665 & 19.996 & -0.034 & -0.121 & 68.35 & -246.25 & 255.56 & 295.72 & 80.76 & 58.82 & \nodata & \nodata  \\
  56491911002841472 & 54.3534401 & 18.1963693 & 2.817 & 0.392 & 40.4 & -124.83 & 19.145 & 0.298 & 129830543533736420 & 19.147 & -0.152 & -0.188 & 90.19 & -201.48 & 220.74 & 203.01 & 126.26 & 75.58 & \nodata & \nodata  \\
  3274818245718197888 & 54.7234187 & 4.6761181 & 2.237 & 0.684 & 34.51 & -118.8 & 20.254 & 0.158 & 113610547233622048 & 20.241 & -0.117 & -0.147 & 111.34 & -237.35 & 262.17 & 401.99 & 235.71 & 78.22 & \nodata & \nodata  \\
  3310153942390461056 & 64.635945 & 12.2847703 & 1.892 & 0.953 & 87.9 & -98.16 & 20.23 & 0.26 & 122740646357812269 & 20.199 & 0.042 & -0.039 & -12.99 & -329.8 & 330.06 & 350.56 & 218.95 & 78.19 & \nodata & \nodata  \\
  3305932019602628864 & 66.8309543 & 10.4553784 & 5.503 & 0.543 & 219.17 & -178.37 & 19.486 & 0.019 & \nodata & \nodata & \nodata & \nodata & -49.49 & -238.32 & 243.41 & 330.95 & 443.28 & 96.58 & \nodata & \nodata  \\
  3282755104763455360 & 71.1887206 & 5.8740543 & 0.971 & 0.803 & 48.42 & -71.85 & 20.145 & 0.481 & 115040711886029475 & 20.192 & 0.238 & 0.189 & 32.94 & -421.53 & 422.82 & 254.06 & 104.34 & 50.07 & \nodata & \nodata  \\
  204593520221297664 & 71.5869113 & 43.6268453 & 1.316 & 0.655 & 49.2 & -95.26 & 19.863 & 0.288 & \nodata & \nodata & \nodata & \nodata & 85.28 & -376.51 & 386.05 & 286.08 & 145.38 & 79.56 & \nodata & \nodata  \\
  3225945817152763520 & 72.0453805 & -2.2484777 & 2.613 & 1.525 & -17.19 & -113.5 & 20.679 & 0.574 & 105300720454292432 & 20.613 & 0.315 & 0.167 & 155.11 & -138.97 & 208.26 & 288.46 & 156.95 & 52.09 & \nodata & \nodata  \\
  187139868345707776 & 79.2651063 & 37.3658771 & 4.739 & 0.636 & 81.73 & -220.72 & 19.599 & 0.433 & \nodata & \nodata & \nodata & \nodata & 60.8 & -227.43 & 235.41 & 210.07 & 234.36 & 87.03 & \nodata & \nodata  \\
  3339036738463632640 & 82.5465994 & 10.6269427 & 6.605 & 0.909 & 168.74 & -239.48 & 20.271 & 1.279 & \nodata & \nodata & \nodata & \nodata & -3.29 & -210.22 & 210.25 & 106.67 & 148.12 & 62.86 & \nodata & \nodata  \\
  3404215714742563584 & 84.4960622 & 22.6291956 & 3.125 & 0.533 & 67.23 & -132.87 & 19.165 & 0.16 & \nodata & \nodata & \nodata & \nodata & 21.96 & -224.79 & 225.86 & 242.82 & 171.39 & 74.75 & \nodata & \nodata  \\
  191526855315318656 & 87.086324 & 39.741628 & 2.101 & 0.514 & 98.69 & -133.83 & 19.688 & 0.338 & \nodata & \nodata & \nodata & \nodata & 32.11 & -373.71 & 375.09 & 247.6 & 195.15 & 96.66 & \nodata & \nodata  \\
  3429403778085842432 & 87.3965174 & 26.496223 & 2.09 & 1.248 & 61.4 & -89.14 & 20.333 & 0.66 & \nodata & \nodata & \nodata & \nodata & -15.45 & -244.99 & 245.47 & 221.83 & 113.81 & 56.06 & \nodata & \nodata  \\
  3429164011534217856 & 87.4158977 & 25.9947762 & 2.048 & 0.896 & -9.08 & -91.38 & 20.145 & 0.337 & \nodata & \nodata & \nodata & \nodata & 126.82 & -170.58 & 212.56 & 305.8 & 133.1 & 54.19 & \nodata & \nodata  \\
  3399867214977802240 & 87.5220758 & 20.5148028 & 1.389 & 0.775 & -23.39 & -69.23 & 19.92 & 0.425 & \nodata & \nodata & \nodata & \nodata & 190.57 & -160.83 & 249.37 & 246.37 & 85.33 & 55.8 & \nodata & \nodata  \\
  3336769201890681088 & 87.6431151 & 10.5632424 & 3.48 & 0.41 & 142.81 & -181.76 & 18.488 & 0.487 & \nodata & \nodata & \nodata & \nodata & -32.51 & -313.13 & 314.81 & 117.43 & 128.67 & 91.58 & \nodata & \nodata  \\
  3457084494415508992 & 91.6018558 & 37.3805445 & 4.209 & 1.247 & 146.44 & -148.03 & 20.535 & 0.932 & \nodata & \nodata & \nodata & \nodata & 63.78 & -225.66 & 234.5 & 178.23 & 175.92 & 68.06 & \nodata & \nodata  \\
  963279255173619840 & 92.1194702 & 45.5036553 & 5.983 & 0.887 & 147.31 & -208.09 & 20.218 & 0.794 & \nodata & \nodata & \nodata & \nodata & 21.41 & -200.85 & 201.99 & 180.19 & 217.75 & 52.46 & \nodata & \nodata  \\
  956217362571364096 & 94.1977572 & 38.6766012 & 2.429 & 0.559 & 50.18 & -102.2 & 19.614 & -0.033 & \nodata & \nodata & \nodata & \nodata & -5.35 & -222.11 & 222.18 & 371.9 & 200.71 & 65.9 & \nodata & \nodata  \\
  3332234708564294272 & 95.5990263 & 13.0594195 & 0.861 & 0.829 & 13.46 & -48.12 & 19.984 & -0.002 & \nodata & \nodata & \nodata & \nodata & 59.57 & -268.66 & 275.18 & 426.49 & 101.01 & 54.22 & \nodata & \nodata  \\
  971164402810466432 & 95.6421956 & 50.2967788 & 1.997 & 0.75 & 114.79 & -18.48 & 20.129 & 0.584 & \nodata & \nodata & \nodata & \nodata & 221.05 & -165.33 & 276.04 & 221.2 & 121.91 & 75.56 & \nodata & \nodata  \\
  953948485966306560 & 102.9326256 & 44.7818967 & 1.521 & 0.998 & 31.65 & -65.45 & 20.229 & -0.103 & \nodata & \nodata & \nodata & \nodata & 12.32 & -226.26 & 226.6 & 531.81 & 183.26 & 56.77 & \nodata & \nodata  \\
  952040627133852800 & 103.0883783 & 42.6805969 & 2.938 & 0.819 & 29.67 & -158.18 & 20.355 & 0.522 & \nodata & \nodata & \nodata & \nodata & -53.44 & -254.09 & 259.64 & 265.16 & 202.27 & 78.42 & \nodata & \nodata  \\
  3381116659072035712 & 103.1115278 & 23.8511315 & 4.531 & 1.409 & 273.45 & -329.35 & 20.476 & 0.494 & \nodata & \nodata & \nodata & \nodata & 130.03 & -428.55 & 447.84 & 290.7 & 589.84 & 83.4 & \nodata & \nodata  \\
  3358236337494875392 & 103.1355128 & 17.0744169 & 1.368 & 0.59 & 22.71 & -58.0 & 19.636 & 0.115 & \nodata & \nodata & \nodata & \nodata & -7.97 & -215.61 & 215.76 & 318.08 & 93.91 & 55.01 & \nodata & \nodata  \\
  937470831051686912 & 103.2039616 & 32.3458302 & 0.934 & 0.407 & 30.52 & -35.27 & 19.647 & -0.053 & \nodata & \nodata & \nodata & \nodata & 75.23 & -224.52 & 236.79 & 385.38 & 85.19 & 63.0 & \nodata & \nodata  \\
  884092526525296640 & 106.2168962 & 27.6386336 & 1.519 & 0.821 & -14.87 & -112.61 & 20.218 & 0.066 & \nodata & \nodata & \nodata & \nodata & -167.92 & -312.11 & 354.41 & 439.81 & 236.8 & 79.08 & \nodata & \nodata  \\
  924723054582853376 & 112.9182082 & 41.7148947 & 2.155 & 1.29 & -69.74 & -131.45 & 20.927 & 0.341 & 158051129183438722 & 20.824 & 0.349 & 0.111 & -228.75 & -234.1 & 327.3 & 436.62 & 307.96 & 72.99 & \nodata & \nodata  \\
  899148139243532032 & 114.1674726 & 38.2891945 & 0.821 & 0.724 & 28.6 & -96.64 & 20.331 & 0.263 & \nodata & \nodata & \nodata & \nodata & 9.15 & -581.77 & 581.84 & 366.19 & 174.93 & 62.4 &  DA  & 6  \\
  880671056793360896 & 118.4195392 & 31.2605592 & 0.78 & 0.435 & 13.16 & -43.29 & 19.438 & -0.471 & \nodata & \nodata & \nodata & \nodata & 18.62 & -274.31 & 274.94 & \nodata & \nodata & 68.58 & \nodata & \nodata  \\
  1032909707356005248 & 122.173552 & 54.8861772 & 0.728 & 0.632 & 21.41 & -39.64 & 20.195 & -0.391 & \nodata & \nodata & \nodata & \nodata & 88.67 & -279.63 & 293.35 & 974.95 & 208.19 & 64.0 & \nodata & \nodata  \\
  928127623619173504 & 122.203988 & 43.7039473 & 0.494 & 0.816 & -4.46 & -77.09 & 20.234 & -0.182 & \nodata & \nodata & \nodata & \nodata & -176.09 & -719.34 & 740.58 & 584.07 & 213.77 & 51.69 &  DA  & 6  \\
  927980048542677248 & 123.7604154 & 43.5326657 & 0.744 & 0.884 & 17.93 & -51.52 & 19.99 & -0.067 & 160241237603960003 & 20.104 & -0.274 & -0.249 & 58.97 & -342.56 & 347.59 & 458.59 & 118.57 & 53.72 & \nodata & \nodata  \\
  708983273892109056 & 126.7955494 & 31.2729189 & 1.793 & 1.066 & -65.61 & -54.14 & 20.563 & -0.078 & 145521267956978239 & 20.485 & -0.019 & -0.149 & -190.77 & -119.16 & 224.93 & 603.94 & 243.5 & 57.52 & \nodata & \nodata  \\
  914266458484496768 & 126.9549724 & 39.1321493 & 2.252 & 0.908 & 62.12 & -111.54 & 20.522 & 0.341 & 154951269549149325 & 20.519 & -0.063 & -0.117 & 99.73 & -249.48 & 268.68 & 362.28 & 219.23 & 73.54 & \nodata & \nodata  \\
  678537968717235072 & 129.0763785 & 24.5469612 & 10.226 & 0.932 & 243.01 & -485.1 & 19.087 & 0.945 & 137451290762277311 & 18.944 & 0.532 & 0.210 & 87.77 & -235.69 & 251.5 & 90.09 & 231.69 & 98.84 &  DQpec  & 4, 12  \\
  710412261051070208 & 130.7056941 & 33.6453844 & 1.578 & 0.626 & -67.36 & -121.33 & 19.857 & 0.052 & 148371307058245324 & 19.897 & -0.085 & -0.115 & -232.67 & -345.87 & 416.84 & 378.21 & 248.78 & 90.59 &  DA  & 7  \\
  1015420295583899776 & 130.7172756 & 50.3988964 & 1.963 & 0.722 & 33.49 & -149.57 & 20.123 & 0.255 & 168471307171969333 & 20.126 & -0.106 & -0.178 & 49.74 & -366.69 & 370.05 & 335.83 & 243.98 & 89.52 & \nodata & \nodata  \\
  1029150236588267520 & 131.1004062 & 51.9287139 & 3.52 & 1.844 & 178.16 & -188.49 & 20.803 & 0.932 & 170311311000085518 & 20.626 & 0.573 & 0.197 & 218.46 & -272.44 & 349.21 & 201.66 & 247.92 & 74.31 & \nodata & \nodata  \\
  716399690274827392 & 132.0347001 & 34.1977731 & 13.733 & 0.675 & -292.73 & -576.84 & 20.018 & 1.202 & \nodata & \nodata & \nodata & \nodata & -114.67 & -191.57 & 223.27 & 103.39 & 317 & 98.42 & \nodata & \nodata  \\
  1014195263537047552 & 132.8692993 & 47.9578412 & 0.568 & 0.682 & -10.41 & -39.23 & 20.084 & -0.19 & \nodata & \nodata & \nodata & \nodata & -106.36 & -321.83 & 338.95 & 551.17 & 106.05 & 54.05 & \nodata & \nodata  \\
  691740358884130432 & 135.1803767 & 26.3170765 & 0.846 & 0.907 & 37.38 & -80.58 & 19.765 & -0.101 & \nodata & \nodata & \nodata & \nodata & 193.9 & -458.1 & 497.45 & 428.3 & 180.34 & 62.76 &  DA  & 12  \\
  718548754471859328 & 135.4326505 & 37.1161381 & 1.62 & 1.108 & -161.25 & -112.4 & 20.555 & 0.299 & \nodata & \nodata & \nodata & \nodata & -481.57 & -314.69 & 575.28 & 387.64 & 361.17 & 80.92 & \nodata & \nodata  \\
  713848372326532608 & 137.731387 & 33.2348463 & 1.277 & 1.215 & -89.94 & -34.04 & 20.624 & 0.287 & 147881377315712482 & 20.581 & 0.001 & -0.075 & -334.18 & -125.25 & 356.88 & 406.36 & 185.23 & 61.78 & \nodata & \nodata  \\
  1024548299384175872 & 139.0633074 & 57.003678 & 1.562 & 0.996 & 20.71 & -71.21 & 20.668 & 0.22 & 176401390633095209 & 20.648 & -0.070 & -0.077 & 65.6 & -215.25 & 225.02 & 450.71 & 158.43 & 55.3 & \nodata & \nodata  \\
  1019449967045185408 & 139.5942891 & 51.8937244 & 1.947 & 1.401 & -53.33 & -95.3 & 20.716 & 0.203 & 170271395943403356 & 20.604 & 0.055 & -0.124 & -125.48 & -234.42 & 265.89 & 470.6 & 243.6 & 62.13 & \nodata & \nodata  \\
  1012116705524378112 & 139.625865 & 48.7221018 & 5.67 & 0.693 & -45.79 & -251.12 & 20.289 & 0.075 & \nodata & \nodata & \nodata & \nodata & -34.29 & -210.61 & 213.38 & 449.98 & 544.44 & 69.21 &  DQ  & 7  \\
  797540517373168000 & 142.9495098 & 34.6962239 & 2.874 & 1.473 & -139.28 & -112.61 & 20.37 & 0.415 & 149631429497036241 & 20.291 & 0.304 & 0.068 & -218.65 & -198.7 & 295.45 & 306.88 & 260.54 & 72.98 & \nodata & \nodata  \\
  800969486118765952 & 144.7536918 & 39.2692757 & 8.802 & 0.78 & 388.04 & -492.59 & 19.826 & 0.888 & \nodata & \nodata & \nodata & \nodata & 229.07 & -248.12 & 337.69 & 135.25 & 402 & 100.0 & WD & 15 \\
  640041558368263424 & 146.3493733 & 21.5200295 & 2.434 & 1.018 & 8.76 & -110.78 & 20.39 & 0.235 & 133821463493964848 & 20.524 & -0.278 & -0.024 & 39.1 & -212.87 & 216.43 & 389.12 & 204.96 & 57.15 & \nodata & \nodata  \\
  646947526477443200 & 147.854113 & 26.9574495 & 1.733 & 2.195 & -114.86 & -166.78 & 20.84 & 0.523 & \nodata & \nodata & \nodata & \nodata & -258.54 & -489.99 & 554.01 & 331.23 & 317.94 & 56.29 & \nodata & \nodata  \\
  643480972473487488 & 149.2148523 & 25.0961978 & 6.032 & 0.574 & -432.65 & -10.48 & 19.801 & 0.785 & 138111492151246020 & 19.836 & 0.308 & 0.195 & -335.8 & -53.85 & 340.09 & 150.26 & 308.25 & 100.0 & WD & 15 \\
  1046146865281895296 & 151.0127437 & 57.2806431 & 2.175 & 1.698 & -56.44 & -121.43 & 20.694 & -0.055 & 176731510128417532 & 20.681 & -0.209 & -0.166 & -80.25 & -280.55 & 291.8 & 625.99 & 397.32 & 64.81 & \nodata & \nodata  \\
  1045429502664329728 & 152.8219188 & 56.4317456 & 0.603 & 0.352 & -54.28 & -8.74 & 19.573 & -0.393 & 175711528219668841 & 19.744 & -0.391 & -0.380 & -407.94 & -142.96 & 432.27 & 737.59 & 192.22 & 81.06 &  DA  & 12 \\
  804369107359559552 & 154.8114379 & 40.9459451 & 2.552 & 0.817 & -9.78 & -121.62 & 20.359 & 0.115 & 157131548114565916 & 20.375 & -0.156 & -0.167 & 25.6 & -225.13 & 226.59 & 443.91 & 256.73 & 64.52 & \nodata & \nodata  \\
  809488360476329088 & 154.8218565 & 45.888586 & 4.155 & 1.683 & -180.81 & -225.68 & 20.657 & 1.016 & \nodata & \nodata & \nodata & \nodata & -152.63 & -292.44 & 329.87 & 171.17 & 234.63 & 77.97 & \nodata & \nodata  \\
  853324381542363136 & 154.8905226 & 56.462368 & 9.369 & 0.787 & -351.27 & -373.67 & 20.445 & 0.928 & 175751548911006063 & 20.372 & 0.626 & 0.308 & -136.17 & -220.85 & 259.45 & 171.78 & 417.58 & 99.71 & \nodata & \nodata  \\
  846852690461618688 & 156.0711659 & 49.3349849 & 4.849 & 2.077 & -70.0 & -396.1 & 20.84 & 1.242 & 167201560711262799 & 20.734 & 0.772 & 0.378 & 13.88 & -392.93 & 393.17 & 144.46 & 275.43 & 72.62 & \nodata & \nodata  \\
  729192473703851264 & 158.1659983 & 28.4565875 & 2.375 & 0.63 & -155.17 & -112.93 & 19.86 & 0.133 & \nodata & \nodata & \nodata & \nodata & -248.45 & -291.44 & 382.97 & 345.39 & 314.19 & 96.35 & \nodata & \nodata  \\
  734945565217194624 & 161.0591851 & 29.6508983 & 1.093 & 1.806 & -49.23 & -50.68 & 20.782 & -0.202 & \nodata & \nodata & \nodata & \nodata & -147.95 & -268.34 & 306.42 & 772.75 & 258.78 & 52.1 & \nodata & \nodata  \\
  780240114227272704 & 162.3530963 & 43.0416738 & 2.701 & 1.761 & -109.39 & -68.49 & 20.425 & 0.583 & \nodata & \nodata & \nodata & \nodata & -151.57 & -168.31 & 226.5 & 253.62 & 155.16 & 55.84 & \nodata & \nodata  \\
  731804943396523264 & 163.1013028 & 29.5007335 & 1.641 & 0.808 & -2.96 & -77.52 & 20.45 & 0.144 & 143401631013331639 & 20.391 & 0.037 & -0.144 & 55.73 & -217.01 & 224.06 & 447.12 & 164.42 & 57.58 & \nodata & \nodata  \\
  729742916713096704 & 163.5807597 & 25.5286321 & 0.975 & 0.872 & 9.35 & -82.48 & 20.553 & 0.103 & 138631635807555027 & 20.615 & -0.196 & -0.080 & 161.49 & -370.03 & 403.73 & 491.92 & 193.56 & 64.74 & \nodata & \nodata  \\
  777395029106166272 & 165.5724246 & 41.2149956 & 28.649 & 0.289 & -102.25 & -1754.7 & 18.772 & 1.357 & \nodata & \nodata & \nodata & \nodata & 73.34 & -281.41 & 290.81 & 49.17 & 409.63 & 100.0 &  DC  & 8  \\
  857027876007243776 & 166.001223 & 57.2534747 & 2.738 & 0.762 & -115.85 & -122.85 & 20.53 & 0.41 & 176701660013935002 & 20.546 & 0.037 & 0.047 & -119.61 & -266.75 & 292.33 & 332.52 & 266.16 & 87.46 & \nodata & \nodata  \\
  838058074908182144 & 167.5329962 & 49.805999 & 5.296 & 1.854 & -262.88 & -200.46 & 20.884 & 0.82 & \nodata & \nodata & \nodata & \nodata & -161.78 & -247.73 & 295.87 & 237.84 & 372.7 & 80.74 & \nodata & \nodata  \\
  764655808213691904 & 168.1400553 & 38.4662383 & 2.043 & 0.735 & -44.26 & -89.18 & 19.703 & -0.268 & 154161681401490261 & 19.793 & -0.262 & -0.287 & -27.74 & -229.35 & 231.03 & 539.54 & 254.61 & 63.88 &  DA  & 12 \\
  788189548935949568 & 168.816665 & 45.8423978 & 5.452 & 1.171 & 348.1 & -298.28 & 20.466 & 0.772 & \nodata & \nodata & \nodata & \nodata & 373.36 & -139.46 & 398.56 & 207.18 & 450.17 & 98.93 & \nodata & \nodata  \\
  765290780473458560 & 169.2007271 & 40.5030671 & 1.438 & 1.355 & -70.89 & -34.0 & 20.127 & 0.012 & 156601692008084327 & 20.102 & -0.037 & -0.201 & -180.66 & -185.76 & 259.13 & 448.38 & 167.1 & 57.9 & \nodata & \nodata  \\
  3970178330024047232 & 169.6586705 & 15.9009058 & 0.469 & 0.71 & 24.76 & -60.72 & 19.916 & -0.27 & 127081696586501742 & 20.036 & -0.250 & -0.261 & 460.29 & -477.35 & 663.13 & 597.85 & 185.84 & 52.22 & \nodata & \nodata  \\
  3967210507622333824 & 171.1584066 & 15.2675422 & 1.333 & 1.029 & 0.14 & -74.57 & 20.68 & 0.123 & 126321711584191755 & 20.792 & -0.315 & -0.157 & 103.0 & -244.38 & 265.2 & 509.55 & 180.1 & 60.18 & \nodata & \nodata  \\
  772157814705317888 & 171.389307 & 43.132527 & 6.727 & 1.008 & -198.44 & -222.27 & 19.96 & 0.95 & \nodata & \nodata & \nodata & \nodata & -72.4 & -197.08 & 209.96 & 134.01 & 189.27 & 61.98 & \nodata & \nodata  \\
  3977100683433224192 & 171.5623042 & 18.224752 & 1.496 & 0.775 & -44.8 & -94.1 & 20.103 & 0.209 & 129871715623890362 & 20.132 & -0.096 & -0.140 & -16.47 & -329.74 & 330.15 & 352.12 & 173.95 & 77.17 & \nodata & \nodata  \\
  3992451210082879488 & 171.7234545 & 22.2768096 & 1.039 & 1.699 & 8.13 & -87.57 & 20.249 & -0.351 & \nodata & \nodata & \nodata & \nodata & 185.7 & -355.51 & 401.09 & 879.83 & 366.79 & 55.96 & \nodata & \nodata  \\
  4018706890623394688 & 171.7969612 & 27.1846689 & 1.378 & 0.605 & -73.35 & -25.58 & 20.063 & 0.049 & \nodata & \nodata & \nodata & \nodata & -201.13 & -175.99 & 267.26 & 417.37 & 153.68 & 71.02 &  DA  & 12 \\
  759058744272603008 & 172.4518762 & 34.3828875 & 2.486 & 0.885 & -94.79 & -131.25 & 19.904 & -0.151 & 149261724520400250 & 19.938 & -0.294 & -0.259 & -73.31 & -299.9 & 308.73 & 481.72 & 369.68 & 83.81 & \nodata & \nodata  \\
  4018843470583215232 & 172.7214869 & 27.9641233 & 1.046 & 1.02 & -101.68 & -65.99 & 19.925 & -0.026 & 141551727215947701 & 20.000 & -0.264 & -0.298 & -311.65 & -452.46 & 549.4 & 425.9 & 244.71 & 67.76 &  DA  & 12 \\
  4032501019908032000 & 176.7150487 & 36.3821109 & 1.203 & 0.979 & -95.87 & -25.59 & 19.9 & -0.104 & 151651767149799336 & 19.984 & -0.152 & -0.185 & -301.57 & -248.79 & 390.95 & 457.46 & 215.16 & 71.71 & \nodata & \nodata  \\
  786798323129999104 & 176.9815593 & 47.970493 & 1.701 & 0.698 & -82.21 & -43.78 & 20.245 & -0.024 & \nodata & \nodata & \nodata & \nodata & -154.9 & -208.22 & 259.52 & 492.13 & 217.27 & 71.25 &  DA  & 7  \\
  4021192852054293632 & 177.4558254 & 30.5497672 & 0.881 & 0.961 & -52.78 & -6.23 & 20.242 & -0.223 & \nodata & \nodata & \nodata & \nodata & -242.98 & -150.49 & 285.81 & 625.73 & 157.64 & 57.87 &  DA  & 11  \\
  4034502719480876160 & 178.0874015 & 39.1777861 & 1.157 & 1.951 & -7.11 & -86.82 & 20.985 & -0.451 & \nodata & \nodata & \nodata & \nodata & 126.45 & -333.76 & 356.91 & \nodata & \nodata & 56.47 & \nodata & \nodata  \\
  4026695083122023552 & 180.1566415 & 32.0574337 & 4.819 & 0.961 & 19.56 & -356.63 & 20.418 & 0.505 & 146461801566289781 & 20.343 & 0.215 & 0.071 & 173.77 & -305.35 & 351.33 & 278.97 & 472.28 & 98.09 & \nodata & \nodata  \\
  1537517065546826368 & 181.6996423 & 42.8395605 & 1.194 & 0.995 & -84.79 & -24.55 & 20.621 & -0.031 & 159401816997628123 & 20.679 & -0.233 & -0.177 & -252.69 & -242.79 & 350.42 & 589.58 & 246.69 & 67.89 & \nodata & \nodata  \\
  3925603372719645184 & 182.3366088 & 16.6772939 & 1.81 & 0.803 & -18.34 & -140.03 & 20.371 & 0.288 & 128011823366493534 & 20.435 & -0.163 & -0.168 & 133.36 & -344.91 & 369.79 & 361.37 & 241.91 & 84.88 & \nodata & \nodata  \\
  4003208934927443584 & 182.3843453 & 25.0283387 & 10.936 & 2.049 & 32.56 & -614.1 & 20.706 & 1.159 & \nodata & \nodata & \nodata & \nodata & 137.06 & -228.6 & 266.54 & 148.89 & 434 & 91.29 & \nodata & \nodata  \\
  4028599883933162496 & 182.6125608 & 33.9049223 & 2.488 & 1.436 & -96.74 & -73.6 & 20.826 & 0.434 & 148681826127576578 & 20.774 & 0.118 & 0.027 & -97.49 & -210.08 & 231.6 & 369.45 & 212.87 & 57.39 & \nodata & \nodata  \\
  3920533662042453760 & 183.7331012 & 12.8493652 & 1.442 & 0.761 & 41.87 & -97.72 & 20.115 & -0.3 & \nodata & \nodata & \nodata & \nodata & 279.1 & -210.43 & 349.54 & 710.73 & 358.15 & 78.48 & WD? & 14 \\
  3908203291972573568 & 185.3695404 & 12.1320703 & 2.657 & 1.725 & -113.35 & -48.26 & 20.707 & 0.427 & 122551853697369057 & 20.550 & 0.207 & 0.025 & -130.04 & -177.2 & 219.8 & 352.75 & 205.98 & 55.02 & \nodata & \nodata  \\
  3901864092042440320 & 185.7784681 & 7.784676 & 1.529 & 1.158 & -65.82 & -14.83 & 20.679 & 0.203 & 117341857786192118 & 20.627 & -0.002 & -0.083 & -149.75 & -146.08 & 209.2 & 462.45 & 147.89 & 50.17 & \nodata & \nodata  \\
  4017082877589080832 & 185.8937387 & 34.6239843 & 5.161 & 1.264 & -146.91 & -184.54 & 20.657 & 0.561 & 149541858939909655 & 20.517 & 0.273 & 0.053 & -33.58 & -214.01 & 216.63 & 290.19 & 324.45 & 62.4 & \nodata & \nodata  \\
  1568682688276118016 & 187.878705 & 50.8549037 & 1.678 & 0.749 & -110.98 & 9.38 & 20.355 & 0.467 & 169021878789616630 & 20.272 & 0.043 & -0.102 & -279.1 & -145.16 & 314.59 & 284.99 & 150.45 & 77.63 & \nodata & \nodata  \\
  3959943251158587520 & 187.9654857 & 24.3254273 & 1.333 & 0.615 & -24.92 & -69.24 & 19.929 & -0.231 & 137191879655261188 & 19.992 & -0.253 & -0.373 & 49.57 & -256.89 & 261.62 & 550.48 & 192.01 & 69.93 &  DAZH  & 12 \\
  3708404196501322624 & 189.0590264 & 6.1930448 & 1.045 & 0.903 & -67.59 & 15.37 & 20.409 & -0.071 & \nodata & \nodata & \nodata & \nodata & -294.43 & -109.93 & 314.28 & 558.19 & 183.41 & 64.39 & WD? & 14 \\
  1543417835215684608 & 189.9399972 & 48.1068825 & 1.536 & 1.511 & -62.8 & -37.75 & 20.772 & -0.101 & \nodata & \nodata & \nodata & \nodata & -98.84 & -203.34 & 226.08 & 681.39 & 236.65 & 53.56 & \nodata & \nodata  \\
  3935585701348778240 & 191.3191598 & 17.0846712 & 1.232 & 1.503 & -85.96 & -53.52 & 20.634 & 0.272 & 128501913191912165 & 20.603 & -0.019 & -0.049 & -167.16 & -352.04 & 389.71 & 416.41 & 199.87 & 55.63 & WD? & 14 \\
  3934327791327194496 & 191.5071315 & 15.9894403 & 0.955 & 0.543 & -25.26 & -39.02 & 19.708 & -0.654 & 127181915072747836 & 19.862 & -0.369 & -0.363 & -0.21 & -230.76 & 230.76 & \nodata & \nodata & 59.24 &  DA  & 12 \\
  3955095916708549504 & 191.5516354 & 22.0201055 & 1.635 & 0.717 & 3.26 & -85.06 & 20.052 & 0.271 & 134421915516864879 & 20.008 & 0.003 & -0.084 & 140.37 & -203.02 & 246.82 & 318.55 & 128.53 & 66.49 & \nodata & \nodata  \\
  1515363624236123136 & 191.5759448 & 34.8617481 & 8.066 & 1.663 & -163.83 & -370.62 & 20.881 & 0.073 & 149831915763244981 & 20.676 & 0.906 & 0.252 & 35.96 & -235.4 & 238.13 & 591.93 & 1136.93 & 77.97 & \nodata & \nodata  \\
  1528518116924626688 & 193.5173249 & 42.7973676 & 2.68 & 2.652 & 7.38 & -147.37 & 20.902 & 0.253 & 159351935173857735 & 20.828 & 0.013 & -0.105 & 157.63 & -208.05 & 261.02 & 482.27 & 337.31 & 58.29 & \nodata & \nodata  \\
  3956422687941416448 & 194.1973105 & 22.2897888 & 0.922 & 0.676 & -47.57 & -2.24 & 19.999 & 0.145 & 134741941974058284 & 19.945 & -0.121 & -0.253 & -197.39 & -144.96 & 244.9 & 362.92 & 81.93 & 54.57 & \nodata & \nodata  \\
  1527701145426221824 & 194.3499628 & 42.3481956 & 1.111 & 0.149 & -51.3 & -58.78 & 17.442 & -0.48 & 158811943500998616 & 17.734 & -0.505 & -0.283 & -37.38 & -330.79 & 332.89 & \nodata & \nodata & 99.89 &  DA  & 1, 13 \\
  1517309381857793920 & 194.6044574 & 36.7147763 & 1.039 & 0.93 & -52.79 & -21.09 & 20.602 & 0.265 & 152051946045378336 & 20.566 & -0.004 & -0.131 & -145.29 & -214.96 & 259.46 & 413.53 & 111.44 & 53.39 & \nodata & \nodata  \\
  3691914373942571904 & 194.9784319 & 1.7018308 & 1.036 & 1.053 & -69.56 & -37.54 & 20.405 & 0.206 & 110041949785432644 & 20.450 & -0.127 & -0.092 & -154.54 & -327.04 & 361.72 & 406.54 & 152.31 & 58.51 & \nodata & \nodata  \\
  3941706961754007936 & 195.1151532 & 19.9040062 & 5.189 & 1.466 & -106.36 & -219.5 & 20.894 & 1.07 & 131881951153905789 & 20.669 & 0.525 & 0.287 & 31.88 & -220.53 & 222.82 & 179.53 & 207.56 & 61.83 & \nodata & \nodata  \\
  1459401025001068288 & 196.9695452 & 25.9570447 & 1.06 & 1.584 & -48.33 & -15.42 & 20.792 & -0.403 & \nodata & \nodata & \nodata & \nodata & -138.26 & -179.75 & 226.77 & 1346.5 & 323.8 & 50.94 & \nodata & \nodata  \\
  1447164972412339584 & 197.1823404 & 24.7922933 & 0.732 & 1.371 & -26.49 & -36.53 & 20.715 & -0.347 & 137751971823611396 & 20.763 & -0.313 & -0.229 & -5.75 & -292.07 & 292.12 & 1075.8 & 230.11 & 50.07 & \nodata & \nodata  \\
  1459966380136554752 & 198.4735241 & 27.4086633 & 0.934 & 0.874 & -2.16 & -67.34 & 20.477 & 0.203 & \nodata & \nodata & \nodata & \nodata & 189.03 & -284.94 & 341.93 & 421.84 & 134.72 & 59.11 &  DA  & 12 \\
  3732580842288407808 & 198.9329868 & 9.565277 & 1.359 & 0.86 & -55.44 & -69.27 & 20.074 & -0.132 & \nodata & \nodata & \nodata & \nodata & -12.66 & -309.18 & 309.44 & 510.78 & 214.81 & 71.24 & \nodata & \nodata  \\
  3936985620169564288 & 199.0623159 & 17.4374818 & 0.899 & 0.946 & 18.85 & -57.95 & 20.437 & -0.048 & 128921990623135622 & 20.460 & -0.078 & -0.103 & 259.05 & -190.0 & 321.26 & 551.76 & 159.39 & 59.38 & \nodata & \nodata  \\
  3744584279448391808 & 199.1433377 & 16.1236377 & 2.514 & 1.839 & -126.93 & -12.27 & 20.93 & 0.726 & 127341991434428939 & 20.839 & 0.236 & 0.044 & -180.51 & -158.82 & 240.44 & 270.31 & 163.4 & 54.06 & \nodata & \nodata  \\
  3744525146338306816 & 199.32236 & 15.8341384 & 1.177 & 0.426 & -64.97 & -2.98 & 19.613 & 0.036 & 127001993224741525 & 19.699 & -0.266 & -0.301 & -204.97 & -163.19 & 262.0 & 344.18 & 106.1 & 73.94 & \nodata & \nodata  \\
  1445708570477675008 & 199.8564202 & 22.5522704 & 1.134 & 0.877 & -46.2 & 23.69 & 20.53 & -0.077 & \nodata & \nodata & \nodata & \nodata & -214.46 & -32.98 & 216.98 & 594.2 & 146.23 & 53.17 & \nodata & \nodata  \\
  3638702276060644864 & 201.3454873 & -1.3646794 & 4.361 & 0.382 & -266.4 & -37.05 & 19.147 & 0.558 & \nodata & \nodata & \nodata & \nodata & -200.5 & -212.71 & 292.31 & 145.36 & 185.32 & 99.97 & \nodata & \nodata  \\
  1473381658945235584 & 201.8084561 & 35.0395267 & 0.768 & 0.716 & -126.48 & -51.73 & 20.377 & 0.158 & \nodata & \nodata & \nodata & \nodata & -426.33 & -728.11 & 843.74 & 425.05 & 275.31 & 66.19 & \nodata & \nodata  \\
  1477073818991419648 & 202.5088359 & 40.9237123 & 1.88 & 0.455 & -69.33 & -59.58 & 20.001 & 0.008 & \nodata & \nodata & \nodata & \nodata & -42.92 & -226.41 & 230.44 & 424.93 & 184.12 & 70.52 & \nodata & \nodata  \\
  1501869592904695168 & 204.4908289 & 44.2747495 & 1.863 & 0.766 & -93.03 & 66.5 & 20.605 & 0.936 & 161132044908910124 & 20.343 & 0.306 & 0.095 & -290.02 & -23.82 & 291.0 & 183.2 & 99.3 & 52.6 & \nodata & \nodata  \\
  1471362203977974144 & 205.4232953 & 35.6253311 & 1.872 & 1.092 & -125.92 & -52.02 & 20.62 & 0.651 & 150752054235411158 & 20.512 & 0.334 & 0.106 & -164.49 & -303.29 & 345.03 & 255.8 & 165.2 & 69.28 & \nodata & \nodata  \\
  3714238583154944512 & 207.0353339 & 5.1109321 & 1.982 & 1.035 & -84.74 & 27.3 & 20.24 & 0.225 & 114132070354693549 & 20.235 & 0.035 & -0.053 & -198.54 & -76.99 & 212.94 & 367.69 & 155.17 & 52.18 & \nodata & \nodata  \\
  3658930743096433536 & 207.8851673 & -1.3827523 & 0.569 & 0.596 & -37.9 & -14.4 & 19.801 & -0.233 & 106342078852371218 & 19.924 & -0.326 & -0.238 & -164.16 & -295.01 & 337.61 & 521.63 & 100.25 & 56.61 &  DA  & 5, 7  \\
  3659052346505556224 & 208.0185948 & -0.9664487 & 1.757 & 1.428 & -84.46 & -37.54 & 20.64 & 0.057 & 106842080187080720 & 20.567 & 0.149 & 0.006 & -109.25 & -224.22 & 249.42 & 539.42 & 236.34 & 58.53 & \nodata & \nodata  \\
  1457242997208273920 & 208.0672152 & 31.390681 & 7.663 & 0.97 & -446.88 & -88.45 & 20.757 & 1.457 & \nodata & \nodata & \nodata & \nodata & -178.14 & -218.32 & 281.77 & 109.74 & 236.96 & 75.28 & BD(esdL0.5)  & 16 \\
  3671868490262516224 & 208.8598958 & 4.5718074 & 3.281 & 0.663 & 102.55 & -113.45 & 19.991 & 0.086 & 113482088597256826 & 20.018 & -0.123 & -0.199 & 218.58 & -32.24 & 220.95 & 387.1 & 280.6 & 68.45 & \nodata & \nodata  \\
  1495840665708099200 & 209.4409855 & 37.9197953 & 1.126 & 0.842 & -64.1 & -14.85 & 20.628 & -0.031 & 153502094411274436 & 20.732 & -0.326 & -0.174 & -161.7 & -224.74 & 276.87 & 591.93 & 184.61 & 63.72 & \nodata & \nodata  \\
  3724461223795155840 & 210.7398109 & 11.6723964 & 1.401 & 0.787 & -73.66 & 12.87 & 20.41 & 0.516 & 122002107398847325 & 20.417 & -0.050 & -0.091 & -220.06 & -124.71 & 252.94 & 274.3 & 97.23 & 58.0 & \nodata & \nodata  \\
  1226400286143982592 & 211.7593753 & 11.7019218 & 0.621 & 0.97 & -42.17 & -0.25 & 20.663 & -0.325 & \nodata & \nodata & \nodata & \nodata & -246.42 & -206.95 & 321.79 & 981.44 & 196.2 & 52.92 & \nodata & \nodata  \\
  3644317722462743680 & 211.8498556 & -4.6663421 & 1.032 & 0.734 & -52.05 & -52.65 & 20.291 & 0.126 & 102402118499460794 & 20.293 & -0.181 & -0.248 & -20.59 & -339.57 & 340.2 & 424.7 & 149.04 & 65.57 & \nodata & \nodata  \\
  1230115295417718144 & 212.6232291 & 14.1037534 & 1.148 & 1.27 & -74.64 & -46.8 & 20.673 & 0.229 & 124922126233305128 & 20.682 & -0.167 & -0.211 & -112.66 & -345.87 & 363.75 & 446.85 & 186.6 & 58.12 & \nodata & \nodata  \\
  6303719789487971456 & 214.2568963 & -11.9244438 & 1.916 & 0.572 & -62.91 & -72.77 & 19.936 & 0.021 & 93692142570121120 & 20.014 & -0.267 & -0.260 & 7.99 & -237.9 & 238.03 & 406.25 & 185.24 & 70.04 & \nodata & \nodata  \\
  3669777253506083456 & 215.8140975 & 5.4035171 & 2.078 & 1.247 & -131.34 & -10.61 & 20.456 & -0.893 & \nodata & \nodata & \nodata & \nodata & -211.53 & -213.53 & 300.57 & \nodata & \nodata & 70.64 & \nodata & \nodata  \\
  3654435424166157312 & 216.4155346 & 1.1572673 & 0.993 & 0.512 & -15.95 & -49.05 & 19.345 & 0.038 & 109382164155049239 & 19.424 & -0.276 & -0.319 & 96.07 & -226.59 & 246.11 & 303.79 & 74.28 & 62.67 &  DA  & 1, 6  \\
  1229171880079404416 & 217.0930476 & 15.8663222 & 1.535 & 1.047 & -74.78 & -53.72 & 20.12 & 0.372 & 127042170931820244 & 20.058 & 0.119 & 0.010 & -65.79 & -276.65 & 284.36 & 289.04 & 126.15 & 63.42 &  DA  & 13 \\
  1241128111253659520 & 218.2670775 & 21.0040366 & 3.743 & 1.494 & -167.19 & -97.3 & 20.705 & 0.303 & 133202182673325570 & 20.640 & 0.274 & 0.009 & -76.45 & -232.7 & 244.94 & 413.41 & 379.06 & 66.51 & \nodata & \nodata  \\
  1228021722197037824 & 218.4276638 & 14.5365108 & 2.64 & 0.682 & -27.83 & -137.58 & 19.937 & 0.06 & 125442184277354517 & 19.909 & 0.072 & -0.124 & 124.84 & -218.97 & 252.06 & 388.92 & 258.77 & 78.41 &  DA  & 13 \\
  1234126691790511232 & 219.3795448 & 15.6747721 & 2.742 & 1.403 & 7.91 & -134.31 & 20.759 & 0.129 & 126812193795900507 & 20.665 & 0.016 & -0.184 & 163.74 & -165.18 & 232.58 & 525.2 & 334.92 & 60.31 & \nodata & \nodata  \\
  1279806318978885888 & 221.2520333 & 27.1763046 & 2.533 & 1.451 & -206.95 & 32.86 & 20.84 & 0.49 & \nodata & \nodata & \nodata & \nodata & -323.91 & -220.9 & 392.07 & 345.69 & 343.35 & 80.25 & M0V & 10  \\
  6330410571691464960 & 221.267966 & -7.9196809 & 1.047 & 1.487 & 27.02 & -50.59 & 20.585 & -0.376 & \nodata & \nodata & \nodata & \nodata & 244.39 & -87.65 & 259.63 & 1114.63 & 303.04 & 54.24 & \nodata & \nodata  \\
  1237640799673210112 & 221.5528902 & 19.9728794 & 1.512 & 0.778 & -39.88 & -60.57 & 20.037 & 0.236 & 131962215530298163 & 20.074 & -0.075 & -0.106 & 35.06 & -224.57 & 227.29 & 330.37 & 113.56 & 57.65 & \nodata & \nodata  \\
  1186164143456393728 & 222.2763149 & 14.8647022 & 9.856 & 0.814 & -86.49 & -445.69 & 20.564 & 1.496 & \nodata & \nodata & \nodata & \nodata & 111.96 & -187.44 & 218.33 & 96.18 & 206.97 & 72.3 & \nodata & \nodata  \\
  1174114969189464576 & 222.7351286 & 9.5961617 & 2.183 & 1.079 & -101.33 & -86.13 & 20.53 & 0.143 & 119512227352915991 & 20.495 & -0.027 & -0.143 & -40.57 & -285.93 & 288.79 & 464.66 & 292.91 & 73.03 & \nodata & \nodata  \\
  3652008492766002560 & 223.1595422 & 0.8628118 & 0.881 & 0.764 & -64.37 & 3.95 & 20.207 & 0.125 & 109032231596365822 & 20.226 & -0.085 & -0.157 & -273.2 & -213.64 & 346.82 & 409.17 & 125.07 & 61.06 &  DA  & 6  \\
  6305347238495511808 & 224.1239163 & -18.3877472 & 0.706 & 0.858 & -60.0 & -43.44 & 20.399 & 0.042 & \nodata & \nodata & \nodata & \nodata & -89.95 & -489.14 & 497.34 & 491.14 & 172.44 & 57.14 & \nodata & \nodata  \\
  6312115905091069952 & 224.7351368 & -13.3420543 & 3.042 & 0.404 & 5.96 & -165.91 & 19.595 & 0.971 & \nodata & \nodata & \nodata & \nodata & 182.31 & -183.55 & 258.71 & 110.52 & 86.97 & 78.73 & \nodata & \nodata  \\
  1180101711219120000 & 225.5056935 & 10.3785003 & 0.948 & 0.31 & -40.55 & -36.08 & 18.132 & 0.079 & 120452255057604739 & 18.190 & -0.122 & -0.146 & -30.39 & -269.75 & 271.45 & 165.84 & 42.66 & 65.36 & \nodata & \nodata  \\
  6227901041052166016 & 226.2721686 & -23.6665035 & 5.209 & 0.905 & -342.25 & -190.87 & 20.032 & 0.592 & 79602262724100711 & 20.007 & 0.178 & -0.026 & -100.37 & -342.21 & 356.63 & 209.38 & 388.92 & 99.37 & \nodata & \nodata  \\
  6318990120507324032 & 227.6506269 & -10.6383495 & 3.764 & 1.269 & -40.99 & -271.63 & 20.674 & 0.033 & \nodata & \nodata & \nodata & \nodata & 191.48 & -288.08 & 345.91 & 563.44 & 733.64 & 89.83 & \nodata & \nodata  \\
  6320306682603175808 & 228.0140076 & -8.8162686 & 1.398 & 0.48 & -30.99 & -65.6 & 19.628 & -0.074 & 97422280140471028 & 19.722 & -0.290 & -0.256 & 70.75 & -235.54 & 245.94 & 391.02 & 134.48 & 70.57 & \nodata & \nodata  \\
  6226688387099769856 & 228.0728988 & -25.5056741 & 0.931 & 1.003 & -32.75 & -69.94 & 20.586 & -0.113 & \nodata & \nodata & \nodata & \nodata & 131.26 & -370.79 & 393.34 & 633.51 & 231.91 & 63.99 & \nodata & \nodata  \\
  6334496013302195200 & 228.9010886 & -6.0739682 & 5.515 & 1.051 & 74.78 & -365.98 & 20.204 & 0.509 & 100712289010381903 & 20.127 & 0.388 & 0.168 & 257.51 & -191.71 & 321.04 & 251.47 & 445.24 & 97.5 & \nodata & \nodata  \\
  6259535231826204544 & 230.1280756 & -16.3040578 & 4.025 & 0.843 & -172.25 & -73.97 & 20.24 & 0.6 & 88432301283235673 & 20.208 & 0.153 & 0.022 & -90.55 & -201.36 & 220.79 & 228 & 202.6 & 67.64 & \nodata & \nodata  \\
  6314180989790944128 & 230.7469407 & -13.446323 & 0.881 & 0.483 & -41.99 & -44.24 & 19.468 & 0.042 & \nodata & \nodata & \nodata & \nodata & -7.81 & -328.14 & 328.23 & 319.93 & 92.5 & 69.05 & \nodata & \nodata  \\
  1209122083683338752 & 231.2618634 & 18.7816809 & 5.81 & 1.197 & -345.09 & -199.44 & 20.629 & 0.704 & \nodata & \nodata & \nodata & \nodata & -91.22 & -312.1 & 325.16 & 241.51 & 456.28 & 96.91 & \nodata & \nodata  \\
  4421166182619455232 & 231.745035 & 2.2528327 & 1.16 & 0.375 & -49.66 & -17.3 & 19.113 & -0.56 & 110702317450533822 & 19.349 & -0.445 & -0.357 & -104.49 & -187.75 & 214.87 & \nodata & \nodata & 58.41 &  DA  & 9  \\
  4420912508966550144 & 232.3337371 & 1.909015 & 15.277 & 1.025 & -414.42 & -643.06 & 20.368 & 1.451 & \nodata & \nodata & \nodata & \nodata & 36.6 & -234.53 & 237.36 & 92.47 & 335.33 & 98.96 & \nodata & \nodata  \\
  6255436183765043840 & 233.0817006 & -17.7213878 & 3.926 & 1.148 & 76.73 & -240.36 & 20.663 & 0.854 & 86732330815575014 & 20.578 & 0.389 & 0.139 & 263.65 & -152.59 & 304.62 & 206.56 & 247.03 & 88.05 & \nodata & \nodata  \\
  6264945000840143744 & 233.6061446 & -15.3597435 & 1.62 & 1.091 & -81.06 & 16.0 & 20.334 & -0.022 & 89562336062888668 & 20.318 & 0.021 & -0.172 & -207.79 & -123.55 & 241.75 & 511.68 & 200.38 & 59.47 & \nodata & \nodata  \\
  1209252027918902016 & 233.7488074 & 17.3092356 & 2.013 & 0.758 & -13.76 & -94.5 & 19.86 & -0.089 & 128772337488551767 & 19.990 & -0.314 & -0.300 & 130.16 & -183.38 & 224.88 & 441.91 & 200.03 & 62.01 & \nodata & \nodata  \\
  6261471162571338112 & 234.339152 & -16.8632152 & 12.485 & 0.956 & -335.24 & -487.08 & 20.053 & 1.153 & 87762343394294881 & 19.940 & 0.722 & 0.271 & 28.81 & -222.63 & 224.48 & 110.98 & 311.06 & 92.1 & \nodata & \nodata  \\
  4403459063250934912 & 235.3375677 & -2.8445498 & 1.655 & 1.001 & -92.56 & 9.65 & 20.649 & 0.246 & 104582353377006914 & 20.580 & -0.048 & -0.051 & -217.35 & -154.23 & 266.51 & 433.08 & 191.03 & 65.98 & \nodata & \nodata  \\
  1196123446766173312 & 235.6253214 & 16.2436992 & 6.06 & 2.394 & -290.41 & -33.84 & 20.58 & 0.974 & \nodata & \nodata & \nodata & \nodata & -146.32 & -175.77 & 228.7 & 173.4 & 240.31 & 61.03 & \nodata & \nodata  \\
  4424976093489782528 & 240.1674725 & 3.5489203 & 2.095 & 1.27 & -10.49 & -100.21 & 20.758 & 0.014 & 112252401674939349 & 20.711 & -0.018 & -0.079 & 132.18 & -185.76 & 227.99 & 598.32 & 285.75 & 57.75 & \nodata & \nodata  \\
  4449852647147141760 & 241.2286124 & 5.6960544 & 1.363 & 1.277 & -17.01 & -80.69 & 20.602 & 0.248 & 114832412286575890 & 20.512 & 0.052 & -0.083 & 142.19 & -249.04 & 286.77 & 422.36 & 165.1 & 58.07 & \nodata & \nodata  \\
  4449711531701855360 & 242.6077279 & 5.6650734 & 1.687 & 1.214 & -113.93 & -114.9 & 20.657 & 0.685 & 114792426078948757 & 20.601 & 0.147 & -0.008 & -25.71 & -453.91 & 454.64 & 250.06 & 191.79 & 64.67 & \nodata & \nodata  \\
  4358438528859200128 & 245.9347756 & -3.0765542 & 6.006 & 0.557 & -176.26 & -205.41 & 19.534 & 0.646 & 104302459350178907 & 19.516 & 0.212 & 0.062 & -2.78 & -213.6 & 213.62 & 156.05 & 200.21 & 75.23 & \nodata & \nodata  \\
  4384725588432355328 & 253.6186858 & 1.7976256 & 9.872 & 0.828 & -398.56 & -177.62 & 20.408 & 1.295 & \nodata & \nodata & \nodata & \nodata & -94.71 & -186.88 & 209.51 & 111.57 & 230.77 & 71.17 & \nodata & \nodata  \\
  6662485730643521152 & 285.1642239 & -47.0305072 & 0.834 & 1.228 & -29.07 & -44.25 & 20.647 & -0.169 & \nodata & \nodata & \nodata & \nodata & 61.84 & -294.47 & 300.89 & 694.51 & 174.3 & 52.66 & \nodata & \nodata  \\
  6662908252346160256 & 286.4667215 & -46.2449114 & 2.305 & 1.357 & -55.44 & -149.71 & 20.521 & -0.486 & \nodata & \nodata & \nodata & \nodata & -1.51 & -328.28 & 328.29 & \nodata & \nodata & 71.76 & \nodata & \nodata  \\
  6644452056320608512 & 286.6744232 & -53.5006599 & 7.121 & 1.342 & -291.12 & -287.55 & 20.588 & 1.191 & \nodata & \nodata & \nodata & \nodata & 112.34 & -248.13 & 272.38 & 136.02 & 263.81 & 89.57 & \nodata & \nodata  \\
  6713142529142569088 & 289.0834679 & -42.2911056 & 0.991 & 1.173 & 8.59 & -51.78 & 20.507 & 0.042 & \nodata & \nodata & \nodata & \nodata & -118.66 & -221.12 & 250.94 & 515.96 & 128.37 & 50.55 & \nodata & \nodata  \\
  6742863844566457472 & 290.2440004 & -35.2053098 & 1.279 & 0.964 & 22.95 & -66.11 & 20.577 & -0.052 & \nodata & \nodata & \nodata & \nodata & -156.89 & -206.61 & 259.42 & 591.17 & 196.09 & 58.23 & \nodata & \nodata  \\
  6745276619756385792 & 291.2040272 & -33.9382153 & 9.173 & 0.654 & 322.52 & -437.08 & 19.476 & 1.181 & \nodata & \nodata & \nodata & \nodata & -226.83 & -165.3 & 280.67 & 82.44 & 212.26 & 93.51 & \nodata & \nodata  \\
  6663268308043562112 & 291.565639 & -46.4606735 & 11.529 & 0.748 & -59.36 & -526.78 & 19.733 & 1.472 & \nodata & \nodata & \nodata & \nodata & -41.38 & -213.99 & 217.96 & 67.4 & 169.36 & 85.96 & WD & 15 \\
  6766131881434082432 & 292.7994046 & -26.8715524 & 1.314 & 1.57 & -33.13 & -82.74 & 20.407 & 0.09 & 75752927994634565 & 20.382 & -0.164 & -0.084 & 28.17 & -320.14 & 321.38 & 466.61 & 197.12 & 56.96 & \nodata & \nodata  \\
  6639093101071983488 & 293.0745223 & -57.480784 & 1.286 & 1.073 & 23.86 & -53.54 & 20.476 & -0.084 & \nodata & \nodata & \nodata & \nodata & -142.11 & -162.71 & 216.03 & 583.77 & 162.19 & 52.55 & \nodata & \nodata  \\
  6446780344049944192 & 293.5278071 & -58.6549717 & 2.309 & 1.513 & 46.27 & -105.37 & 20.879 & 0.637 & \nodata & \nodata & \nodata & \nodata & -153.83 & -179.29 & 236.23 & 292.89 & 159.77 & 55.52 & \nodata & \nodata  \\
  6640949596389193856 & 294.4469228 & -55.6927107 & 1.72 & 0.232 & -34.92 & -190.23 & 17.911 & 0.19 & \nodata & \nodata & \nodata & \nodata & -52.36 & -530.52 & 533.09 & 131.39 & 120.46 & 100.0 & \nodata & \nodata  \\
  6741656752595940608 & 295.0118855 & -34.2405258 & 1.974 & 1.585 & -60.68 & -120.16 & 20.441 & 0.247 & \nodata & \nodata & \nodata & \nodata & 65.46 & -316.54 & 323.24 & 392.87 & 250.67 & 57.33 & \nodata & \nodata  \\
  6684906314626292224 & 295.94713 & -44.4873188 & 0.877 & 0.938 & -37.45 & -16.07 & 20.379 & -0.459 & \nodata & \nodata & \nodata & \nodata & 174.16 & -134.76 & 220.21 & \nodata & \nodata & 51.94 & \nodata & \nodata  \\
  6740533597172140416 & 296.5503422 & -35.5637289 & 4.512 & 0.569 & 42.99 & -194.13 & 19.71 & 0.654 & \nodata & \nodata & \nodata & \nodata & -93.51 & -186.78 & 208.88 & 167.67 & 158.03 & 63.08 & \nodata & \nodata  \\
  6447232101594309632 & 297.6649393 & -58.892855 & 9.047 & 0.603 & 94.54 & -500.78 & 19.962 & 1.281 & \nodata & \nodata & \nodata & \nodata & -111.97 & -242.39 & 267.0 & 92.32 & 223.02 & 99.81 & WD & 15 \\
  6748341817652987904 & 298.8931874 & -31.0579869 & 4.415 & 1.408 & -116.89 & -220.5 & 20.495 & 1.067 & \nodata & \nodata & \nodata & \nodata & 70.27 & -258.55 & 267.93 & 149.84 & 177.25 & 75.05 & \nodata & \nodata  \\
  6449089073654366592 & 298.9594714 & -55.3277045 & 2.091 & 0.743 & 88.44 & -39.29 & 20.347 & 0.079 & \nodata & \nodata & \nodata & \nodata & -215.37 & -41.78 & 219.39 & 459.66 & 210.86 & 59.19 & \nodata & \nodata  \\
  6698374546088091904 & 299.0396368 & -35.4559238 & 8.44 & 0.963 & -267.99 & -356.83 & 20.353 & 0.79 & \nodata & \nodata & \nodata & \nodata & 103.49 & -228.24 & 250.61 & 192.65 & 407.5 & 96.18 & \nodata & \nodata  \\
  6687238623602683008 & 299.1846003 & -40.9788943 & 1.593 & 0.981 & 69.21 & -44.28 & 20.61 & -0.313 & \nodata & \nodata & \nodata & \nodata & -229.48 & -84.54 & 244.56 & 925.95 & 360.62 & 61.42 & \nodata & \nodata  \\
  6685603542438305792 & 300.2161516 & -44.7391979 & 1.272 & 2.037 & -2.82 & -79.91 & 20.873 & -0.54 & \nodata & \nodata & \nodata & \nodata & -50.36 & -293.56 & 297.85 & \nodata & \nodata & 55.86 & \nodata & \nodata  \\
  6699098810716856704 & 301.062208 & -32.965139 & 2.037 & 1.122 & -19.14 & -94.13 & 20.34 & 0.352 & \nodata & \nodata & \nodata & \nodata & 0.91 & -223.53 & 223.53 & 328.26 & 149.46 & 56.36 & \nodata & \nodata  \\
  6686132652344016640 & 301.099572 & -42.2432146 & 2.598 & 1.803 & -53.56 & -137.47 & 20.757 & -0.041 & \nodata & \nodata & \nodata & \nodata & 47.37 & -265.01 & 269.22 & 634.46 & 443.67 & 64.84 & \nodata & \nodata  \\
  6698611009807377152 & 301.2698072 & -34.6687584 & 2.042 & 1.52 & 43.67 & -79.32 & 20.752 & 0.007 & \nodata & \nodata & \nodata & \nodata & -134.91 & -161.2 & 210.21 & 600.89 & 257.91 & 52.71 & \nodata & \nodata  \\
  6700589714124195456 & 301.3136857 & -32.8780843 & 3.17 & 0.88 & -79.36 & -175.26 & 20.381 & 0.225 & \nodata & \nodata & \nodata & \nodata & 65.98 & -280.04 & 287.71 & 392.81 & 358.21 & 86.68 & \nodata & \nodata  \\
  6672990975835965696 & 304.151134 & -44.8168078 & 3.132 & 0.715 & 21.56 & -154.79 & 20.036 & 0.295 & \nodata & \nodata & \nodata & \nodata & -69.59 & -226.03 & 236.5 & 306.9 & 227.35 & 75.08 & \nodata & \nodata  \\
  6668918522205180160 & 304.1799225 & -48.40447 & 0.662 & 0.81 & 27.06 & -38.29 & 19.976 & -0.252 & \nodata & \nodata & \nodata & \nodata & -235.1 & -239.48 & 335.6 & 589.12 & 130.93 & 55.26 & \nodata & \nodata  \\
  6693326924427420800 & 304.4055377 & -38.1979707 & 1.469 & 0.458 & -40.37 & -88.74 & 19.651 & -0.268 & \nodata & \nodata & \nodata & \nodata & 83.85 & -303.23 & 314.61 & 526.52 & 243.3 & 87.49 & \nodata & \nodata  \\
  6680524142314193408 & 304.9986211 & -40.4259533 & 4.81 & 0.765 & 54.64 & -197.06 & 20.067 & 0.487 & \nodata & \nodata & \nodata & \nodata & -82.3 & -183.96 & 201.54 & 243.26 & 235.79 & 52.8 & \nodata & \nodata  \\
  6853349473073333632 & 305.0271048 & -20.9223084 & 0.652 & 0.589 & -43.48 & -98.47 & 19.597 & -0.252 & \nodata & \nodata & \nodata & \nodata & 198.45 & -756.79 & 782.38 & 494.27 & 252.19 & 73.0 & \nodata & \nodata  \\
  6475404544435702656 & 305.1254504 & -51.5169551 & 1.204 & 1.259 & 22.12 & -54.1 & 20.675 & 0.03 & \nodata & \nodata & \nodata & \nodata & -118.17 & -197.38 & 230.05 & 565.06 & 156.54 & 51.57 & \nodata & \nodata  \\
  6694734578483744896 & 306.5910589 & -37.4191614 & 2.593 & 1.03 & -32.93 & -120.81 & 20.497 & 0.382 & \nodata & \nodata & \nodata & \nodata & 30.55 & -226.82 & 228.87 & 339.42 & 201.46 & 59.61 & \nodata & \nodata  \\
  6795420603450748288 & 312.6782242 & -29.2486706 & 2.605 & 0.736 & 47.35 & -131.23 & 19.817 & 0.081 & 72903126781152157 & 19.856 & -0.135 & -0.204 & -101.05 & -232.83 & 253.82 & 359.53 & 237.74 & 77.28 & \nodata & \nodata  \\
  6581307786436278784 & 316.4381139 & -41.745506 & 1.712 & 0.957 & 16.73 & -137.33 & 20.536 & -0.044 & \nodata & \nodata & \nodata & \nodata & -53.22 & -379.3 & 383.02 & 575.35 & 377.3 & 80.5 & \nodata & \nodata  \\
  6462732501127422080 & 319.4040219 & -56.406682 & 1.085 & 0.267 & 54.8 & -75.3 & 18.729 & -0.353 & \nodata & \nodata & \nodata & \nodata & -233.74 & -332.81 & 406.69 & 440.12 & 194.28 & 97.97 & \nodata & \nodata  \\
  6580324376364577152 & 319.4678332 & -43.2533865 & 1.362 & 0.897 & 32.17 & -48.97 & 20.494 & -0.023 & \nodata & \nodata & \nodata & \nodata & -109.01 & -172.26 & 203.85 & 551.61 & 153.2 & 51.58 & \nodata & \nodata  \\
  6576369265535725440 & 322.0012222 & -43.8420438 & 1.721 & 0.918 & -71.21 & -123.46 & 20.493 & 0.464 & \nodata & \nodata & \nodata & \nodata & 211.66 & -330.53 & 392.49 & 304.89 & 205.98 & 80.74 & \nodata & \nodata  \\
  6558768558275852800 & 326.1683186 & -50.8821509 & 1.974 & 0.465 & 84.45 & -27.63 & 19.426 & -0.018 & \nodata & \nodata & \nodata & \nodata & -195.47 & -85.43 & 213.32 & 335.25 & 141.19 & 60.68 & \nodata & \nodata  \\
  6410759415411547264 & 327.4155441 & -58.3883566 & 2.857 & 1.161 & -54.53 & -114.19 & 20.72 & 0.358 & \nodata & \nodata & \nodata & \nodata & 111.43 & -177.96 & 209.97 & 388.31 & 232.91 & 54.61 & \nodata & \nodata  \\
  6410333629532786816 & 327.9245347 & -60.0762402 & 9.37 & 0.964 & 435.17 & -587.46 & 20.615 & 1.395 & \nodata & \nodata & \nodata & \nodata & -182.58 & -321.61 & 369.82 & 110.23 & 381.99 & 98.15 & \nodata & \nodata  \\
  6591844578163525504 & 328.5573188 & -32.3041824 & 1.1 & 1.108 & -25.23 & -41.36 & 20.312 & -0.249 & \nodata & \nodata & \nodata & \nodata & 129.81 & -163.41 & 208.7 & 682.29 & 156.69 & 51.13 & \nodata & \nodata  \\
  6619616764412601472 & 330.5589588 & -26.8101526 & 2.073 & 1.431 & 83.96 & -38.86 & 20.193 & 0.077 & \nodata & \nodata & \nodata & \nodata & -176.58 & -116.45 & 211.52 & 429.46 & 188.34 & 52.35 & \nodata & \nodata  \\
  6571466955503740928 & 331.5771754 & -42.2549553 & 5.534 & 1.484 & 258.47 & -15.97 & 20.929 & 1.378 & \nodata & \nodata & \nodata & \nodata & -216.54 & -48.06 & 221.81 & 129.81 & 159.34 & 52.97 & \nodata & \nodata  \\
  6411523850869878528 & 333.5755444 & -58.0344025 & 8.839 & 0.961 & 144.74 & -507.42 & 20.749 & 1.367 & \nodata & \nodata & \nodata & \nodata & -25.43 & -281.82 & 282.96 & 120.92 & 302.44 & 99.36 & \nodata & \nodata  \\
  6518883327301776256 & 336.6280141 & -45.6225259 & 1.795 & 1.282 & -93.73 & -233.55 & 20.546 & 0.058 & \nodata & \nodata & \nodata & \nodata & 373.39 & -549.85 & 664.65 & 515.96 & 615.47 & 82.8 & \nodata & \nodata  \\
  6620768056166209536 & 337.6210589 & -28.007001 & 2.203 & 0.784 & -4.28 & -164.87 & 20.057 & -0.03 & \nodata & \nodata & \nodata & \nodata & 89.83 & -343.35 & 354.91 & 454.33 & 355.16 & 89.08 & \nodata & \nodata  \\
  6622233670806215808 & 338.196452 & -25.717863 & 1.069 & 0.608 & 54.92 & -20.87 & 19.887 & 0.129 & 77133381962749069 & 19.899 & -0.101 & -0.286 & -214.84 & -147.5 & 260.6 & 351.36 & 97.85 & 62.89 & \nodata & \nodata  \\
  6597521154834007936 & 339.74884 & -34.4345329 & 3.757 & 1.946 & -30.62 & -171.56 & 20.703 & 0.223 & \nodata & \nodata & \nodata & \nodata & 90.95 & -200.17 & 219.87 & 456.73 & 377.27 & 56.8 & \nodata & \nodata  \\
  2397310934852457728 & 342.1566164 & -21.6689875 & 1.097 & 0.814 & 49.21 & -2.67 & 20.337 & -0.331 & \nodata & \nodata & \nodata & \nodata & -200.55 & -71.45 & 212.9 & 859.34 & 200.73 & 53.12 & \nodata & \nodata  \\
  6503816234135502848 & 342.6370756 & -58.1885873 & 0.922 & 0.705 & 63.84 & -0.56 & 20.491 & 0.071 & \nodata & \nodata & \nodata & \nodata & -313.03 & -98.63 & 328.2 & 495.52 & 149.95 & 65.8 & \nodata & \nodata  \\
  6541000931407251072 & 344.2210928 & -44.1531334 & 1.139 & 0.87 & 53.51 & -45.65 & 20.412 & -0.07 & \nodata & \nodata & \nodata & \nodata & -156.75 & -247.18 & 292.69 & 558.49 & 186.2 & 65.44 & \nodata & \nodata  \\
  2400136404857982464 & 346.5763477 & -17.6488552 & 0.937 & 0.953 & 57.93 & -122.91 & 19.949 & 0.336 & 86823465762151904 & 19.961 & 0.006 & -0.125 & -66.45 & -683.79 & 687.01 & 280.05 & 180.36 & 53.7 & \nodata & \nodata  \\
  6549702427775142784 & 346.8447379 & -38.5399124 & 2.301 & 0.86 & 93.56 & -56.12 & 20.343 & 0.333 & \nodata & \nodata & \nodata & \nodata & -145.44 & -171.28 & 224.7 & 336.9 & 174.22 & 61.68 & \nodata & \nodata  \\
  6493817382766475904 & 347.9907655 & -55.9076062 & 2.899 & 0.989 & -84.67 & -93.67 & 20.747 & 0.624 & \nodata & \nodata & \nodata & \nodata & 183.06 & -95.44 & 206.45 & 279.98 & 167.57 & 53.52 & \nodata & \nodata  \\
  6527103001353417472 & 349.3278847 & -47.719468 & 2.083 & 0.774 & 89.66 & 39.06 & 20.001 & 0.455 & \nodata & \nodata & \nodata & \nodata & -222.2 & 11.66 & 222.51 & 245.79 & 113.94 & 60.29 & \nodata & \nodata  \\
  2330002990527676800 & 349.4936535 & -29.3054249 & 1.1 & 0.476 & 45.77 & -11.32 & 19.225 & -0.298 & 72833494935633869 & 19.394 & -0.328 & -0.332 & -167.7 & -114.8 & 203.23 & 468.82 & 104.78 & 51.93 &  DA2.0  & 1, 3  \\
  6526040357725094528 & 351.3267796 & -49.8153021 & 1.946 & 1.027 & 26.41 & -80.74 & 20.594 & 0.185 & \nodata & \nodata & \nodata & \nodata & 13.83 & -206.45 & 206.92 & 454.59 & 183.04 & 52.96 & \nodata & \nodata  \\
  2330134450887360512 & 351.3341907 & -29.2840516 & 3.987 & 1.294 & 164.15 & -88.51 & 20.392 & 0.534 & 72853513339279634 & 20.347 & 0.206 & 0.024 & -142.75 & -169.65 & 221.72 & 265.88 & 235.03 & 61.79 & \nodata & \nodata  \\
  6528897644848988928 & 351.3884108 & -44.9337852 & 0.533 & 0.819 & 40.09 & -1.81 & 20.125 & -0.36 & \nodata & \nodata & \nodata & \nodata & -325.62 & -146.72 & 357.15 & 854.94 & 162.65 & 51.48 & \nodata & \nodata  \\
  2330500455114847232 & 351.5282175 & -28.1726235 & 1.573 & 0.897 & 7.92 & -70.61 & 20.277 & -0.022 & \nodata & \nodata & \nodata & \nodata & 56.67 & -206.43 & 214.07 & 498.63 & 167.94 & 53.23 &  DA  & 2, 5  \\
  2395704136047011968 & 353.343993 & -15.9825526 & 0.714 & 0.813 & 42.08 & -29.9 & 20.244 & -0.415 & \nodata & \nodata & \nodata & \nodata & -174.84 & -294.51 & 342.5 & 1096.74 & 268.33 & 60.05 & \nodata & \nodata  \\
  6539184332039545600 & 354.0321122 & -36.318116 & 1.317 & 1.864 & 88.51 & -26.22 & 20.582 & -0.058 & \nodata & \nodata & \nodata & \nodata & -256.2 & -211.37 & 332.14 & 596.56 & 261.02 & 54.46 & \nodata & \nodata  \\
  6498607748769652352 & 354.0536252 & -52.1373324 & 1.449 & 0.681 & 39.91 & -50.96 & 20.138 & 0.036 & \nodata & \nodata & \nodata & \nodata & -51.83 & -205.28 & 211.73 & 438.39 & 134.5 & 55.0 & \nodata & \nodata  \\
  2393804867149529856 & 355.0962889 & -18.7495341 & 0.528 & 0.621 & 58.69 & -12.67 & 19.836 & -0.388 & 85503550961860928 & 20.004 & -0.380 & -0.357 & -432.21 & -322.51 & 539.28 & 818.67 & 232.98 & 63.52 & \nodata & \nodata  \\
  2334422138213510912 & 358.8053188 & -27.0455611 & 2.784 & 0.872 & 178.74 & -173.86 & 20.526 & 0.365 & 75543588050315925 & 20.454 & 0.087 & 0.006 & -144.37 & -399.26 & 424.56 & 351.82 & 415.82 & 95.43 & \nodata & \nodata  \\
  2421058122564640640 & 358.8616432 & -13.231794 & 2.325 & 1.392 & -57.25 & -103.25 & 20.542 & -0.458 & 92123588616952422 & 20.523 & -0.123 & -0.294 & 200.3 & -133.5 & 240.71 & \nodata & \nodata & 61.47 & \nodata & \nodata  \\
  2326873849154764416 & 359.4225687 & -29.8951177 & 1.078 & 1.149 & -33.53 & -49.0 & 20.62 & 0.226 & 72123594225446228 & 20.458 & 0.262 & -0.102 & 227.28 & -128.44 & 261.06 & 437.65 & 123.17 & 50.41 & \nodata & \nodata  \\
\enddata
\tablerefs{
1. \citet{mccook:99}; 2. \citet{croom:01}; 3. \citet{vennes:02}; 4. \citet{lepine:03}; 5. \citet{croom:04}; 6. \citet{kleinman:04}; 7. \citet{eisenstein:06}; 8. \citet{hall:08}; 9. \citet{girven:11}; 10. \citet{west:11}; 11. \citet{carter:13}; 12. \citet{kleinman:13}; 13. \citet{kepler:15}; 14. \citet{fantin:17}; 15. \citet{kilic:19}; 16. \citet{zhang:19}}
\end{deluxetable*}
\end{longrotatetable}

==> tab4_setc.tex <==
\begin{longrotatetable}
\begin{deluxetable*}{lcccccclcccccccc}
\tablecolumns{16}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecaption{White Dwarf Candidates in Set C \label{tab:tab5}}
\tablehead {
   \colhead{} &
   \colhead{RA} &
   \colhead{Dec} &
   \colhead{$\mu_{\alpha}$} &
   \colhead{$\mu_{\delta}$} &
   \colhead{$G$} &
   \colhead{} &
   \colhead{} &
   \colhead{$r_{\rm PS}$ } &
   \colhead{} &
   \colhead{} &
   \colhead{} &
   \colhead{WD} &
   \colhead{Halo WD} &
   \colhead{} &
   \colhead{}  \\
   \colhead{source\_id} &
   \colhead{(deg)} &
   \colhead{(deg)} & 
   \colhead{(mas yr$^{-1}$)} &
   \colhead{(mas yr$^{-1}$)} &
   \colhead{(mag)} &
   \colhead{$\bpmrp$} &
   \colhead{PS1\_ID} &
   \colhead{(mag)} &
   \colhead{$g_{\rm PS}\, \, -\, \, r_{\rm PS}$} &
   \colhead{$r_{\rm PS}\, \, -\, \, i_{\rm PS}$} &
   \colhead{Halo\_Status} &
   \colhead{Likelihood (\%)} &
   \colhead{Likelihood (\%)} &
   \colhead{Spec\_Type} &
   \colhead{Ref.}
}
\decimals
\startdata
  2417140047238388864 & 3.6801333 & -14.3027568 & 95.22 & -16.06 & 19.608 & 0.673 & 90830036799957120 & 19.544 & 0.219 & 0.054 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  2320117629375536512 & 5.1560428 & -29.920615 & 45.73 & 3.26 & 20.49 & 0.243 & 72090051559605579 & 20.478 & 0.07 & -0.041 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  2349743076832651648 & 12.5277632 & -20.9737167 & 58.39 & -10.95 & 19.396 & 0.151 & 82830125277821944 & 19.126 & 0.145 & -0.172 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  2355740496149824640 & 12.918436 & -20.8993984 & 47.17 & -3.23 & 20.335 & 0.229 & 82920129184271074 & 20.339 & -0.008 & -0.095 & \nodata & 100.0 & 0.01 & \nodata & \nodata \\
  2355806024466166784 & 14.0156541 & -20.6681025 & 46.74 & -21.32 & 20.891 & 0.341 & 83190140156208650 & 20.837 & 0.026 & -0.119 & * & 100.0 & 59.57 & \nodata & \nodata \\
  2359697329260374656 & 15.5801257 & -15.741508 & 42.47 & 0.35 & 20.26 & 0.316 & 89110155800590566 & 20.228 & -0.013 & -0.158 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  5031258418636331520 & 16.2096309 & -30.0769827 & 42.51 & 28.35 & 20.738 & 0.524 & 71900162095197913 & 20.778 & -0.078 & -0.138 & * & 100.0 & 65.78 & \nodata & \nodata \\
  2470708562982465536 & 20.0203554 & -10.1553754 & 43.2 & -4.34 & 20.748 & 0.462 & 95810200202463965 & 20.673 & -0.178 & -0.207 & * & 99.96 & 53.1 & \nodata & \nodata \\
  2471224985554204800 & 21.2886393 & -9.2751516 & 50.06 & 18.1 & 20.693 & 0.423 & 96870212885360164 & 20.7 & -0.187 & -0.207 & * & 99.97 & 99.19 & \nodata & \nodata \\
  5039114257418161280 & 26.0468449 & -23.6735663 & 29.96 & 36.45 & 20.836 & 0.823 & 79590260467662005 & 20.582 & 0.378 & 0.157 & \nodata & 91.48 & 0.0 & \nodata & \nodata \\
  2508768325480884224 & 26.1920683 & -0.8112961 & 119.16 & -25.63 & 20.775 & 1.402 & 107020261919436922 & 20.29 & 0.818 & 0.32 & \nodata & 81.34 & 0.0 & \nodata & \nodata \\
  2511132447278844928 & 26.8352708 & 1.232855 & 3.12 & -52.58 & 20.326 & 0.48 & 109470268352359834 & 20.294 & -0.064 & -0.16 & \nodata & 100.0 & 19.85 & DA & 1, 2 \\
  2505973813599878656 & 27.4353014 & -1.655268 & 110.26 & -52.16 & 20.696 & 0.216 & 106010274353164131 & 20.568 & 0.294 & 0.068 & * & 100.0 & 99.99 & \nodata & \nodata  \\
  2514391915139488384 & 33.3397164 & 2.6388072 & 39.48 & -10.43 & 20.474 & 0.262 & 111160333396997241 & 20.409 & 0.021 & -0.111 & \nodata & 99.41 & 0.0 & \nodata & \nodata \\
  5151755684630745088 & 34.673131 & -10.7551621 & 25.21 & -38.85 & 20.61 & 0.644 & 95090346730504214 & 20.571 & 0.09 & -0.056 & \nodata & 99.34 & 0.3 & \nodata & \nodata \\
  5070059535441127936 & 37.9606765 & -27.5700037 & -42.24 & -37.05 & 20.544 & 0.237 & 74910379606806377 & 20.44 & 0.099 & -0.133 & \nodata & 100.0 & 42.88 & \nodata & \nodata \\
  25097594150205184 & 39.3105684 & 10.7592542 & 36.37 & -21.43 & 20.809 & 0.672 & 120910393104931644 & 20.711 & 0.206 & 0.077 & \nodata & 91.24 & 0.0 & \nodata & \nodata \\
  5177063319860855680 & 40.1086589 & -8.4259041 & 39.8 & -11.02 & 19.775 & 0.975 & 97880401085049355 & 19.14 & 0.466 & 0.121 & \nodata & 55.03 & 0.0 & \nodata & \nodata \\
  14916146541369216 & 47.1402586 & 10.0880542 & 9.68 & -40.13 & 20.735 & 0.064 & 120100471402246268 & 20.721 & -0.077 & -0.087 & \nodata & 100.0 & 2.68 & \nodata & \nodata \\
  5104365427803800832 & 47.3880385 & -18.7638954 & 20.62 & -54.13 & 20.269 & -0.036 & 85480473880463765 & 20.267 & -0.115 & -0.12 & \nodata & 100.0 & 12.73 & \nodata & \nodata \\
  54963211883250304 & 50.9079401 & 16.7883965 & 43.57 & -41.53 & 20.478 & 0.114 & 128140509079286695 & 20.434 & -0.067 & -0.14 & * & 100.0 & 66.45 & \nodata & \nodata \\
  5107552710149616640 & 56.7095376 & -17.6367811 & -38.71 & 20.82 & 20.756 & 0.144 & 86830567095086203 & 20.926 & 0.274 & 0.301 & \nodata & 52.43 & 0.0 & \nodata & \nodata \\
  69967151853011072 & 56.8922425 & 25.6049249 & -40.99 & 21.17 & 20.057 & 0.883 & 138720568921806448 & 19.592 & 0.369 & 0.142 & \nodata & 95.5 & 0.0 & \nodata & \nodata \\
  70916236547866752 & 57.4695225 & 28.2643694 & 78.32 & -103.32 & 20.324 & 0.577 & 141910574694597926 & 20.31 & 0.104 & 0.004 & * & 100.0 & 100.0 & \nodata & \nodata \\
  43785267437420800 & 57.839885 & 17.3410588 & 52.01 & 23.92 & 20.907 & 0.502 & 128800578397369743 & 20.725 & 0.149 & 0.033 & \nodata & 100.0 & 1.38 & \nodata & \nodata \\
  70533567842731008 & 58.1035168 & 26.9999257 & 50.89 & -11.84 & 19.978 & 1.137 & 140400581036150370 & 19.767 & 0.643 & 0.228 & \nodata & 42.16 & 0.0 & \nodata & \nodata \\
  51714532980776576 & 59.4984144 & 21.4906182 & -45.15 & -11.72 & 20.052 & 0.939 & 133780594985359307 & 19.897 & 0.394 & 0.158 & \nodata & 95.35 & 0.0 & \nodata & \nodata \\
  65903906632116608 & 60.8410287 & 23.8044163 & 33.91 & -53.24 & 20.601 & 0.272 & 136560608409875884 & 20.572 & -0.094 & -0.134 & * & 100.0 & 91.71 & \nodata & \nodata \\
  3287109789284560640 & 68.0536514 & 7.7255727 & 31.1 & -29.41 & 20.761 & 0.173 & 117270680535381190 & 20.805 & -0.243 & -0.128 & \nodata & 100.0 & 15.67 & \nodata & \nodata \\
  3313285145348871040 & 68.5059165 & 16.8806257 & 24.99 & -35.06 & 20.644 & 0.391 & 128250685058677308 & 20.587 & 0.09 & -0.054 & \nodata & 100.0 & 0.13 & \nodata & \nodata \\
  3279507220430687232 & 68.5515216 & 2.2946378 & 47.26 & -20.57 & 20.631 & 0.918 & 110750685515053984 & 20.034 & 0.625 & 0.167 & \nodata & 99.71 & 0.0 & \nodata & \nodata \\
  3225103896188242048 & 72.8297584 & -2.7379603 & 86.72 & -189.02 & 20.95 & 0.688 & 104710728295795153 & 20.9 & 0.154 & 0.1 & * & 100.0 & 100.0 & \nodata & \nodata \\
  895798447005540096 & 116.0922234 & 36.6730394 & 32.15 & -129.87 & 20.676 & 0.614 & 152001160921678511 & 20.607 & 0.151 & 0.098 & * & 100.0 & 100.0 & \nodata & \nodata \\
  1081395975413005824 & 119.0099579 & 56.8959881 & -24.58 & -47.3 & 20.639 & 0.579 & 176271190099515955 & 20.548 & 0.098 & -0.114 & \nodata & 99.58 & 22.5 & \nodata & \nodata \\
  877525315369742208 & 119.5933114 & 30.4280434 & -35.94 & -40.36 & 20.846 & 0.326 & 144511195933554299 & 20.793 & 0.153 & 0.029 & \nodata & 99.99 & 2.15 & \nodata & \nodata \\
  902177259417972096 & 122.0259443 & 32.8163095 & -77.62 & -68.74 & 20.773 & -0.034 & 147381220261040388 & 20.729 & 0.695 & 0.384 & \nodata & 97.66 & 0.0 & \nodata & \nodata \\
  683545556987849472 & 122.1106872 & 26.84708 & -27.52 & -30.22 & 20.849 & 0.895 & 140211221106046990 & 20.848 & 0.105 & 0.025 & \nodata & 90.46 & 0.02 & \nodata & \nodata \\
  681030630296850560 & 122.3195645 & 24.7367231 & -52.75 & -12.66 & 20.696 & 1.053 & 137681223196674679 & 20.569 & 0.674 & 0.228 & \nodata & 85.84 & 0.0 & \nodata & \nodata \\
  914989662257379072 & 128.9159205 & 41.7416162 & -7.88 & -48.63 & 20.885 & 0.476 & 158091289159510678 & 20.827 & 0.237 & 0.026 & \nodata & 99.97 & 0.03 & \nodata & \nodata \\
  910234278763116032 & 129.0460867 & 37.9204517 & -29.65 & -27.3 & 20.713 & 0.41 & 153501290460775237 & 20.626 & 0.099 & 0.03 & \nodata & 99.94 & 0.04 & \nodata & \nodata \\
  914014670321623040 & 131.814855 & 43.620202 & -20.63 & -50.78 & 20.877 & 0.911 & 160341318149505022 & 20.735 & 0.343 & 0.099 & \nodata & 97.54 & 0.0 & \nodata & \nodata \\
  704937796950890752 & 131.9808829 & 28.2011163 & 12.73 & -46.18 & 20.71 & 0.259 & 141841319808741987 & 20.566 & -0.121 & 0.187 & \nodata & 99.93 & 0.0 & DAH & 2 \\
  1010494071176681600 & 133.3987754 & 46.4390534 & -7.69 & -41.71 & 20.727 & 0.571 & 163721333986427645 & 20.744 & -0.13 & -0.024 & \nodata & 99.65 & 0.66 & \nodata & \nodata \\
  812282013364243584 & 139.0561236 & 39.4920269 & -19.81 & -52.34 & 20.887 & 0.144 & 155391390561921138 & 20.821 & 0.136 & -0.01 & \nodata & 100.0 & 11.41 & \nodata & \nodata \\
  701210521254140544 & 141.5226486 & 32.7800034 & -106.76 & -22.6 & 20.725 & 0.856 & 147331415228086654 & 20.62 & 0.296 & 0.136 & * & 99.99 & 62.02 & \nodata & \nodata \\
  1021559448822517376 & 143.3008198 & 54.4533526 & -51.86 & -17.87 & 20.651 & 0.376 & 173341433009824749 & 20.611 & -0.006 & -0.049 & \nodata & 100.0 & 5.46 & \nodata & \nodata \\
  808095180461572992 & 150.555926 & 43.8637112 & -56.47 & -31.43 & 20.722 & 1.045 & 160631505559817178 & 20.603 & 0.249 & -0.016 & \nodata & 76.53 & 10.61 & \nodata & \nodata \\
  722523690868494208 & 158.4246628 & 23.6684843 & 22.79 & -54.46 & 19.894 & 0.263 & 136401584246462886 & 19.897 & -0.142 & -0.186 & \nodata & 100.0 & 6.09 & \nodata & \nodata \\
  3987517387875312896 & 161.0088271 & 20.2385842 & -11.56 & -42.37 & 20.477 & -0.139 & 132281610088476926 & 20.582 & -0.302 & -0.187 & \nodata & 100.0 & 25.88 & \nodata & \nodata \\
  854253636371912448 & 163.3029472 & 57.7826251 & -65.34 & -24.58 & 20.963 & 0.725 & 177331633030839918 & 20.834 & 0.457 & 0.15 & \nodata & 99.92 & 0.02 & \nodata & \nodata \\
  3983149131259112448 & 163.7051 & 18.6557853 & -62.93 & -29.21 & 20.836 & 0.776 & 130381637052117545 & 20.776 & 0.192 & 0.145 & \nodata & 98.5 & 0.37 & \nodata & \nodata \\
  837990966043987840 & 167.5983338 & 49.470456 & -37.61 & 21.78 & 20.931 & 1.233 & 167361675984205209 & 20.71 & 0.484 & 0.187 & \nodata & 54.46 & 0.0 & \nodata & \nodata \\
  785046079552350080 & 168.6787067 & 44.5957229 & -48.35 & -43.2 & 20.876 & 0.766 & 161511686787275471 & 20.744 & 0.458 & 0.127 & \nodata & 98.13 & 0.76 & \nodata & \nodata \\
  3997395400339472256 & 168.7379011 & 26.420239 & 42.73 & -34.9 & 20.368 & -0.088 & 139701687378644927 & 20.401 & -0.1 & -0.107 & \nodata & 99.99 & 9.35 & \nodata & \nodata \\
  844211697891241856 & 169.9150884 & 56.0786199 & -24.61 & -64.45 & 20.966 & 0.415 & 175291699150405056 & 20.861 & 0.407 & 0.165 & \nodata & 99.99 & 0.01 & \nodata & \nodata \\
  842862111792610304 & 170.2179782 & 53.9406737 & -53.11 & 9.25 & 20.868 & -0.106 & 172721702180529544 & 20.835 & -0.023 & -0.018 & \nodata & 100.0 & 7.18 & \nodata & \nodata \\
  764141442930300416 & 170.5431374 & 38.5767272 & -64.97 & 7.92 & 20.919 & 0.205 & 154291705432082735 & 20.837 & 0.256 & 0.044 & \nodata & 100.0 & 11.75 & \nodata & \nodata \\
  784094074280983808 & 170.8659063 & 44.1294388 & -90.94 & -45.56 & 20.77 & 0.482 & 160951708659546160 & 20.72 & 0.201 & 0.015 & * & 99.95 & 98.44 & \nodata & \nodata \\
  3992735639996014080 & 171.1427449 & 23.0539407 & -81.78 & 35.39 & 19.919 & 0.464 & 135661711428765211 & 19.901 & 0.017 & -0.032 & \nodata & 100.0 & 11.89 & \nodata & \nodata \\
  4023953214650226176 & 171.3237248 & 32.3877252 & 60.38 & 16.41 & 18.911 & 0.753 & 146861713236745851 & 18.563 & 0.33 & 0.105 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  759122687745444352 & 172.1670506 & 34.522386 & -47.26 & -8.79 & 20.521 & -0.217 & 149421721672237369 & 20.528 & -0.202 & -0.221 & * & 100.0 & 73.13 & \nodata & \nodata \\
  3976945038114078976 & 172.1758374 & 18.5040695 & -44.03 & 10.77 & 20.654 & -0.094 & 130201721759245377 & 20.679 & -0.109 & -0.152 & \nodata & 99.99 & 29.03 & \nodata & \nodata \\
  786245066918092416 & 174.356229 & 46.6400412 & -73.54 & -19.64 & 20.264 & 0.071 & 163961743564198773 & 20.314 & -0.185 & -0.188 & * & 100.0 & 100.0 & \nodata & \nodata \\
  3924301654031558912 & 176.0348944 & 15.4217186 & 41.27 & -48.01 & 20.639 & 0.839 & 126501760349066581 & 20.587 & 0.351 & 0.214 & \nodata & 93.26 & 0.0 & \nodata & \nodata \\
  3975779104816805120 & 176.3270961 & 19.4897703 & -22.72 & -54.72 & 20.198 & 0.5 & 131381763270928423 & 20.133 & 0.043 & 0.002 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4027653101342536192 & 177.8820162 & 32.5364188 & -70.0 & -6.2 & 20.81 & 0.723 & 147041778821824322 & 20.808 & 0.027 & 0.014 & \nodata & 99.13 & 47.17 & \nodata & \nodata \\
  3925168859468263296 & 179.276561 & 15.1328089 & -43.8 & -10.57 & 20.617 & -0.066 & 126151792765939868 & 20.602 & -0.103 & -0.11 & \nodata & 100.0 & 3.62 & \nodata & \nodata \\
  3922599472592544384 & 182.4033279 & 16.5906726 & 62.25 & -27.0 & 20.821 & -0.009 & 127901824032509378 & 20.765 & 0.168 & 0.055 & \nodata & 99.99 & 6.78 & \nodata & \nodata \\
  4030678063989167616 & 182.4326701 & 37.9841321 & 46.16 & -29.4 & 20.975 & 1.242 & 153581824325461630 & 20.794 & 0.34 & -0.042 & \nodata & 63.04 & 15.3 & \nodata & \nodata \\
  3953328902738683008 & 183.7883951 & 21.7446608 & 1.07 & -41.0 & 20.817 & 0.47 & 134091837884284180 & 20.77 & -0.033 & -0.016 & \nodata & 99.63 & 0.02 & \nodata & \nodata \\
  3902485217327647744 & 188.6357864 & 8.0397354 & -82.25 & -24.36 & 20.917 & 0.233 & 117641886359438217 & 20.873 & 0.278 & 0.114 & \nodata & 100.0 & 38.0 & \nodata & \nodata \\
  3933929252722241024 & 191.2169427 & 15.0571278 & -33.05 & 62.79 & 20.719 & 0.743 & 126061912169049263 & 20.619 & 0.587 & 0.242 & \nodata & 99.88 & 0.0 & \nodata & \nodata \\
  3934695788420686336 & 193.0498727 & 17.0574224 & -46.75 & -25.32 & 20.858 & 1.124 & 128461930500549541 & 20.124 & 0.878 & 0.257 & \nodata & 77.67 & 0.0 & \nodata & \nodata \\
  3942043098780692736 & 193.1951543 & 19.7873398 & -40.78 & 2.63 & 20.716 & -0.227 & 131741931951805276 & 20.75 & -0.204 & -0.119 & \nodata & 99.99 & 13.45 & \nodata & \nodata \\
  1555453437387263360 & 195.5969605 & 48.5245948 & -237.83 & -89.9 & 20.667 & 0.601 & 166231955974730327 & 20.426 & 0.466 & 0.219 & * & 100.0 & 100.0 & \nodata & \nodata \\
  3943886159440919808 & 197.5712964 & 22.6083381 & -44.97 & 1.96 & 19.493 & -0.124 & 135131975713210511 & 19.325 & -0.275 & -0.315 & \nodata & 100.0 & 0.0 & DA & 2 \\
  1466879903093949440 & 197.5852262 & 33.0762826 & -17.01 & -40.55 & 20.881 & 1.213 & 147691975849532213 & 20.593 & 0.994 & 0.267 & \nodata & 29.26 & 0.56 & \nodata & \nodata \\
  3743344343864867456 & 200.3675769 & 14.1438575 & -43.07 & -79.71 & 20.98 & 1.116 & 124972003676883142 & 20.841 & 0.951 & 0.363 & \nodata & 96.34 & 0.0 & \nodata & \nodata \\
  3745741893393740928 & 204.0031508 & 17.2517993 & -40.83 & 1.86 & 20.762 & 0.136 & 128702040032772647 & 20.697 & -0.115 & -0.186 & \nodata & 100.0 & 22.56 & \nodata & \nodata \\
  3721647814057772160 & 206.679295 & 8.1119196 & -10.86 & -39.57 & 20.615 & 0.105 & 117732066793524906 & 20.606 & -0.224 & -0.324 & * & 100.0 & 93.94 & \nodata & \nodata \\
  1452628827944168192 & 211.3143129 & 28.5213855 & -41.75 & 32.57 & 20.206 & 0.416 & 142222113143026242 & 19.504 & 0.165 & 0.046 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  6302968002707447168 & 214.714763 & -13.4607929 & -39.2 & 21.14 & 20.883 & -0.091 & 91842147148407369 & 20.786 & 0.135 & 0.052 & \nodata & 100.0 & 0.01 & \nodata & \nodata \\
  1480585113669572096 & 215.1231377 & 34.6368505 & -28.27 & -47.34 & 19.031 & 0.71 & 149562151231464817 & 18.668 & 0.27 & 0.065 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  1183279501686290688 & 228.9436081 & 15.2313771 & -24.31 & -69.15 & 19.779 & -0.448 & 126272289436398212 & 19.988 & -0.461 & -0.383 & * & 100.0 & 100.0 & \nodata & \nodata \\
  6210277935537301120 & 232.2508788 & -28.5379768 & -45.66 & -18.22 & 20.529 & 0.407 & 73752322508954751 & 20.476 & 0.069 & -0.236 & * & 99.18 & 58.42 & \nodata & \nodata \\
  4401968056765783424 & 234.3832556 & -3.223584 & 39.53 & -17.01 & 20.427 & 0.281 & 104132343832162147 & 20.387 & -0.007 & -0.157 & \nodata & 99.76 & 1.87 & \nodata & \nodata \\
  6235898377534605952 & 240.0797341 & -25.132704 & -44.27 & -36.93 & 20.664 & 0.236 & 77842400797811168 & 20.622 & 0.028 & -0.197 & * & 100.0 & 91.09 & \nodata & \nodata \\
  4409810087226545920 & 241.1443803 & 0.0165078 & -39.26 & -31.44 & 20.885 & 0.406 & 108022411444400338 & 20.81 & 0.069 & -0.175 & * & 99.99 & 82.83 & \nodata & \nodata \\
  4350682200175112704 & 248.6540814 & -8.2470068 & -112.14 & -61.81 & 19.753 & 0.997 & 98102486541844008 & 19.172 & 0.431 & 0.222 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4383383733275069312 & 249.7718567 & 0.1884729 & 35.5 & -22.28 & 19.736 & 0.761 & 108222497718596604 & 19.246 & 0.397 & 0.116 & \nodata & 99.06 & 0.0 & \nodata & \nodata \\
  6751824722597647488 & 295.7603482 & -29.9971734 & -30.36 & -41.4 & 20.38 & 0.806 & 72002957602333743 & 19.812 & 0.557 & 0.18 & \nodata & 86.93 & 0.0 & \nodata & \nodata \\
  6755191637657414400 & 297.1150607 & -26.1403626 & 47.2 & -10.13 & 20.958 & 1.035 & 76632971149421899 & 20.976 & 0.125 & 0.018 & \nodata & 73.52 & 2.17 & \nodata & \nodata \\
  6800432138795126144 & 309.2380837 & -24.8241447 & -25.7 & -36.37 & 20.487 & 0.236 & 78213092380991393 & 20.494 & 0.025 & -0.043 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  6785907968149061760 & 322.0572061 & -30.5054837 & -25.4 & -41.76 & 20.657 & 0.046 & 71393220572233856 & 20.619 & -0.043 & -0.069 & \nodata & 99.99 & 16.77 & \nodata & \nodata \\
  6810587606146932096 & 324.594041 & -28.3670898 & 32.92 & -35.0 & 20.159 & 0.134 & 73953245939839871 & 20.142 & -0.085 & -0.194 & \nodata & 100.0 & 8.56 & \nodata & \nodata \\
  6615682265131986560 & 334.6819375 & -27.9647022 & 37.05 & -23.75 & 20.475 & 0.075 & 74443346817672806 & 20.329 & -0.087 & -0.061 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  6614294166062606976 & 336.9697021 & -30.0708141 & 41.76 & 1.3 & 20.508 & -0.121 & 71913369695875347 & 20.572 & -0.139 & -0.135 & \nodata & 100.0 & 6.02 & \nodata & \nodata \\
  2396095459107189120 & 344.1145274 & -23.5388261 & 45.73 & -5.71 & 20.671 & 0.092 & 79753441144323779 & 20.613 & 0.033 & -0.069 & \nodata & 100.0 & 0.62 & \nodata & \nodata \\
  2328352937107620864 & 357.2615792 & -27.5335507 & 3.68 & -59.67 & 20.819 & 0.552 & 74963572615690125 & 20.824 & 0.174 & 0.135 & \nodata & 99.97 & 0.06 & \nodata & \nodata \\
  2339318877674994816 & 358.0884434 & -22.9675101 & -21.92 & -40.33 & 20.543 & 0.957 & 80433580884319341 & 20.502 & 0.202 & 0.099 & \nodata & 85.71 & 0.0 & \nodata & \nodata \\
\enddata
\tablerefs{1. \citet{eisenstein:06}; 2. \citet{kleinman:13}}
\end{deluxetable*}
\end{longrotatetable}



==> tab5_setd.tex <==
\begin{longrotatetable}
\begin{deluxetable*}{lccccccclcccccccc}
\tablecolumns{17}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecaption{White Dwarf Candidates in Set D \label{tab:tab6}}
\tablehead {
   \colhead{} &
   \colhead{RA} &
   \colhead{Dec} &
   \colhead{$\pi$} &
   \colhead{$\sigma_{\pi}$} &
   \colhead{$\mu_{\alpha}$} &
   \colhead{$\mu_{\delta}$} &
   \colhead{$G$} &
   \colhead{} &
   \colhead{$r_{\rm PS}$} &
   \colhead{} &
   \colhead{} &
   \colhead{} &
   \colhead{WD} &
   \colhead{Halo WD} &
   \colhead{} &
   \colhead{}  \\
   \colhead{source\_id} &
   \colhead{(deg)} &
   \colhead{(deg)} & 
   \colhead{(mas)} &
   \colhead{(mas)} &
   \colhead{(mas yr$^{-1}$)} &
   \colhead{(mas yr$^{-1}$)} &
   \colhead{(mag)} &
   \colhead{PS1\_ID} &
   \colhead{(mag)} &
   \colhead{$g_{\rm PS}\,\,-\,\,r_{\rm PS}$} &
   \colhead{$r_{\rm PS}\,\,-\,\,i_{\rm PS}$} &
   \colhead{Halo\_Status} &
   \colhead{Likelihood (\%)} &
   \colhead{Likelihood (\%)} &
   \colhead{Spec\_Type} &
   \colhead{Ref.}
}
\decimals
\startdata
  2361704045355924352 & 5.2793135 & -21.0576421 & 4.355 & 0.222 & -34.45 & -34.98 & 17.285 & 82730052791791209 & 15.295 & 1.193 & -1.324 & * & 100.0 & 100.0 & \nodata & \nodata \\
  5041666743597100928 & 19.655093 & -22.9164157 & 5.461 & 0.175 & 31.32 & -82.7 & 17.677 & 80500196549740655 & 16.453 & -0.349 & 0.056 & \nodata & 80.84 & 0.0 & \nodata & \nodata \\
  2482500275433240832 & 21.0240977 & -4.3160092 & 1.543 & 0.713 & 24.87 & -41.54 & 20.375 & 102820210240741366 & 20.326 & 0.504 & 0.11 & \nodata & 98.09 & 0.0 & \nodata & \nodata \\
  5121322444019559936 & 32.8875957 & -24.837461 & 6.226 & 1.632 & 19.43 & -72.89 & 20.797 & 78190328874785551 & 20.631 & 0.515 & 0.105 & \nodata & 100.0 & 2.6 & \nodata & \nodata \\
  5075663260876120064 & 42.2124742 & -26.5199788 & 5.141 & 0.97 & 1.89 & -40.74 & 20.626 & 76170422124306424 & 20.515 & 0.209 & 0.014 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  5075666598066824192 & 42.2770636 & -26.3861662 & 4.173 & 1.81 & 62.84 & -12.22 & 20.905 & 76330422769286989 & 20.63 & 0.661 & 0.096 & \nodata & 100.0 & 0.1 & \nodata & \nodata \\
  5076603107094492800 & 43.7928599 & -23.8654198 & 2.97 & 0.54 & 36.21 & 24.16 & 19.714 & 79360437927821831 & 19.674 & -0.116 & -0.0 & \nodata & 98.89 & 0.0 & \nodata & \nodata \\
  69571568183047552 & 53.3924201 & 25.9757628 & 5.615 & 1.067 & 30.72 & -34.76 & 20.147 & 139170533923901526 & 20.102 & 0.166 & 0.167 & \nodata & 97.88 & 0.0 & \nodata & \nodata \\
  3279148607839935360 & 67.4960255 & 1.8249609 & 3.704 & 0.191 & 68.1 & -247.04 & 17.856 & 110190674959410756 & 17.473 & 2.115 & 0.283 & \nodata & 99.19 & 0.0 & \nodata & \nodata \\
  3433782686223459584 & 95.2606155 & 28.8865484 & 6.181 & 0.117 & 24.49 & -118.52 & 17.403 & 142660952605714640 & 17.472 & -0.249 & -0.264 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  955484645445590144 & 97.5867639 & 38.1691785 & 4.005 & 0.086 & 13.27 & -43.77 & 15.774 & 153800975867433790 & 15.041 & 0.364 & -0.743 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  974476784668826240 & 110.9800825 & 45.3246857 & 5.313 & 0.175 & -31.53 & -71.54 & 17.535 & 162391109801250397 & 17.61 & -0.262 & -0.313 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  908824842294721152 & 122.9175109 & 38.7000603 & 8.343 & 2.033 & 102.63 & -139.23 & 20.89 & 154441229173590940 & 20.835 & 0.786 & 0.399 & \nodata & 99.93 & 24.66 & DC & 9 \\
  1011412025945567232 & 136.9243253 & 46.341861 & 1.991 & 1.029 & 73.3 & -167.17 & 20.475 & 163611369242541011 & 20.337 & 0.08 & 0.169 & * & 100.0 & 96.26 & \nodata & \nodata \\
  820423832544837376 & 149.760312 & 45.1859286 & 7.223 & 0.591 & -25.63 & -89.67 & 19.717 & 162221497604303887 & 18.632 & 0.028 & -0.04 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  809744825860297984 & 152.2200353 & 44.9822256 & 8.038 & 1.551 & 54.53 & -32.96 & 20.979 & 161971522199729387 & 20.838 & 0.689 & 0.298 & \nodata & 97.2 & 0.0 & \nodata & \nodata \\
  3983149135552914560 & 163.7055791 & 18.6568122 & 2.972 & 0.527 & -63.06 & -23.27 & 19.746 & 130381637057088745 & 19.765 & -0.028 & -0.062 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  3983132471079800704 & 163.9093379 & 18.5703241 & 7.59 & 0.075 & -39.58 & -11.2 & 16.468 & 130281639094225002 & 16.59 & -0.328 & -0.316 & \nodata & 100.0 & 0.0 & DA & 3,5 \\
  3996301764227060096 & 164.6598821 & 25.3655813 & 8.148 & 0.219 & 41.94 & -81.39 & 18.522 & 138431646598559423 & 18.559 & -0.141 & -0.19 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  3994965479641913728 & 166.4545829 & 23.783548 & 8.372 & 0.564 & -11.25 & -88.59 & 19.84 & 136541664545720927 & 19.744 & 0.573 & 0.254 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  3995765275567003520 & 167.0955964 & 25.3722832 & 5.072 & 1.116 & -25.07 & 52.13 & 20.494 & 138441670955737132 & 20.422 & 0.136 & 0.068 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  779106487673928576 & 167.4555045 & 44.5116745 & 10.463 & 1.967 & -12.11 & -131.23 & 20.134 & 161411674554504919 & 19.123 & 0.39 & 0.177 & \nodata & 91.72 & 4.04 & \nodata & \nodata \\
  3991433642135017856 & 167.5910891 & 21.7356013 & 4.854 & 0.532 & -45.41 & -15.06 & 19.766 & 134081675911693308 & 19.746 & -0.013 & -0.115 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  3984115430179696128 & 167.6086461 & 19.207256 & 16.644 & 0.123 & -109.13 & -234.5 & 17.207 & 131041676088009557 & 17.234 & 0.124 & -0.001 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  3971301034475965824 & 167.8896505 & 17.1035725 & 7.246 & 1.331 & -49.26 & -16.45 & 20.507 & 128521678898394727 & 20.342 & 0.091 & 0.1 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  3991483772993312128 & 167.9817132 & 21.7943327 & 3.647 & 0.768 & 30.13 & -40.34 & 19.823 & 134151679817103780 & 19.778 & 0.122 & -0.037 & \nodata & 100.0 & 0.0 & DA & 10 \\
  3998218659671120896 & 168.0952148 & 26.8642571 & 4.833 & 1.446 & -46.84 & 21.91 & 20.808 & 140231680952177712 & 20.694 & 0.044 & -0.048 & \nodata & 100.0 & 5.62 & \nodata & \nodata \\
  3984167931859990400 & 168.1483783 & 19.3402402 & 9.311 & 0.205 & -114.58 & -12.96 & 17.361 & 131201681485488830 & 17.4 & -0.089 & -0.119 & \nodata & 100.0 & 0.0 & DA & 4 \\
  3972130684717312000 & 168.1906072 & 18.9552992 & 6.449 & 0.976 & -22.64 & -48.93 & 19.621 & 130741681906916944 & 19.606 & 0.012 & -0.092 & \nodata & 100.0 & 0.0 & DAH & 4 \\
  3999150942451828480 & 168.2674851 & 29.3809918 & 10.791 & 0.25 & -87.81 & -51.21 & 18.009 & 143251682676687872 & 17.779 & 0.185 & 0.011 & \nodata & 100.0 & 0.0 & DA & 3,4 \\
  3971641608201399936 & 168.7985013 & 17.4017835 & 8.878 & 0.137 & -15.93 & -46.45 & 16.833 & 128881687985092761 & 16.871 & -0.076 & -0.136 & \nodata & 100.0 & 0.0 & DA & 2,4 \\
  4023258765683278720 & 169.4215274 & 30.495085 & 11.165 & 0.24 & -0.83 & -48.97 & 18.216 & 144591694214984758 & 18.213 & 0.056 & -0.006 & \nodata & 100.0 & 0.0 & DA & 3,4 \\
  3997617467328764160 & 170.2517307 & 26.8372401 & 9.698 & 0.289 & 23.92 & -91.13 & 18.769 & 140201702518415154 & 18.748 & 0.197 & 0.045 & \nodata & 100.0 & 0.0 & DA & 4 \\
  3993742891433729408 & 171.2014087 & 24.3058879 & 4.97 & 0.56 & -23.67 & -43.01 & 19.829 & 137161712014567761 & 19.662 & 0.224 & -0.051 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  3980426431229496960 & 171.7572898 & 21.9305264 & 5.503 & 0.124 & -51.2 & 3.31 & 17.177 & 134311717573737226 & 17.276 & -0.309 & -0.276 & \nodata & 100.0 & 0.0 & DA & 10 \\
  3980503087806012800 & 172.7875831 & 22.4126224 & 4.709 & 0.568 & 16.03 & -41.18 & 18.665 & 134891727876025731 & 18.692 & -0.202 & -0.22 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4022610156901792128 & 172.8504258 & 30.0737478 & 5.717 & 1.925 & -54.6 & -56.15 & 20.575 & 144081728504859224 & 20.432 & 0.81 & 0.254 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4018868591847502208 & 173.0637112 & 28.1595623 & 19.613 & 0.108 & -112.72 & 14.75 & 16.906 & 141791730638662035 & 16.908 & 0.098 & -0.014 & \nodata & 100.0 & 0.0 & DAH & 1,3 \\
  4022280612651006976 & 173.1179841 & 28.8258201 & 5.188 & 0.574 & -60.03 & -15.65 & 18.827 & 142591731180771579 & 18.819 & 0.037 & -0.06 & \nodata & 100.0 & 0.0 & DA & 3,4 \\
  4022438598728579456 & 173.6316336 & 29.6426827 & 1.051 & 0.83 & -3.89 & -40.14 & 19.908 & 143571736315861872 & 20.103 & 1.215 & 0.043 & \nodata & 99.63 & 0.0 & \nodata & \nodata \\
  4024276501133339776 & 173.7958453 & 31.1728907 & 6.902 & 0.725 & -21.02 & -78.98 & 19.431 & 145401737958958198 & 19.359 & 0.381 & 0.139 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4025889145389304320 & 174.4861754 & 34.2393557 & 1.969 & 0.381 & -67.08 & -26.65 & 19.362 & 149081744863157900 & 19.448 & -0.277 & -0.333 & * & 100.0 & 100.0 & \nodata & \nodata \\
  4017694519587168128 & 174.5477108 & 26.7448022 & 12.758 & 0.114 & 83.86 & -26.1 & 15.565 & 140091745476004408 & 15.694 & -0.274 & -0.278 & \nodata & 100.0 & 0.0 & DA & 3 \\
  4020999612885617152 & 174.788867 & 30.3958358 & 4.245 & 1.122 & -50.13 & -13.55 & 20.029 & 144471747889445563 & 20.052 & -0.038 & -0.048 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4005382081005433216 & 175.7656704 & 25.7376043 & 11.665 & 0.537 & -182.76 & -33.34 & 19.294 & 138881757659955797 & 19.259 & 0.362 & 0.151 & \nodata & 100.0 & 0.97 & \nodata & \nodata \\
  4017937954038864128 & 176.1643357 & 26.9503584 & 3.244 & 0.252 & -43.89 & -23.4 & 18.69 & 140341761643961109 & 18.738 & -0.25 & -0.254 & \nodata & 100.0 & 0.0 & \nodata & 3 \\
  4005750181176897664 & 176.3382075 & 25.8462052 & 5.149 & 1.109 & -46.36 & -64.71 & 20.117 & 139011763382296061 & 20.04 & 0.141 & -0.045 & \nodata & 100.0 & 5.93 & \nodata & \nodata \\
  4032775038821332608 & 176.4161753 & 37.1908087 & 5.318 & 0.427 & 33.8 & -22.57 & 18.696 & 152621764161649628 & 18.709 & -0.035 & -0.098 & \nodata & 100.0 & 0.0 & DA & 3,4 \\
  4005676616977092480 & 176.4292233 & 25.4904714 & 4.768 & 0.603 & -80.97 & -10.41 & 19.574 & 138581764293489153 & 19.511 & 0.154 & 0.006 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4019789359821201536 & 176.9937656 & 28.532317 & 6.701 & 0.136 & -130.97 & 21.21 & 17.528 & 142231769939589371 & 17.592 & -0.2 & -0.23 & \nodata & 100.0 & 0.0 & DA & 1,2,3,4,5 \\
  4021685368839370368 & 177.1047241 & 32.2850351 & 3.216 & 0.77 & -27.78 & -46.8 & 20.007 & 146741771048332752 & 19.971 & -0.048 & -0.161 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4019886426081471872 & 177.1535009 & 28.7365303 & 2.971 & 1.129 & -58.18 & -14.78 & 20.807 & 142481771536404418 & 20.694 & 0.19 & -0.063 & \nodata & 100.0 & 45.13 & \nodata & \nodata \\
  4005946233549712384 & 177.3204533 & 27.1204496 & 5.79 & 1.957 & -98.64 & -52.9 & 20.719 & 140541773205815225 & 20.657 & 0.376 & 0.202 & \nodata & 100.0 & 8.06 & \nodata & \nodata \\
  4021207592381567744 & 177.4043576 & 30.6651191 & 0.798 & 1.024 & -37.48 & -19.78 & 20.209 & 144791774044458816 & 20.166 & -0.111 & -0.234 & \nodata & 100.0 & 6.67 & DA & 4 \\
  4021196395402263424 & 177.7256714 & 30.608195 & 14.946 & 0.181 & -120.38 & -38.06 & 18.348 & 144731777258800370 & 18.287 & 0.382 & 0.157 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4004546795764990848 & 177.9807979 & 24.0739347 & 7.887 & 1.803 & -44.49 & -44.99 & 20.481 & 136881779808839316 & 20.381 & 0.44 & 0.19 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4005599101408013440 & 178.2324549 & 26.1859403 & 3.298 & 1.17 & -48.51 & -15.87 & 20.33 & 139421782325453787 & 20.263 & 0.189 & 0.08 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4004336965137773056 & 178.2627246 & 23.7941765 & 1.72 & 0.693 & 21.05 & -159.88 & 19.903 & 136551782627393768 & 19.909 & -0.201 & -0.296 & * & 100.0 & 100.0 & \nodata & \nodata \\
  4020555925583936000 & 178.6411266 & 30.8244012 & 4.599 & 0.756 & -42.38 & -2.74 & 20.22 & 144981786411009934 & 20.147 & 0.189 & -0.006 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4004280335994432000 & 178.7389863 & 23.7572692 & 5.285 & 0.684 & -107.15 & -54.42 & 19.948 & 136501787391449344 & 19.93 & 0.011 & -0.045 & * & 100.0 & 100.0 & \nodata & \nodata \\
  4034562466771216128 & 178.8206926 & 39.2597191 & 7.066 & 0.581 & -51.51 & -67.6 & 19.721 & 155111788207182316 & 19.669 & 0.229 & 0.042 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4007541629216778496 & 178.8559291 & 27.8448758 & 11.587 & 0.548 & 119.08 & -186.09 & 19.629 & 141411788557774700 & 19.552 & 0.549 & 0.238 & \nodata & 100.0 & 37.23 & \nodata & \nodata \\
  4026530981006645504 & 179.2543265 & 31.1937726 & 6.156 & 0.474 & 33.65 & -68.0 & 19.653 & 145431792543083170 & 19.606 & 0.145 & 0.003 & \nodata & 100.0 & 0.0 & DA & 6 \\
  4007923739575343104 & 179.2641 & 28.0494166 & 2.723 & 0.744 & -32.62 & -53.06 & 19.552 & 141651792641769952 & 19.582 & -0.286 & -0.243 & \nodata & 100.0 & 25.97 & \nodata & \nodata \\
  4006040379232922880 & 179.5141009 & 25.1732176 & 1.123 & 0.793 & -19.55 & -46.59 & 20.349 & 138201795141158533 & 20.302 & -0.168 & -0.277 & * & 100.0 & 95.99 & \nodata & \nodata \\
  4007958339827909248 & 179.6911372 & 28.3954452 & 5.169 & 0.717 & -57.07 & 33.04 & 20.468 & 142071796912185071 & 20.369 & 0.275 & 0.12 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4031471636506212352 & 179.9131048 & 35.633663 & 21.542 & 0.12 & -218.8 & -166.18 & 17.357 & 150761799133201138 & 17.346 & 0.11 & 0.004 & \nodata & 100.0 & 0.0 & DA6.9 & 1,2,3,4 \\
  4006090720544113792 & 179.9799739 & 25.8213384 & 4.757 & 2.44 & -41.95 & -4.82 & 20.954 & 138981799800456208 & 20.817 & 0.311 & 0.218 & \nodata & 90.41 & 0.0 & \nodata & \nodata \\
  3999265291661178112 & 180.4045994 & 20.3335388 & 9.122 & 0.208 & 40.49 & -57.81 & 18.461 & 132401804045670804 & 18.445 & 0.109 & 0.007 & \nodata & 100.0 & 0.0 & DA & 3,4 \\
  3999369745265960704 & 180.6224226 & 20.6144262 & 2.271 & 0.369 & -55.22 & -9.55 & 19.294 & 132731806225077865 & 19.337 & -0.271 & -0.267 & \nodata & 100.0 & 0.0 & DA & 4 \\
  4002914643768684288 & 180.8320112 & 24.6654862 & 10.076 & 0.11 & -114.52 & 6.31 & 16.753 & 137591808321259141 & 16.838 & -0.235 & -0.23 & \nodata & 100.0 & 0.0 & DBAZ & 2,4,7,8 \\
  4002869490776900864 & 180.841723 & 24.2829358 & 6.505 & 0.538 & -119.96 & -101.12 & 19.791 & 137141808417790209 & 19.684 & 0.651 & 0.27 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4028113212599022592 & 181.1639687 & 34.4453983 & 16.696 & 0.225 & -66.58 & 32.29 & 18.439 & 149331811640215084 & 18.39 & 0.474 & 0.181 & \nodata & 92.68 & 0.0 & \nodata & \nodata \\
  4006739806067153152 & 181.9090895 & 27.2632777 & 13.669 & 0.39 & -137.24 & -143.6 & 19.238 & 140711819093106718 & 19.148 & 0.624 & 0.241 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4028779486581092736 & 182.1069864 & 33.9922521 & 9.232 & 1.282 & -81.46 & -19.03 & 20.708 & 148791821070341365 & 20.587 & 0.685 & 0.322 & \nodata & 98.44 & 0.0 & \nodata & \nodata \\
  4006723455126726016 & 182.3561064 & 27.4811305 & 5.434 & 0.723 & 44.91 & 4.6 & 20.164 & 140971823560377859 & 20.105 & 0.195 & 0.083 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4006707542272362112 & 182.5796883 & 27.3650626 & 6.308 & 0.28 & -47.17 & -33.62 & 18.501 & 140831825797748729 & 18.496 & 0.04 & -0.05 & \nodata & 100.0 & 0.0 & DA & 3,4 \\
  4002779227744626688 & 182.5989258 & 24.7608065 & 8.653 & 0.428 & -95.91 & 1.07 & 19.445 & 137711825990963489 & 19.366 & 0.304 & 0.076 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4013163462233870592 & 182.867709 & 29.2447 & 6.532 & 0.227 & -91.84 & -78.42 & 18.587 & 143091828678564350 & 18.591 & 0.052 & -0.036 & \nodata & 100.0 & 0.0 & DA & 3,4 \\
  4012913117179929344 & 183.9329881 & 28.803763 & 13.328 & 0.32 & 15.24 & -131.28 & 19.116 & 142561839329535381 & 19.05 & 0.537 & 0.216 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4013288359882438016 & 184.0818652 & 28.8588284 & 5.815 & 0.553 & -64.97 & 8.62 & 19.57 & 142631840820531120 & 19.559 & 0.164 & 0.05 & \nodata & 100.0 & 0.0 & DA & 10 \\
  4002256895297236992 & 184.5130042 & 24.8841233 & 3.702 & 1.438 & -49.27 & -2.71 & 20.576 & 137861845131641532 & 20.437 & 0.21 & 0.009 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4010252058522880128 & 184.5285869 & 28.5127871 & 2.581 & 0.404 & -45.51 & 4.5 & 18.994 & 142211845286605902 & 19.002 & -0.205 & -0.211 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4002174290190652416 & 184.6257352 & 24.2475499 & 10.419 & 0.98 & -161.94 & -426.48 & 20.495 & 137091846258577966 & 20.436 & 0.919 & 0.405 & * & 100.0 & 100.0 & \nodata & \nodata \\
  4016935096354518528 & 184.8079309 & 33.6888597 & 5.074 & 0.196 & -55.08 & 6.88 & 17.864 & 148421848080377227 & 17.922 & -0.216 & -0.256 & \nodata & 100.0 & 0.0 & DA & 3,4 \\
  4016930045472966656 & 184.9671167 & 33.5793009 & 3.405 & 0.813 & -45.28 & 13.79 & 20.563 & 148291849672475720 & 20.445 & 0.351 & 0.02 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  1531762329061003264 & 185.8291926 & 38.2663451 & 0.416 & 0.331 & -55.83 & -61.26 & 18.498 & 153921858292130232 & 17.516 & 0.463 & 0.07 & \nodata & 99.98 & 0.0 & \nodata & \nodata \\
  4008477034440224000 & 186.3954787 & 26.3452436 & 17.833 & 0.374 & -400.17 & 287.88 & 19.019 & 139611863958334629 & 18.948 & 0.801 & 0.311 & * & 100.0 & 100.0 & \nodata & \nodata \\
  4008849120340897408 & 186.9108093 & 26.5873692 & 4.141 & 1.503 & -139.88 & -4.5 & 20.719 & 139901869109505438 & 20.546 & 0.453 & 0.127 & * & 100.0 & 99.89 & \nodata & \nodata \\
  4008769474467341312 & 187.169826 & 26.0961172 & 3.904 & 0.855 & 15.9 & -47.0 & 20.327 & 139311871697935978 & 20.255 & 0.283 & 0.082 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  3902672615340360576 & 187.4523504 & 8.0249058 & 1.515 & 0.95 & -37.01 & -69.49 & 19.993 & 117631874524660505 & 19.127 & 1.292 & 0.217 & \nodata & 69.46 & 0.0 & \nodata & \nodata \\
  4011852917388429440 & 187.6002236 & 30.45967 & 5.965 & 0.144 & -14.49 & -54.85 & 17.573 & 144551876000862331 & 17.658 & -0.234 & -0.248 & \nodata & 100.0 & 0.0 & DA3.6 & 1,3,4 \\
  3962146706820263936 & 189.4346911 & 26.8799285 & 5.526 & 1.204 & -37.19 & 30.2 & 20.446 & 140251894347146241 & 20.335 & 0.252 & 0.065 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  3961289401283173248 & 190.1211745 & 25.9965978 & 10.544 & 0.667 & -235.5 & -35.4 & 20.131 & 139191901213256516 & 20.072 & 0.765 & 0.357 & \nodata & 100.0 & 48.83 & \nodata & \nodata \\
  3948209267362328448 & 190.2488445 & 19.6445168 & 3.466 & 0.195 & -85.11 & -5.3 & 16.757 & 131571902487763974 & 15.7 & 0.347 & -0.009 & \nodata & 61.32 & 0.0 & \nodata & \nodata \\
  3954268744662162176 & 191.3332724 & 20.2514108 & 6.926 & 2.115 & -66.27 & 19.69 & 20.834 & 132301913333172183 & 20.671 & 0.578 & 0.202 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  3956389698297187072 & 191.4646836 & 24.3221674 & 8.651 & 0.597 & -77.81 & -99.64 & 19.734 & 137181914648637325 & 19.647 & 0.531 & 0.187 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  3960959096823247744 & 191.5217408 & 25.1924067 & 3.071 & 0.259 & -29.09 & -75.64 & 18.647 & 138231915218071596 & 18.761 & -0.321 & -0.328 & * & 100.0 & 99.49 & \nodata & \nodata \\
  1464839316885981568 & 193.006001 & 29.2629072 & 9.581 & 0.881 & -25.92 & -64.07 & 19.903 & 143111930059226318 & 19.749 & 0.524 & 0.151 & \nodata & 95.22 & 0.0 & \nodata & \nodata \\
  3941125354463573504 & 194.3095359 & 18.7546933 & 7.281 & 0.115 & -48.02 & 9.16 & 17.372 & 130501943096336144 & 17.441 & -0.229 & -0.249 & \nodata & 100.0 & 0.0 & DA & 3,4 \\
  1454785451283968512 & 205.5182836 & 28.4171858 & 0.011 & 1.132 & -41.32 & -25.61 & 20.142 & 142102055183841185 & 19.488 & 0.253 & -0.058 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  3665527198683112832 & 208.6442084 & 3.2218032 & 3.724 & 0.593 & -62.05 & -21.02 & 19.372 & 111862086442696657 & 19.371 & -0.047 & -0.114 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  1233961563189063936 & 213.9246794 & 19.0857227 & 0.832 & 0.624 & -14.31 & -63.16 & 19.755 & 130902139248133346 & 18.46 & 1.481 & -0.32 & \nodata & 96.08 & 32.51 & \nodata & \nodata \\
  6327870223089249664 & 215.7679343 & -10.9789047 & 2.996 & 0.826 & -38.02 & -13.13 & 19.824 & 94822157680385720 & 19.881 & -0.248 & -0.327 & \nodata & 100.0 & 7.3 & \nodata & \nodata \\
  1284442615916116992 & 216.8981488 & 29.7763001 & 0.924 & 0.155 & -4.06 & -53.23 & 17.979 & 143732168982092215 & 17.416 & 0.463 & -0.235 & \nodata & 95.71 & 0.31 & \nodata & \nodata \\
  3643119804543537024 & 217.1276702 & -3.2494162 & 2.374 & 0.547 & -49.35 & 0.01 & 19.882 & 104102171277711087 & 19.957 & -0.265 & -0.084 & \nodata & 100.0 & 0.01 & \nodata & \nodata \\
  1172063108698664832 & 217.9339635 & 6.0585177 & 2.742 & 0.090 & -34.94 &  19.75 & 16.434 & 115272179340590622 & 16.803 & 0.232 & -0.040 & \nodata & 60.02 & 0.0 & \nodata & \nodata \\
  6256819743048506752 & 227.2954492 & -19.5765057 & 14.036 & 0.216 & 9.45 & -121.3 & 18.174 & 84502272954188742 & 18.171 & 0.16 & -0.011 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  6226739514388957952 & 227.4219282 & -25.2897753 & 0.458 & 0.353 & -6.13 & -58.27 & 16.732 & 77652274221262746 & 15.911 & 0.63 & -0.167 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4429660665859520896 & 235.0817391 & 5.9246649 & 0.418 & 0.628 & -41.12 & -17.16 & 19.313 & 115112350817530111 & 18.751 & 0.405 & 0.085 & \nodata & 95.25 & 0.0 & \nodata & \nodata \\
  4427863965075761536 & 235.7349387 & 5.1477761 & 0.11 & 0.056 & 8.77 & -39.78 & 15.724 & 114172357350537600 & 15.558 & 0.034 & -0.306 & \nodata & 88.0 & 0.0 & \nodata & \nodata \\
  6233943548939183104 & 237.2874417 & -26.9602178 & 2.698 & 0.152 & -59.99 & -34.27 & 17.195 & 75642372872788229 & 16.473 & 0.432 & -0.016 & \nodata & 86.27 & 0.0 & \nodata & \nodata \\
  1202750409505163648 & 238.327929 & 17.8075511 & 0.934 & 0.282 & -61.51 & -71.55 & 19.042 & 129362383279999698 & 19.125 & 1.104 & 0.28 & \nodata & 64.88 & 0.0 & \nodata & \nodata \\
  4458059852911092608 & 241.9391857 & 12.6737005 & 5.178 & 1.172 & -74.96 & -3.29 & 20.752 & 123202419393118988 & 20.635 & 0.136 & 0.199 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4348801210657333888 & 243.57444 & -8.0446995 & 4.197 & 0.429 & 24.93 & -68.08 & 19.277 & 98342435744756804 & 19.164 & 0.193 & 0.003 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  4345129047980944512 & 243.9607859 & -9.0156398 & 8.371 & 0.825 & -40.65 & 15.6 & 20.198 & 97182439608151619 & 20.124 & 0.36 & 0.171 & \nodata & 97.94 & 0.0 & \nodata & \nodata \\
  6246092877542423680 & 245.124823 & -18.5493598 & 5.989 & 0.536 & -40.58 & -69.92 & 19.456 & 85742451248151164 & 19.271 & 0.295 & 0.003 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  6805529410278331264 & 313.6252763 & -25.505509 & 3.816 & 0.248 & -29.76 & -30.34 & 15.777 & 77393136252133723 & 15.703 & 0.961 & -1.169 & * & 100.0 & 100.0 & \nodata & \nodata \\
  6788781374284558336 & 318.5671151 & -28.8828849 & 8.29 & 1.276 & -33.39 & -44.09 & 20.496 & 73343185672610938 & 20.294 & 0.464 & 0.129 & \nodata & 91.63 & 0.54 & \nodata & \nodata \\
  6820467066013847936 & 331.8648461 & -20.7416715 & 3.037 & 0.652 & 9.97 & -56.38 & 19.569 & 83113318647860448 & 18.793 & 2.269 & -0.1 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  2342904595544115328 & 13.193195 & -26.6043585 & -11.45 & 1.462 & 29.3 & 99.24 & 19.647 & 76070131932525004 & 18.93 & 0.568 & 0.105 & \nodata & 100.0 & 0.0 & \nodata & \nodata \\
  5069394605783984768 & 40.8795242 & -28.1055145 & -2.651 & 1.671 & 0.32 & -49.68 & 20.762 & 74270408793013755 & 20.096 & 1.473 & 0.085 & \nodata & 93.93 & 0.29 & \nodata & \nodata \\
  1047465080939412608 & 154.6366483 & 59.0896157 & -0.269 & 0.68 & -53.88 & -39.14 & 19.771 & 178901546367758392 & 18.875 & 2.083 & -0.148 & \nodata & 99.98 & 1.93 & \nodata & \nodata \\
\enddata
\tablerefs{1. \citet{mccook:99}; 2. \citet{debes:11}; 3. \citet{girven:11}; 4. \citet{kleinman:13}; 5. \citet{guo:15}; 6. \citet{kepler:15}; 7. \citet{koester:15}; 8. \citet{limoges:15}; 9. \citet{dame:16}; 10. \citet{kepler:16} }
\end{deluxetable*}
\end{longrotatetable}


==> tab6.tex <==
\begin{deluxetable*}{cl}
\tablecolumns{2}
\tablewidth{0pt}
\tabletypesize{\footnotesize}
\tablecaption{Column Description Provided in Tables\label{tab:tab2}}
\tablehead{
	\colhead{Header} &
	\colhead{Description}
}
\startdata
 source\_id & \gaia DR2 unique source identifier \\
 RA & Right ascension in J2015.5 (deg) \\
 Dec & Declination in J2015.5 (deg)  \\
 $\pi$ & \gaia DR2 parallax (mas) \\
 $\sigma_{\pi}$ & \gaia DR2 standard error of parallax (mas) \\
 $\mu_{\alpha}$ & \gaia proper motion in right ascension direction (mas yr$^{-1}$) \\
 $\mu_{\delta}$ & \gaia proper motion in declination direction (mas yr$^{-1}$) \\
 $G$ & \gaia $G$-band mean magnitude (mag) \\
 $\bpmrp$ & \gaia BP - RP color (mag) \\
 PS1\_id & \panstarrs DR1 identifier \\
 $r_{\rm PS}$ & \panstarrs $r$-band magnitude (mag) \\
 \gmr & \panstarrs \gmr~color (mag) \\
 \rmi & \panstarrs \rmi~color (mag) \\
 $v_{T,\,r}$ & Transverse velocity in $r$~direction from \gaia parallax (km s$^{-1}$) \\
 $v_{T,\,s}$ & Transverse velocity in $s$~direction from \gaia parallax (km s$^{-1}$) \\
 $v_{T,\,{\rm tot}}$ & Total transverse velocity from \gaia parallax (km s$^{-1}$)\\
 Phot\_Dist & Photometric distance for Set B only (pc) \\
 $v_{T,\,{\rm phot}}$ & Total transverse velocity from photometric distance for Set B only (km s$^{-1}$)\\
 WD Likelihood & Confidence level to pass the white dwarf selection (\%)\\
 Halo WD Likelihood & Confidence level to pass the the halo white dwarf selection expressed (\%)\\
 Halo\_Status & Halo status of white dwarf candidates for Sets C and D only\tablenotemark{a} \\
 Spec\_Type & Spectral type of a known white dwarf given in the SIMBAD database \\
 Ref. & References \\
\enddata
\tablenotetext{a}{\*: Halo white dwarf candidates with likelihood $> 50$\%}
\end{deluxetable*}

